VulLibGen: Generating Names of Vulnerability-Affected Packages via a Large Language Model

Security practitioners maintain vulnerability reports (e.g., GitHub Advisory) to help developers mitigate security risks. An important task for these databases is automatically extracting structured information mentioned in the report, e.g., the affected software packages, to accelerate the defense of the vulnerability ecosystem. However, it is challenging for existing work on affected package identification to achieve a high accuracy. One reason is that all existing work focuses on relatively smaller models, thus they cannot harness the knowledge and semantic capabilities of large language models. To address this limitation, we propose VulLibGen, the first method to use LLM for affected package identification. In contrast to existing work, VulLibGen proposes the novel idea to directly generate the affected package. To improve the accuracy, VulLibGen employs supervised fine-tuning (SFT), retrieval augmented generation (RAG) and a local search algorithm. The local search algorithm is a novel postprocessing algorithm we introduce for reducing the hallucination of the generated packages. Our evaluation results show that VulLibGen has an average accuracy of 0.806 for identifying vulnerable packages in the four most popular ecosystems in GitHub Advisory (Java, JS, Python, Go) while the best average accuracy in previous work is 0.721. Additionally, VulLibGen has high value to security practice: we submitted 60 <vulnerability, affected package> pairs to GitHub Advisory (covers four ecosystems). 34 of them have been accepted and merged and 20 are pending approval. Our code and dataset can be found in the attachments.

==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.63	New journals: TQUANT, FACMP

Version 1.63a   Moved TQUANT to TQC

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

==> backup/abstract-backup.tex <==
To avoid potential risks posed by vulnerabilities in third-party packages, security practitioners  maintain vulnerability reports in vulnerability databases (e.g., GitHub Advisory) to help developers realize and deploy vulnerability patches.
However, existing work shows that in more than half of the vulnerability reports, the field of vulnerability-affected packages is missing or incorrect.
% \xueqing{is "missing or incomplete" correct?}. 
To help improve the affected-package field in vulnerability databases, existing work seeks to rank existing packages based on their similarity to the vulnerability description in each vulnerability report, incurring high analysis cost. 
%Nevertheless, due to the high inference cost, ranking-based approaches cannot scale to larger language models. 
%To leverage the capability of LLMs for vulnerable package identification, 
To address this issue, in this paper, we propose to directly generate the package names rather than ranking them, to maintain a relatively low inference cost. First, we conduct a pilot study to examine the feasibility of LLM generation for this task, which shows that the raw generation output has a 42\% accuracy. Based on the study results, we propose a \detector{} framework by employing the retrieval augmented generation (RAG) and a post-processing local search algorithm so the generated package must exist. Our evaluation results show that \detector{} has an average accuracy of 0.806 for identifying vulnerable packages in the four most popular ecosystems in the GitHub Advisory database (Java, JS, Python, Go) while the SOTA ranking-based approach achieves 0.721. 
Additionally, \detector{} has shown high value to security practice. 
We have submitted 28 pairs of <vulnerability, affected package> to GitHub Advisory, and 22 of them have been accepted and merged.

==> backup/approach-backup-1.tex <==
\begin{figure*}[t]
\centering
\includegraphics[width=1\linewidth]{figures/workflow.drawio.pdf}
\caption{\detector{} Framework}
\label{fig: framework}
\end{figure*}


\section{Approach}\label{sec:approach}
In this section, we introduce the framework of \detector{} which we illustrate in Figure~\ref{fig: framework}.
Our key insight is to address the scalability problems faced by existing retrieval approaches by utilizing the generation capabilities of Large Language Models (LLMs).


Given the input description of a vulnerability, \detector{} leverages a LLM to generate a package name given the following prompt: "\emph{Below is a [Programming Language] vulnerability description. Please identify the software name affected by it. Input: [DESCRIPTION]. The top k search results are: [$L_1$][$L_2$]$\cdots$[$L_k$]. Please output the package name as the format "ecosystem:library name".
\#\#\# Response: The affected packages:}". To address the challenges in the generation approach, our framework includes the following components: 
(1) \textbf{Before generation}: We leverage retrieval augmented generation (RAG)~\cite{lewis2020retrieval} to reduce the hallucination in the generation results. In particular, we add the top k retrieved package names to the prompt; (2) \textbf{During generation}: since the generated package name may not exist, we leverage constrained decoding~\cite{hokamp2017lexically,anderson2016guided} so the generation result includes the name(s) of at least one existing package(s); 
(3) \textbf{Post generation}: we further match the generation result with the closest package name in the list of existing package names. Below we explain each component in more details. 


\subsection{Before Generation: Retrieval Augmented Generation (RAG)}

Retrieval augmented generation (RAG) is a framework that enhances the performance of a generative model by incorporating knowledge from an external corpus~\cite{lewis2020retrieval,gao2023retrieval}. Given the user input, RAG leverages a retrieval model to obtain the top-$k$ most similar paragraphs/documents, and combine them in the input for the generation~\cite{gao2023retrieval}. RAG can solve the problem of hallucination when the generative model lacks knowledge of the corpus. Since our initial study (Section~\ref{sec: empirical_study}) shows that hallucination also exists in our raw generation results. we employ RAG in VulLibGen. 

\noindent \textbf{Retriever setting}. Given the description of a vulnerability, our retriever ranks all the unique package names (Table~\ref{tab: dataset info}) based on their similarity $sim(d_v, d_p)$ with the description, where $d_v$ and $d_p$ are the descriptions of the vulnerability $v$ and package name $p$. The descriptions for packages in Java and Python are obtained from the Maven~\footnote{https://mvnrepository.com} and Pypi~\footnote{https://pypi.org} documentations while for JavaScript and Go are from NPM~\footnote{https://www.npmjs.com} and Go~\footnote{https://pkg.go.dev}.
For example, the description of the package ``org.jenkins -ci.plugins:mailcommander'' is \textit{``This plug-in provides function that read a mail subject as a CLI Command.''}.
We use two models for the similarity function: TF-IDF, and a BERT-base model fine-tuned on GitHub Advisory.


\subsection{During Generation: Constrained Decoding}

Although RAG 

We design our constrained decoding algorithm to restrict the open-source LLMs to include the name of at least one existing package.
This constraint is written as follows:

\begin{equation*}
    \exists l \in \mathcal{L}, \mbox{ s.t. } l \in \mathcal{F}_{generation} (v)
\end{equation*}

However, adopting constrained decoding has two technical challenges to address.
First, each package name contains more than one token (e.g., Python packages have 6 tokens on average) while LLMs generate only one token at once.
Therefore, we cannot greedily check whether the constraints are satisfied during decoding.
To address this challenge, we construct a Trie tree to represent the constraints (as shown in Figure~\ref{fig: framework}) and then conduct beam search~\cite{kumar2013beam} to ensure that the output contains at least one path (corresponding to an existing package name) on this Trie tree.

Second, the large number of packages in each ecosystem (e.g., 435,642 in Maven and 506,848 in Pypi) brings a heavy efficiency burden as the Trie tree for constrained decoding might have more than 1,000,000 nodes. 
We empirically notice that invoking an LLM with 7B parameters might cost more than 2 hours, which is unacceptable.
To address this challenge, we follow the similar idea of VulLibMiner, using a TF-IDF~\cite{jones1972statistical, jones2004idf} technique to filter a small candidate of packages.
Its empirical results indicate that 512 is a proper candidate size with a recall of at least 0.9.
Thus, the decoding constraint is modified as:

\begin{equation*}
\begin{aligned}
    &\mathcal{L}(v) = \mathop{\mbox{Top512}}\limits_{l_i \in \mathcal{L}}\ TF\mathit{-}IDF(v, l_i) \\
    &\exists l \in \mathcal{L}(v), \mbox{ s.t. } l \in \mathcal{F}_{generation} (v)
\end{aligned}
\end{equation*}

\subsection{Post Generation: Local Search}
We design our local search algorithm to find the closest package name from the output of LLMs.
The input of this algorithm includes one package name generated by LLM together with the name list of existing libraries under the same ecosystem.
The output of this algorithm is the name of one existing package that is the closest to the generated package name.

This technique can help address the former three types of incorrect responses based on the observation in Table~\ref{tab: fault case study} that the generated name has already specified the targeted library (i.e., most components of this generated name are correct) with only slight differences.
Therefore, we use the Levenshtein distance to find the closest and existing package name as the output of this algorithm.
The details of this algorithm are listed in the Appendix.

Additionally, we conduct a two-staged local search when given a Java vulnerability because the names of Java packages are relatively complex and structural compared to package names of other programming languages. 
A Java package name consists of its group ID and artifact ID.
In this scenario, we first search for an existing artifact ID and then search for an existing group ID corresponding to this artifact ID.
Our rationale is that the artifact IDs include each package's functionalities, which is easier to identify from a vulnerability's description.





% Unlike conventional information retrieval (IR)/classification approaches, \detector{} utilizes the tremendous capabilities of Large Language Models (LLMs) in comprehending vulnerability descriptions.
% Our key insight is that conventional approaches highly depend on their training set and thus face the scalability problem and this problem can be alleviated by modeling this task as a generation task.

% As formalized in Section~\ref{sec: formal}, the training input of \detector{} includes the textual descriptions of vulnerabilities, $\mathcal{V}$, the textual descriptions of all Java libraries in Maven, $\mathcal{L}$, and the mapping relationship from vulnerabilities to libraries, $\mathcal{M}$.
% When applied in practice, \detector{} takes only the textual descriptions of one vulnerability as input and outputs a series of names of libraries affected by this vulnerability.


% \begin{figure}[t]
% \centering
% \includegraphics[width=1\linewidth]{figures/approach-illustration.drawio.pdf}
% \caption{An Illustration of the Motivation of our RAG and Constrained Decoding/Local Search Techniques}
% \label{fig: case}
% \end{figure}

% \subsection{Fine-tuning and Prompt-tuning}




% LLMs can correlate the input vulnerability description to vulnerable libraries based on their prior knowledge of these libraries, e.g., their functionalities, usages, and even history issues.

% As formalized in Section~\ref{sec: formal}, the training input of \detector{} includes the textual descriptions of vulnerabilities, $\mathcal{V}$, the textual descriptions of all Java libraries in Maven, $\mathcal{L}$, and the mapping relationship from vulnerabilities to libraries, $\mathcal{M}$.
% When applied in practice, \detector{} takes only the textual descriptions of one vulnerability as input and outputs a series of names of libraries affected by this vulnerability.


% The process of \detector{} is shown in Figure~\ref{fig: framework} with two steps.
% First, we conduct unsupervised fine-tuning on Maven Corpus, which includes all Java libraries and their descriptions.
% This step aims at activating their knowledge of each Java library, including its name and functionalities.
% Second, we conduct supervised fine-tuning on the input dataset $(\mathcal{V}, \mathcal{L}, \mathcal{M})$ to learn the mapping relationship from vulnerabilities to libraries.



% During supervised fine-tuning, we design two specific techniques to improve the effectiveness of \detector{}.
% To help identify zero-shot libraries, we design an input augmentation technique, which feeds the names of vulnerable libraries (a.k.a., recommended libraries) identified by the SOTA approach~\cite{vullibminer} to \detector{} as input.
% This technique provides examples of libraries whose functionalities are likely to be affected by a given vulnerability.
% Thus, \detector{} can generate library names from those with similar functionalities instead of all libraries when \detector{} has no prior knowledge of how these zero-shot libraries are affected by vulnerabilities.
% To address \detector{}'s hallucinations, we design our post-processing technique based on the Levenshtein distance~\cite{levenshtein} to obtain existing Java library names from the response of LLMs.
% We find that \detector{} can generate the components of the targeted library names (i.e., the targeted functionalities and scopes), and make mistakes when jointing these components of library names, thus leading to hallucinations.
% Therefore, hallucination library names are close to the targeted names of vulnerable libraries, and their closest library names tend to be the targeted names.


% \subsection{Two Stages of Fine-Tuning with Input Augmentation}
% \detector{} mainly consists of two stages of fine-tuning on LLMs.
% In this paper, we choose one of the state-of-the-art (SOTA) open-source LLMs, LLaMa~\cite{llama}, as our base LLM with 7B and 13B parameters.

% During unsupervised fine-tuning, \detector{} takes the input of one library description, and its targeted output is its library name.
% Table~\ref{tab: lib-aws} shows an example case in this step.
% Its input describes the functionality of this package, e.g., configuration on AWS plugins, and its output is a structural Java library name, \CodeIn{maven:io.jenkins.plugins: aws-global-configuration}.
% The rationale of unsupervised fine-tuning is to activate their knowledge of each Java library by correlating each Java library's functionality description with its name. 

% After unsupervised fine-tuning, \detector{} conducts supervised fine-tuning on the input dataset, $(\mathcal{V}, \mathcal{L}, \mathcal{M})$ with two steps.
% First, \detector{} invokes another approach of identifying vulnerable libraries to recommend a list of vulnerable library names for input augmentation.
% Note that our rationale for input augmentation is to help identify zero-shot libraries because LLMs have no prior knowledge of how these libraries are affected, so we choose two representative approaches that effectively identify zero-shot libraries.
% Specifically, we choose VulLibMiner and the TF-IDF matcher in VulLibMiner because each of them identifies zero-shot and full-shot (non-zero-shot) libraries with a similar F1 score~\cite{vullibminer} while the TF-IDF matcher, as a NER approach, is less effective than VulLibMiner.
% Second, \detector{} concatenates the description of a given vulnerability with the recommended libraries as the input prompt used for supervised fine-tuning.
% The targeted output in this step is a name list of vulnerable libraries that are affected by this vulnerability.

% Table~\ref{tab: cve-mail} shows an example case of \CodeIn{CVE-2020-2318} in this step.
% The description of this vulnerability mentions the vulnerable functionality, \CodeIn{Jenkins Mail Commander Plugin}, its package source, \CodeIn{Jenkins-ci Plugin 1.0.0}, and how this vulnerability is exploited.
% We also show that the recommended library is another Java library with the same group id and a similar artifact id.
% However, \detector{} rejects this recommended result and outputs the correct vulnerable library, thus indicating its generation capability instead of simply judging whether recommended libraries are correct or not.







% \subsection{Post-Processing of Library Names}





% \begin{algorithm}[t]
% \caption{Post-Processing of Library Names}
% \label{alg: post-processing}
% \begin{algorithmic}[1]
% \Require $rawResponse$, raw text of LLM's Response.
% \Require $libMaven$, Java library names from Maven.
% \Ensure $vulnNames$, a list of vulnerable library names.
% \Function{Post-Processing}{$rawResponse, libMaven$}
%     \State $rawNames \gets rawResponse.findall(\mbox{``maven:\textbackslash 
%  w*:\textbackslash w*''})$
%     \State $artifacts \gets \emptyset{}, groups \gets \{ \}$
%     \For{$mavenName \in libMaven$}
%         \State $\mbox{``maven''}, groupid, artifactid \gets mavenName.split()$
%         \State $artifacts.append(artifactid)$
%         \State $groups[artifactid].append(groupid)$
%     \EndFor
%     \For{$rawName \in rawNames$}
%         \State $\mbox{``maven''}, groupid, artifactid \gets rawName.split()$
%         \State $Levenshtein.weight \gets (W_{insert}, W_{delete}, W_{replace})$
%         \State $artifactid^{\prime} \gets \mathop{argmin}\limits_{id \in artifacts}{Levenshtein(artifactid, id)}$
%         \State $subgroups \gets groups[artifactid^{\prime}]$
%         \State $groupid^{\prime} \gets \mathop{argmin}\limits_{id \in subgroups}{Levenshtein(groupid, id)}$
%         \State $vulnNames \gets \mbox{``maven''}: groupid^{\prime}: artifactid^{\prime}$
%     \EndFor
%     \State \Return{$vulnNames$}
% \EndFunction
% \end{algorithmic}
% \end{algorithm}

% To address \detector{}'s hallucinations, we design our post-processing technique based on the Levenshtein distance~\cite{levenshtein} to obtain existing Java library names from the response of LLMs.
% We find that \detector{} can generate the components of the targeted library names (i.e., the targeted functionalities and scopes), and make mistakes when jointing these components of library names, thus leading to hallucinations.
% Therefore, hallucination library names are close to the targeted names of vulnerable libraries, and their closest library names tend to be the targeted names.



% To address \detector{}'s hallucinations, we design our post-processing algorithm based on the Levenshtein distance~\cite{levenshtein} to obtain correct Java library names from the response of LLMs.
% Our goal is to ensure that the generated library names belong to existing Java libraries.
% One major difficulty for this problem is that Java library names are relatively complex and structural when compared with library names of other programming languages.
% A correct Java library name consists of its group id and artifact id.
% Here we take only libraries collected in Maven into consideration, so we add a prefix identifier, \CodeIn{maven}, before each library name.
% Thus, an example of correct Java library names is \CodeIn{maven:com.google.code.gson:gson}.

% Our post-processing algorithm is designed based on the rationale that hallucinations library names are slightly different from the real names of vulnerable libraries.
% For example, the group id of a Java library consists of multiple components separated by periods (\CodeIn{.}) and some of these components might be neglected or incorrectly replaced.
% Therefore, we use Levenshtein distance to find the correct affected libraries.

% Our technique is shown in Algorithm~\ref{alg: post-processing}.
% It takes the raw-text output of our fine-tuned LLM and outputs a list of vulnerable library names after post-processing.
% This algorithm conducts post-processing through two steps: parsing the raw-text output into a list of library names, and identifying their closest existing library names.

% In Line 2, we parse the raw-text output into a list of library names.
% Here we use a regex expression that contains the identifier ``maven'', group id, and artifact id, to extract library names from our fine-tuned LLM's output, $rawResponse$.

% In Lines 3-16, we identify the closest library names based on the library names extracted in the first step.
% In Lines 3-8, we divide the names of all Java libraries in Maven into multiple groups where library names in each group have the same artifact id.
% In Lines 9-10, for each generated library name, we first split it into its group id and artifact id.
% In Line 12, we use its artifact id, $artifactid$ to find its closest and existing artifact id, $artifactid^{\prime}$.
% Then in Lines 13-14, we use its group id, $groupid$ to find its closest and existing group id, $groupid^{\prime}$ from library names with the same artifact id, $artifactid^{\prime}$.
% Then, we concatenate the ``maven'' identifier with the search results, $groupid^{\prime}$ and $artifactid^{\prime}$ as one post-processed library name.
% Additionally, in Line 11, we manually set the weight used in calculating Levenshtein distances because LLMs change the library names in terms of tokens instead of characters.
% Thus, the weight of inserting one character should be smaller than that of deleting and replacing one, and we set the empirical Levenshtein weights as follows, $W_{insert} = 1, W_{delete} = 4, W_{replace} = 4$.
% \begin{equation}
%     W_{insert} = 1, W_{delete} = 4, W_{replace} = 4
% \end{equation}

% Our empirical statistics show that the average length of tokens in library names is 5.7, and their average number of different characters is 1.7



% \tianyu{group id reflect the sources of library, artifact id reflects its functionalities}

% \CodeIn{maven:com.sdklite:gson}
% Thus, library names generated by LLMs might neglect part of the components or include more components.


% \begin{table}[t]
% \renewcommand\arraystretch{1}
% \centering
% \caption{An Example of Java Library}
% \label{tab: lib-aws}
% \begin{tabular}{p{1.8cm}|p{6cm}}
% \toprule
% Input Prompt              & Below is a Java lib description \\
% \midrule
% \makecell[l]{Library\\ Description} & \makecell[l]{Input: Configure all AWS related plugins from\\ a single page.} \\
% \midrule
% \makecell[l]{Model\\ Response} & \makecell[l]{This package's name is\\ \textit{maven:io.jenkins.plugins:aws-global-configuration}.}\\
% \bottomrule
% \end{tabular}
% \end{table}


% \begin{table}[t]
% \centering
% \caption{An Example of CVE-2020-2318}
% \label{tab: cve-mail}
% \begin{tabular}{p{1.8cm}|p{6cm}}
% \toprule
% Input Prompt              & Below is a Java vulnerability description.   Please identify the software name affected by it \\
% \midrule
% Vulnerability Description & Input: Jenkins Mail Commander Plugin for Jenkins-ci Plugin 1.0.0 and   earlier stores passwords unencrypted in job config.xml files on the Jenkins   controller where they can be viewed by users with Extended Read permission,   or access to the Jenkins controller file system. \\
% \midrule
% \makecell[l]{Recommended\\ Library}       & \makecell[l]{Top 1 search result are \textit{maven:org.jenkins-ci.plugins:job-direct-mail}} \\
% \midrule
% \makecell[l]{Model\\ Response} & \makecell[l]{The affected packages is\\ \textit{maven:org.jenkins-ci.plugins:mail-commander.}}\\
% \midrule
% \makecell[l]{Post-processed\\ Library}    & \makecell[l]{\textit{maven:org.jenkins-ci.plugins:mailcommander}} \\
% \bottomrule
% \end{tabular}
% \end{table}

==> backup/approach-backup-3.tex <==
\begin{figure*}[t]
\centering
\includegraphics[width=1\linewidth]{figures/workflow-new-1.drawio.pdf}
\caption{\detector{} Framework}
\label{fig: framework}
\end{figure*}


\section{Approach}\label{sec:approach}
In this section, we introduce the framework of \detector{} which we illustrate in Figure~\ref{fig: framework}.
Our key insight is to address the scalability problems faced by existing retrieval approaches by utilizing the generation capabilities of Large Language Models (LLMs).


Given the input description of a vulnerability, \detector{} leverages a LLM to generate a package name given the following prompt: "\emph{Below is a [Programming Language] vulnerability description. Please identify the software name affected by it. Input: [DESCRIPTION]. The top k search results are: [$L_1$][$L_2$]$\cdots$[$L_k$]. Please output the package name as the format "ecosystem:library name".
\#\#\# Response: The affected packages:}". To address the challenges in the generation approach, our framework includes the following components: 
(1) \textbf{Before generation}: We leverage retrieval augmented generation (RAG)~\cite{lewis2020retrieval} to reduce the hallucination in the generation results. In particular, we add the top k retrieved package names to the prompt; (2) \textbf{During generation}: since the generated package name may not exist, we leverage constrained decoding~\cite{hokamp2017lexically,anderson2016guided} so the generation result includes the name(s) of at least one existing package(s); 
(3) \textbf{Post generation}: we further match the generation result with the closest package name in the list of existing package names. Below we explain each component in more details. 


\subsection{Before Generation: Retrieval Augmented Generation (RAG)}

Retrieval augmented generation (RAG) is a framework that enhances the performance of a generative model by incorporating knowledge from an external corpus~\cite{lewis2020retrieval,gao2023retrieval}. Given the user input, RAG leverages a retrieval model to obtain the top-$k$ most similar paragraphs/documents, and combine them in the input for the generation~\cite{gao2023retrieval}. RAG can solve the problem of hallucination when the generative model lacks knowledge of the corpus. Since our initial study (Section~\ref{sec: empirical_study}) shows that hallucination also exists in our raw generation results. we employ RAG in VulLibGen. 

\noindent \textbf{Retriever setting}. Given the description of a vulnerability, our retriever ranks all the unique package names (Table~\ref{tab: dataset info}) based on their similarity $sim(d_v, d_p)$ with the description, where $d_v$ and $d_p$ are the descriptions of the vulnerability $v$ and package name $p$. The descriptions for packages in Java and Python are obtained from the Maven~\footnote{https://mvnrepository.com} and Pypi~\footnote{https://pypi.org} documentations while for JavaScript and Go are from NPM~\footnote{https://www.npmjs.com} and Go~\footnote{https://pkg.go.dev}.
For example, the description of the package ``org.jenkins -ci.plugins:mailcommander'' is \textit{``This plug-in provides function that read a mail subject as a CLI Command.''}.
We use two models for the similarity function: TF-IDF, and a BERT-base model fine-tuned on GitHub Advisory.


\subsection{During Generation: Constrained Decoding}

We design our constrained decoding algorithm to restrict the open-source LLMs to include the name of at least one existing package.
This constraint is written as follows:

\begin{equation*}
    \exists l \in \mathcal{L}, \mbox{ s.t. } l \in \mathcal{F}_{generation} (v)
\end{equation*}

However, adopting constrained decoding has two technical challenges to address.
First, each package name contains more than one token (e.g., Python packages have 6 tokens on average) while LLMs generate only one token at once.
Therefore, we cannot greedily check whether the constraints are satisfied during decoding.
To address this challenge, we construct a Trie tree to represent the constraints (as shown in Figure~\ref{fig: framework}) and then conduct beam search~\cite{kumar2013beam} to ensure that the output contains at least one path (corresponding to an existing package name) on this Trie tree.

Second, the large number of packages in each ecosystem (e.g., 435,642 in Maven and 506,848 in Pypi) brings a heavy efficiency burden as the Trie tree for constrained decoding might have more than 1,000,000 nodes. 
We empirically notice that invoking an LLM with 7B parameters might cost more than 2 hours, which is unacceptable.
To address this challenge, we relax the ``hard'' constraints to ``soft'' ones.

Our implementation of ``soft'' constraints consists of two steps.
(1) We replace the entire Trie tree with a bi-gram Trie tree with only two depth of nodes.
For example, if a package name consists of three tokens \CodeIn{[``org'', ``google'', ``gson'']}, we add two edges in this bi-gram Trie tree, \CodeIn{``org''} $\rightarrow$ \CodeIn{``google''} and \CodeIn{``google''} $\rightarrow$ \CodeIn{``gson''}.
The bi-gram Trie tree can remove a large portion (more than 50\%) of leaf nodes in the Trie tree, thus substantially speeding up beam searching during decoding.
(2) We add another term of probability $\log p_{trie} (w_{i+1}|w_{i})$ to ensure that the output is quite similar to an existing package name.
Specifically, when decoding the i+1 th token $w_{i+1}$, each token's probability $p(w_{i+1}|w_{0:i})$ is defined as follows:
\begin{equation*}
    \begin{aligned}
        \log p(w_{i+1}|w_{0:i}) \propto &\lambda_{LLM} \log p_{LLM}(w_{i+1}|w_{0:i})\\
        + &\lambda_{cons} \log p_{trie} (w_{i+1}|w_{i})\\
        p_{trie}(w_{i+1}|w_{i}) \propto &\ \sum_{l \in \mathcal{L}, j} l[j,j+1] = w[i,i+1]
    \end{aligned}
\end{equation*}
where $\lambda_{LLM}$ and $\lambda_{cons}$ are two hyper-parameters that determine the respective contribution of an LLM and our constraints. 

\tianyu{is it necessary to mention trie tree with top512 results?}

% To address this challenge, we follow the similar idea of VulLibMiner, using a TF-IDF~\cite{jones1972statistical, jones2004idf} technique to filter a small candidate of packages.
% Its empirical results indicate that 512 is a proper candidate size with a recall of at least 0.9.
% Thus, the decoding constraint is modified as:

% \begin{equation*}
% \begin{aligned}
%     &\mathcal{L}(v) = \mathop{\mbox{Top512}}\limits_{l_i \in \mathcal{L}}\ TF\mathit{-}IDF(v, l_i) \\
%     &\exists l \in \mathcal{L}(v), \mbox{ s.t. } l \in \mathcal{F}_{generation} (v)
% \end{aligned}
% \end{equation*}

% However, this resolution

\subsection{Post Generation: Local Search}
We design our local search algorithm to find the closest package name from the output of LLMs.
The input of this algorithm includes one package name generated by LLM together with the name list of existing libraries under the same ecosystem.
The output of this algorithm is the name of one existing package that is the closest to the generated package name.

This technique can help address the former three types of incorrect responses based on the observation in Table~\ref{tab: fault case study} that the generated name has already specified the targeted library (i.e., most components of this generated name are correct) with only slight differences.
Therefore, we use the Levenshtein distance to find the closest and existing package name as the output of this algorithm.
The details of this algorithm are listed in the Appendix.

Additionally, we conduct a two-staged local search when given a Java vulnerability because the names of Java packages are relatively complex and structural compared to package names of other programming languages. 
A Java package name consists of its group ID and artifact ID.
In this scenario, we first search for an existing artifact ID and then search for an existing group ID corresponding to this artifact ID.
Our rationale is that the artifact IDs include each package's functionalities, which is easier to identify from a vulnerability's description.





% Unlike conventional information retrieval (IR)/classification approaches, \detector{} utilizes the tremendous capabilities of Large Language Models (LLMs) in comprehending vulnerability descriptions.
% Our key insight is that conventional approaches highly depend on their training set and thus face the scalability problem and this problem can be alleviated by modeling this task as a generation task.

% As formalized in Section~\ref{sec: formal}, the training input of \detector{} includes the textual descriptions of vulnerabilities, $\mathcal{V}$, the textual descriptions of all Java libraries in Maven, $\mathcal{L}$, and the mapping relationship from vulnerabilities to libraries, $\mathcal{M}$.
% When applied in practice, \detector{} takes only the textual descriptions of one vulnerability as input and outputs a series of names of libraries affected by this vulnerability.


% \begin{figure}[t]
% \centering
% \includegraphics[width=1\linewidth]{figures/approach-illustration.drawio.pdf}
% \caption{An Illustration of the Motivation of our RAG and Constrained Decoding/Local Search Techniques}
% \label{fig: case}
% \end{figure}

% \subsection{Fine-tuning and Prompt-tuning}




% LLMs can correlate the input vulnerability description to vulnerable libraries based on their prior knowledge of these libraries, e.g., their functionalities, usages, and even history issues.

% As formalized in Section~\ref{sec: formal}, the training input of \detector{} includes the textual descriptions of vulnerabilities, $\mathcal{V}$, the textual descriptions of all Java libraries in Maven, $\mathcal{L}$, and the mapping relationship from vulnerabilities to libraries, $\mathcal{M}$.
% When applied in practice, \detector{} takes only the textual descriptions of one vulnerability as input and outputs a series of names of libraries affected by this vulnerability.


% The process of \detector{} is shown in Figure~\ref{fig: framework} with two steps.
% First, we conduct unsupervised fine-tuning on Maven Corpus, which includes all Java libraries and their descriptions.
% This step aims at activating their knowledge of each Java library, including its name and functionalities.
% Second, we conduct supervised fine-tuning on the input dataset $(\mathcal{V}, \mathcal{L}, \mathcal{M})$ to learn the mapping relationship from vulnerabilities to libraries.



% During supervised fine-tuning, we design two specific techniques to improve the effectiveness of \detector{}.
% To help identify zero-shot libraries, we design an input augmentation technique, which feeds the names of vulnerable libraries (a.k.a., recommended libraries) identified by the SOTA approach~\cite{vullibminer} to \detector{} as input.
% This technique provides examples of libraries whose functionalities are likely to be affected by a given vulnerability.
% Thus, \detector{} can generate library names from those with similar functionalities instead of all libraries when \detector{} has no prior knowledge of how these zero-shot libraries are affected by vulnerabilities.
% To address \detector{}'s hallucinations, we design our post-processing technique based on the Levenshtein distance~\cite{levenshtein} to obtain existing Java library names from the response of LLMs.
% We find that \detector{} can generate the components of the targeted library names (i.e., the targeted functionalities and scopes), and make mistakes when jointing these components of library names, thus leading to hallucinations.
% Therefore, hallucination library names are close to the targeted names of vulnerable libraries, and their closest library names tend to be the targeted names.


% \subsection{Two Stages of Fine-Tuning with Input Augmentation}
% \detector{} mainly consists of two stages of fine-tuning on LLMs.
% In this paper, we choose one of the state-of-the-art (SOTA) open-source LLMs, LLaMa~\cite{llama}, as our base LLM with 7B and 13B parameters.

% During unsupervised fine-tuning, \detector{} takes the input of one library description, and its targeted output is its library name.
% Table~\ref{tab: lib-aws} shows an example case in this step.
% Its input describes the functionality of this package, e.g., configuration on AWS plugins, and its output is a structural Java library name, \CodeIn{maven:io.jenkins.plugins: aws-global-configuration}.
% The rationale of unsupervised fine-tuning is to activate their knowledge of each Java library by correlating each Java library's functionality description with its name. 

% After unsupervised fine-tuning, \detector{} conducts supervised fine-tuning on the input dataset, $(\mathcal{V}, \mathcal{L}, \mathcal{M})$ with two steps.
% First, \detector{} invokes another approach of identifying vulnerable libraries to recommend a list of vulnerable library names for input augmentation.
% Note that our rationale for input augmentation is to help identify zero-shot libraries because LLMs have no prior knowledge of how these libraries are affected, so we choose two representative approaches that effectively identify zero-shot libraries.
% Specifically, we choose VulLibMiner and the TF-IDF matcher in VulLibMiner because each of them identifies zero-shot and full-shot (non-zero-shot) libraries with a similar F1 score~\cite{vullibminer} while the TF-IDF matcher, as a NER approach, is less effective than VulLibMiner.
% Second, \detector{} concatenates the description of a given vulnerability with the recommended libraries as the input prompt used for supervised fine-tuning.
% The targeted output in this step is a name list of vulnerable libraries that are affected by this vulnerability.

% Table~\ref{tab: cve-mail} shows an example case of \CodeIn{CVE-2020-2318} in this step.
% The description of this vulnerability mentions the vulnerable functionality, \CodeIn{Jenkins Mail Commander Plugin}, its package source, \CodeIn{Jenkins-ci Plugin 1.0.0}, and how this vulnerability is exploited.
% We also show that the recommended library is another Java library with the same group id and a similar artifact id.
% However, \detector{} rejects this recommended result and outputs the correct vulnerable library, thus indicating its generation capability instead of simply judging whether recommended libraries are correct or not.







% \subsection{Post-Processing of Library Names}





% \begin{algorithm}[t]
% \caption{Post-Processing of Library Names}
% \label{alg: post-processing}
% \begin{algorithmic}[1]
% \Require $rawResponse$, raw text of LLM's Response.
% \Require $libMaven$, Java library names from Maven.
% \Ensure $vulnNames$, a list of vulnerable library names.
% \Function{Post-Processing}{$rawResponse, libMaven$}
%     \State $rawNames \gets rawResponse.findall(\mbox{``maven:\textbackslash 
%  w*:\textbackslash w*''})$
%     \State $artifacts \gets \emptyset{}, groups \gets \{ \}$
%     \For{$mavenName \in libMaven$}
%         \State $\mbox{``maven''}, groupid, artifactid \gets mavenName.split()$
%         \State $artifacts.append(artifactid)$
%         \State $groups[artifactid].append(groupid)$
%     \EndFor
%     \For{$rawName \in rawNames$}
%         \State $\mbox{``maven''}, groupid, artifactid \gets rawName.split()$
%         \State $Levenshtein.weight \gets (W_{insert}, W_{delete}, W_{replace})$
%         \State $artifactid^{\prime} \gets \mathop{argmin}\limits_{id \in artifacts}{Levenshtein(artifactid, id)}$
%         \State $subgroups \gets groups[artifactid^{\prime}]$
%         \State $groupid^{\prime} \gets \mathop{argmin}\limits_{id \in subgroups}{Levenshtein(groupid, id)}$
%         \State $vulnNames \gets \mbox{``maven''}: groupid^{\prime}: artifactid^{\prime}$
%     \EndFor
%     \State \Return{$vulnNames$}
% \EndFunction
% \end{algorithmic}
% \end{algorithm}

% To address \detector{}'s hallucinations, we design our post-processing technique based on the Levenshtein distance~\cite{levenshtein} to obtain existing Java library names from the response of LLMs.
% We find that \detector{} can generate the components of the targeted library names (i.e., the targeted functionalities and scopes), and make mistakes when jointing these components of library names, thus leading to hallucinations.
% Therefore, hallucination library names are close to the targeted names of vulnerable libraries, and their closest library names tend to be the targeted names.



% To address \detector{}'s hallucinations, we design our post-processing algorithm based on the Levenshtein distance~\cite{levenshtein} to obtain correct Java library names from the response of LLMs.
% Our goal is to ensure that the generated library names belong to existing Java libraries.
% One major difficulty for this problem is that Java library names are relatively complex and structural when compared with library names of other programming languages.
% A correct Java library name consists of its group id and artifact id.
% Here we take only libraries collected in Maven into consideration, so we add a prefix identifier, \CodeIn{maven}, before each library name.
% Thus, an example of correct Java library names is \CodeIn{maven:com.google.code.gson:gson}.

% Our post-processing algorithm is designed based on the rationale that hallucinations library names are slightly different from the real names of vulnerable libraries.
% For example, the group id of a Java library consists of multiple components separated by periods (\CodeIn{.}) and some of these components might be neglected or incorrectly replaced.
% Therefore, we use Levenshtein distance to find the correct affected libraries.

% Our technique is shown in Algorithm~\ref{alg: post-processing}.
% It takes the raw-text output of our fine-tuned LLM and outputs a list of vulnerable library names after post-processing.
% This algorithm conducts post-processing through two steps: parsing the raw-text output into a list of library names, and identifying their closest existing library names.

% In Line 2, we parse the raw-text output into a list of library names.
% Here we use a regex expression that contains the identifier ``maven'', group id, and artifact id, to extract library names from our fine-tuned LLM's output, $rawResponse$.

% In Lines 3-16, we identify the closest library names based on the library names extracted in the first step.
% In Lines 3-8, we divide the names of all Java libraries in Maven into multiple groups where library names in each group have the same artifact id.
% In Lines 9-10, for each generated library name, we first split it into its group id and artifact id.
% In Line 12, we use its artifact id, $artifactid$ to find its closest and existing artifact id, $artifactid^{\prime}$.
% Then in Lines 13-14, we use its group id, $groupid$ to find its closest and existing group id, $groupid^{\prime}$ from library names with the same artifact id, $artifactid^{\prime}$.
% Then, we concatenate the ``maven'' identifier with the search results, $groupid^{\prime}$ and $artifactid^{\prime}$ as one post-processed library name.
% Additionally, in Line 11, we manually set the weight used in calculating Levenshtein distances because LLMs change the library names in terms of tokens instead of characters.
% Thus, the weight of inserting one character should be smaller than that of deleting and replacing one, and we set the empirical Levenshtein weights as follows, $W_{insert} = 1, W_{delete} = 4, W_{replace} = 4$.
% \begin{equation}
%     W_{insert} = 1, W_{delete} = 4, W_{replace} = 4
% \end{equation}

% Our empirical statistics show that the average length of tokens in library names is 5.7, and their average number of different characters is 1.7



% \tianyu{group id reflect the sources of library, artifact id reflects its functionalities}

% \CodeIn{maven:com.sdklite:gson}
% Thus, library names generated by LLMs might neglect part of the components or include more components.


% \begin{table}[t]
% \renewcommand\arraystretch{1}
% \centering
% \caption{An Example of Java Library}
% \label{tab: lib-aws}
% \begin{tabular}{p{1.8cm}|p{6cm}}
% \toprule
% Input Prompt              & Below is a Java lib description \\
% \midrule
% \makecell[l]{Library\\ Description} & \makecell[l]{Input: Configure all AWS related plugins from\\ a single page.} \\
% \midrule
% \makecell[l]{Model\\ Response} & \makecell[l]{This package's name is\\ \textit{maven:io.jenkins.plugins:aws-global-configuration}.}\\
% \bottomrule
% \end{tabular}
% \end{table}


% \begin{table}[t]
% \centering
% \caption{An Example of CVE-2020-2318}
% \label{tab: cve-mail}
% \begin{tabular}{p{1.8cm}|p{6cm}}
% \toprule
% Input Prompt              & Below is a Java vulnerability description.   Please identify the software name affected by it \\
% \midrule
% Vulnerability Description & Input: Jenkins Mail Commander Plugin for Jenkins-ci Plugin 1.0.0 and   earlier stores passwords unencrypted in job config.xml files on the Jenkins   controller where they can be viewed by users with Extended Read permission,   or access to the Jenkins controller file system. \\
% \midrule
% \makecell[l]{Recommended\\ Library}       & \makecell[l]{Top 1 search result are \textit{maven:org.jenkins-ci.plugins:job-direct-mail}} \\
% \midrule
% \makecell[l]{Model\\ Response} & \makecell[l]{The affected packages is\\ \textit{maven:org.jenkins-ci.plugins:mail-commander.}}\\
% \midrule
% \makecell[l]{Post-processed\\ Library}    & \makecell[l]{\textit{maven:org.jenkins-ci.plugins:mailcommander}} \\
% \bottomrule
% \end{tabular}
% \end{table}

==> backup/approach_backup.tex <==
\begin{figure*}[t]
\centering
\includegraphics[width=1\linewidth]{figures/workflow.drawio.pdf}
\caption{Workflow of \detector{}}
\label{fig: framework}
\end{figure*}


\section{Approach}\label{sec:approach}
In this section, we propose \detector{}, the first approach to generate the names of vulnerable third-party libraries.
Our key insight is to address the scalability problems faced by existing IR/classification approaches by utilizing the generation capabilities of Large Language Models (LLMs) after comprehending vulnerability descriptions.


The process of \detector{} is shown in Figure~\ref{fig: framework} with three steps.
(1) We design a retrieval augmented generation (RAG) technique that provides domain knowledge into the input of LLMs.
In this step, we feed the names of affected libraries generated by IR approaches as our recommended packages to the inputs of \detector{}.
Our rationale is that these recommended packages might be close to the targeted packages, thus helping LLMs capture the correct keywords in the vulnerability descriptions.
(2) We invoke one LLM to generate the names of affected packages.
Specifically, we considered three categories of LLMs: commercial LLMs, such as ChatGPT/GPT4, fine-tuned open-source LLMs, such as LLaMa/Vicuna, and base LLMs with prompting-tuning.
(3) We design a local search algorithm and a constrained decoding algorithm to avoid non-existing package names.
The constrained decoding algorithm is more effective and can be only applied to open-source LLMs while the local search algorithm is non-intrinsic and can be applied to the results of commercial LLMs.
Our rationale is to utilize the name list of existing libraries to restrict the outputs of LLMs into existing package names, thus avoiding non-existing package names.


\subsection{Retrieval Augmented Generation}
Our RAG technique feeds the recommended names of affected packages to the inputs of \detector{} by invoking one SOTA IR approach, VulLibMiner~\cite{vullibminer}.
VulLibMiner uses two techniques to calculate the similarity between a given vulnerability and package, a TF-IDF matcher and a fine-tuned BERT model.
It retrieves the most related package with a given vulnerability based on the vulnerability description and each package's description in its corresponding ecosystem, e.g., Maven or Pypi.
For example, in Figure~\ref{fig: framework}, the input prompt with RAG consists of both the vulnerability description and the names of Top k search results (packages).

This technique can help address the latter two types of incorrect responses as it provides a list of candidate packages for LLMs. 
Compared with directly generating the affected packages, our RAG technique provides an easier option for LLMs to determine whether these candidate packages are correct or not and choose a proper one from them.
Additionally, LLMs can modify the retrieved results to proper ones based on the vulnerability descriptions.
% Even though LLMs face difficulty in comprehending the given 


\subsection{Local Search}
We design our local search algorithm to find the closest package name from the output of LLMs.
The input of this algorithm includes one package name generated by LLM together with the name list of existing libraries under the same ecosystem.
The output of this algorithm is the name of one existing package that is the closest to the generated package name.

This technique can help address the former three types of incorrect responses based on the observation in Table~\ref{tab: fault case study} that the generated name has already specified the targeted library (i.e., most components of this generated name are correct) with only slight differences.
Therefore, we use the Levenshtein distance to find the closest and existing package name as the output of this algorithm.
The details of this algorithm in listed in the Appendix.

Additionally, we conduct a two-staged local search when given a Java vulnerability because the names of Java packages are relatively complex and structural compared to package names of other programming languages. 
A Java package name consists of its group ID and artifact ID.
In this scenario, we first search for an existing artifact ID and then search for an existing group ID corresponding to this artifact ID.
Our rationale is that the artifact IDs include each package's functionalities, which is easier to identify from a vulnerability's description.

\subsection{Constrained Decoding}
We design our constrained decoding algorithm to restrict the open-source LLMs to include the name of at least one existing package.
This constraint is written as follows:

\begin{equation*}
    \exists l \in \mathcal{L}, \mbox{ s.t. } l \in \mathcal{F}_{generation} (v)
\end{equation*}

However, adopting constrained decoding has two technical challenges to address.
First, each package name contains more than one token (e.g., Python packages have 6 tokens on average) while LLMs generate only one token at once.
Therefore, we cannot greedily check whether the constraints are satisfied during decoding.
To address this challenge, we construct a Trie tree to represent the constraints (as shown in Figure~\ref{fig: framework}) and then conduct beam search~\cite{kumar2013beam} to ensure that the output contains at least one path (corresponding to an existing package name) on this Trie tree.

Second, the large number of packages in each ecosystem (e.g., 435,642 in Maven and 506,848 in Pypi) brings a heavy efficiency burden as the Trie tree for constrained decoding might have more than 1,000,000 nodes. 
We empirically notice that invoking an LLM with 7B parameters might cost more than 2 hours, which is unacceptable.
To address this challenge, we follow the similar idea of VulLibMiner, using a TF-IDF~\cite{jones1972statistical, jones2004idf} technique to filter a small candidate of packages.
Its empirical results indicate that 512 is a proper candidate size with a recall of at least 0.9.
Thus, the decoding constraint is modified as:

\begin{equation*}
\begin{aligned}
    &\mathcal{L}(v) = \mathop{\mbox{Top512}}\limits_{l_i \in \mathcal{L}}\ TF\mathit{-}IDF(v, l_i) \\
    &\exists l \in \mathcal{L}(v), \mbox{ s.t. } l \in \mathcal{F}_{generation} (v)
\end{aligned}
\end{equation*}



% Unlike conventional information retrieval (IR)/classification approaches, \detector{} utilizes the tremendous capabilities of Large Language Models (LLMs) in comprehending vulnerability descriptions.
% Our key insight is that conventional approaches highly depend on their training set and thus face the scalability problem and this problem can be alleviated by modeling this task as a generation task.

% As formalized in Section~\ref{sec: formal}, the training input of \detector{} includes the textual descriptions of vulnerabilities, $\mathcal{V}$, the textual descriptions of all Java libraries in Maven, $\mathcal{L}$, and the mapping relationship from vulnerabilities to libraries, $\mathcal{M}$.
% When applied in practice, \detector{} takes only the textual descriptions of one vulnerability as input and outputs a series of names of libraries affected by this vulnerability.


% \begin{figure}[t]
% \centering
% \includegraphics[width=1\linewidth]{figures/approach-illustration.drawio.pdf}
% \caption{An Illustration of the Motivation of our RAG and Constrained Decoding/Local Search Techniques}
% \label{fig: case}
% \end{figure}

% \subsection{Fine-tuning and Prompt-tuning}




% LLMs can correlate the input vulnerability description to vulnerable libraries based on their prior knowledge of these libraries, e.g., their functionalities, usages, and even history issues.

% As formalized in Section~\ref{sec: formal}, the training input of \detector{} includes the textual descriptions of vulnerabilities, $\mathcal{V}$, the textual descriptions of all Java libraries in Maven, $\mathcal{L}$, and the mapping relationship from vulnerabilities to libraries, $\mathcal{M}$.
% When applied in practice, \detector{} takes only the textual descriptions of one vulnerability as input and outputs a series of names of libraries affected by this vulnerability.


% The process of \detector{} is shown in Figure~\ref{fig: framework} with two steps.
% First, we conduct unsupervised fine-tuning on Maven Corpus, which includes all Java libraries and their descriptions.
% This step aims at activating their knowledge of each Java library, including its name and functionalities.
% Second, we conduct supervised fine-tuning on the input dataset $(\mathcal{V}, \mathcal{L}, \mathcal{M})$ to learn the mapping relationship from vulnerabilities to libraries.



% During supervised fine-tuning, we design two specific techniques to improve the effectiveness of \detector{}.
% To help identify zero-shot libraries, we design an input augmentation technique, which feeds the names of vulnerable libraries (a.k.a., recommended libraries) identified by the SOTA approach~\cite{vullibminer} to \detector{} as input.
% This technique provides examples of libraries whose functionalities are likely to be affected by a given vulnerability.
% Thus, \detector{} can generate library names from those with similar functionalities instead of all libraries when \detector{} has no prior knowledge of how these zero-shot libraries are affected by vulnerabilities.
% To address \detector{}'s hallucinations, we design our post-processing technique based on the Levenshtein distance~\cite{levenshtein} to obtain existing Java library names from the response of LLMs.
% We find that \detector{} can generate the components of the targeted library names (i.e., the targeted functionalities and scopes), and make mistakes when jointing these components of library names, thus leading to hallucinations.
% Therefore, hallucination library names are close to the targeted names of vulnerable libraries, and their closest library names tend to be the targeted names.


% \subsection{Two Stages of Fine-Tuning with Input Augmentation}
% \detector{} mainly consists of two stages of fine-tuning on LLMs.
% In this paper, we choose one of the state-of-the-art (SOTA) open-source LLMs, LLaMa~\cite{llama}, as our base LLM with 7B and 13B parameters.

% During unsupervised fine-tuning, \detector{} takes the input of one library description, and its targeted output is its library name.
% Table~\ref{tab: lib-aws} shows an example case in this step.
% Its input describes the functionality of this package, e.g., configuration on AWS plugins, and its output is a structural Java library name, \CodeIn{maven:io.jenkins.plugins: aws-global-configuration}.
% The rationale of unsupervised fine-tuning is to activate their knowledge of each Java library by correlating each Java library's functionality description with its name. 

% After unsupervised fine-tuning, \detector{} conducts supervised fine-tuning on the input dataset, $(\mathcal{V}, \mathcal{L}, \mathcal{M})$ with two steps.
% First, \detector{} invokes another approach of identifying vulnerable libraries to recommend a list of vulnerable library names for input augmentation.
% Note that our rationale for input augmentation is to help identify zero-shot libraries because LLMs have no prior knowledge of how these libraries are affected, so we choose two representative approaches that effectively identify zero-shot libraries.
% Specifically, we choose VulLibMiner and the TF-IDF matcher in VulLibMiner because each of them identifies zero-shot and full-shot (non-zero-shot) libraries with a similar F1 score~\cite{vullibminer} while the TF-IDF matcher, as a NER approach, is less effective than VulLibMiner.
% Second, \detector{} concatenates the description of a given vulnerability with the recommended libraries as the input prompt used for supervised fine-tuning.
% The targeted output in this step is a name list of vulnerable libraries that are affected by this vulnerability.

% Table~\ref{tab: cve-mail} shows an example case of \CodeIn{CVE-2020-2318} in this step.
% The description of this vulnerability mentions the vulnerable functionality, \CodeIn{Jenkins Mail Commander Plugin}, its package source, \CodeIn{Jenkins-ci Plugin 1.0.0}, and how this vulnerability is exploited.
% We also show that the recommended library is another Java library with the same group id and a similar artifact id.
% However, \detector{} rejects this recommended result and outputs the correct vulnerable library, thus indicating its generation capability instead of simply judging whether recommended libraries are correct or not.







% \subsection{Post-Processing of Library Names}





% \begin{algorithm}[t]
% \caption{Post-Processing of Library Names}
% \label{alg: post-processing}
% \begin{algorithmic}[1]
% \Require $rawResponse$, raw text of LLM's Response.
% \Require $libMaven$, Java library names from Maven.
% \Ensure $vulnNames$, a list of vulnerable library names.
% \Function{Post-Processing}{$rawResponse, libMaven$}
%     \State $rawNames \gets rawResponse.findall(\mbox{``maven:\textbackslash 
%  w*:\textbackslash w*''})$
%     \State $artifacts \gets \emptyset{}, groups \gets \{ \}$
%     \For{$mavenName \in libMaven$}
%         \State $\mbox{``maven''}, groupid, artifactid \gets mavenName.split()$
%         \State $artifacts.append(artifactid)$
%         \State $groups[artifactid].append(groupid)$
%     \EndFor
%     \For{$rawName \in rawNames$}
%         \State $\mbox{``maven''}, groupid, artifactid \gets rawName.split()$
%         \State $Levenshtein.weight \gets (W_{insert}, W_{delete}, W_{replace})$
%         \State $artifactid^{\prime} \gets \mathop{argmin}\limits_{id \in artifacts}{Levenshtein(artifactid, id)}$
%         \State $subgroups \gets groups[artifactid^{\prime}]$
%         \State $groupid^{\prime} \gets \mathop{argmin}\limits_{id \in subgroups}{Levenshtein(groupid, id)}$
%         \State $vulnNames \gets \mbox{``maven''}: groupid^{\prime}: artifactid^{\prime}$
%     \EndFor
%     \State \Return{$vulnNames$}
% \EndFunction
% \end{algorithmic}
% \end{algorithm}

% To address \detector{}'s hallucinations, we design our post-processing technique based on the Levenshtein distance~\cite{levenshtein} to obtain existing Java library names from the response of LLMs.
% We find that \detector{} can generate the components of the targeted library names (i.e., the targeted functionalities and scopes), and make mistakes when jointing these components of library names, thus leading to hallucinations.
% Therefore, hallucination library names are close to the targeted names of vulnerable libraries, and their closest library names tend to be the targeted names.



% To address \detector{}'s hallucinations, we design our post-processing algorithm based on the Levenshtein distance~\cite{levenshtein} to obtain correct Java library names from the response of LLMs.
% Our goal is to ensure that the generated library names belong to existing Java libraries.
% One major difficulty for this problem is that Java library names are relatively complex and structural when compared with library names of other programming languages.
% A correct Java library name consists of its group id and artifact id.
% Here we take only libraries collected in Maven into consideration, so we add a prefix identifier, \CodeIn{maven}, before each library name.
% Thus, an example of correct Java library names is \CodeIn{maven:com.google.code.gson:gson}.

% Our post-processing algorithm is designed based on the rationale that hallucinations library names are slightly different from the real names of vulnerable libraries.
% For example, the group id of a Java library consists of multiple components separated by periods (\CodeIn{.}) and some of these components might be neglected or incorrectly replaced.
% Therefore, we use Levenshtein distance to find the correct affected libraries.

% Our technique is shown in Algorithm~\ref{alg: post-processing}.
% It takes the raw-text output of our fine-tuned LLM and outputs a list of vulnerable library names after post-processing.
% This algorithm conducts post-processing through two steps: parsing the raw-text output into a list of library names, and identifying their closest existing library names.

% In Line 2, we parse the raw-text output into a list of library names.
% Here we use a regex expression that contains the identifier ``maven'', group id, and artifact id, to extract library names from our fine-tuned LLM's output, $rawResponse$.

% In Lines 3-16, we identify the closest library names based on the library names extracted in the first step.
% In Lines 3-8, we divide the names of all Java libraries in Maven into multiple groups where library names in each group have the same artifact id.
% In Lines 9-10, for each generated library name, we first split it into its group id and artifact id.
% In Line 12, we use its artifact id, $artifactid$ to find its closest and existing artifact id, $artifactid^{\prime}$.
% Then in Lines 13-14, we use its group id, $groupid$ to find its closest and existing group id, $groupid^{\prime}$ from library names with the same artifact id, $artifactid^{\prime}$.
% Then, we concatenate the ``maven'' identifier with the search results, $groupid^{\prime}$ and $artifactid^{\prime}$ as one post-processed library name.
% Additionally, in Line 11, we manually set the weight used in calculating Levenshtein distances because LLMs change the library names in terms of tokens instead of characters.
% Thus, the weight of inserting one character should be smaller than that of deleting and replacing one, and we set the empirical Levenshtein weights as follows, $W_{insert} = 1, W_{delete} = 4, W_{replace} = 4$.
% \begin{equation}
%     W_{insert} = 1, W_{delete} = 4, W_{replace} = 4
% \end{equation}

% Our empirical statistics show that the average length of tokens in library names is 5.7, and their average number of different characters is 1.7



% \tianyu{group id reflect the sources of library, artifact id reflects its functionalities}

% \CodeIn{maven:com.sdklite:gson}
% Thus, library names generated by LLMs might neglect part of the components or include more components.


% \begin{table}[t]
% \renewcommand\arraystretch{1}
% \centering
% \caption{An Example of Java Library}
% \label{tab: lib-aws}
% \begin{tabular}{p{1.8cm}|p{6cm}}
% \toprule
% Input Prompt              & Below is a Java lib description \\
% \midrule
% \makecell[l]{Library\\ Description} & \makecell[l]{Input: Configure all AWS related plugins from\\ a single page.} \\
% \midrule
% \makecell[l]{Model\\ Response} & \makecell[l]{This package's name is\\ \textit{maven:io.jenkins.plugins:aws-global-configuration}.}\\
% \bottomrule
% \end{tabular}
% \end{table}


% \begin{table}[t]
% \centering
% \caption{An Example of CVE-2020-2318}
% \label{tab: cve-mail}
% \begin{tabular}{p{1.8cm}|p{6cm}}
% \toprule
% Input Prompt              & Below is a Java vulnerability description.   Please identify the software name affected by it \\
% \midrule
% Vulnerability Description & Input: Jenkins Mail Commander Plugin for Jenkins-ci Plugin 1.0.0 and   earlier stores passwords unencrypted in job config.xml files on the Jenkins   controller where they can be viewed by users with Extended Read permission,   or access to the Jenkins controller file system. \\
% \midrule
% \makecell[l]{Recommended\\ Library}       & \makecell[l]{Top 1 search result are \textit{maven:org.jenkins-ci.plugins:job-direct-mail}} \\
% \midrule
% \makecell[l]{Model\\ Response} & \makecell[l]{The affected packages is\\ \textit{maven:org.jenkins-ci.plugins:mail-commander.}}\\
% \midrule
% \makecell[l]{Post-processed\\ Library}    & \makecell[l]{\textit{maven:org.jenkins-ci.plugins:mailcommander}} \\
% \bottomrule
% \end{tabular}
% \end{table}

==> backup/background-backup.tex <==
\section{Background}\label{sec:background}
In this section, we first formalize the task of identifying vulnerable libraries and introduce the scalability limitation of existing IR/classification approaches.
To address the scalability limitation, we model this task as a generation task and then investigate the challenges of generating the names of affected packages.


\begin{table*}[t]
    \centering
    \caption{The Classified Reasons for ChatGPT's Incorrect Response in Maven}
    \label{tab: fault case study}
\scriptsize
\begin{tabular}{lclll}
\toprule
\textbf{Fault Reason}                         & Number                    & Example                             & ChatGPT's Output                                                   & Ground Truth (Affected Packages)                                                         \\
\midrule
\textbf{Mixed Artifact ID}                    & 21                        & CVE-2019-1010250                    & org.onosproject:onos-core                                    & org.onosproject:onos-rest                                      \\
\multicolumn{5}{l}{Mistake a widely used token in artifact ids "-core" as the targeted artifact id}                                                                                                                                                                                \\
\midrule
\textbf{Mixed Group ID}                       & 15                        & CVE-2020-2167                       & org.jenkins-ci.plugins:openshift-pipeline                    & com.openshift.jenkins:openshift-pipeline                       \\
\multicolumn{5}{l}{Mistake a widely used group id "org.jenkins-ci.plugins" as the targeted group id}                                                                                                                                                                      \\
\midrule
\textbf{More/Fewer Tokens}                      & 28                        & CVE-2015-1830                       & org.apache.activemq:activemq                                 & org.apache.activemq:activemq-client                            \\
\multicolumn{5}{l}{ChatGPT's output lacks the token "client"}                                                                                                                                                                                      \\
\midrule
\textbf{Misleaded Name}                       & 23                        & CVE-2020-11974                      & mysql:mysql-connector-java                                   & org.apache.dolphinscheduler:dolphinscheduler                   \\
\multicolumn{5}{l}{The Description is "In DolphinScheduler 1.2.0 and 1.2.1, with mysql connector …...", and ChatGPT incorrectly captures mysql}                          \\
\midrule
\textbf{No Structural Output}                            & 13                        & CVE-2019-13234                      & -                                                                  & org.opencms:opencms-core                                       \\
\multicolumn{5}{l}{ChatGPT only repeats the unstructured result: "Alkacon OpenCms Apollo Template version 10.5.4 and 10.5.5".}  \\
\bottomrule
\end{tabular}
\end{table*}



\subsection{Task Formalization}~\label{sec: formal}
\noindent \textbf{Target:}
The target of this task is to find an ideal correlation $\mathcal{F}: \mathcal{V} \rightarrow \mathcal{L}$ where $\mathcal{V}$ is the set of all vulnerabilities, and $\mathcal{L}$ is the set of all packages.
The mapping results are defined as subsets of $\mathcal{L}$ as one vulnerability can affect more than one package: $\forall v \in \mathcal{V}, \mathcal{F}(v) \subseteq \mathcal{L}$.

\noindent \textbf{Labelled Dataset:}
The dataset $\mathcal{D}$ of this task includes $(\mathcal{V_D}, \mathcal{L_D}, \mathcal{F_D})$ where $\mathcal{V_D}$ is a set of collected vulnerabilities, $\mathcal{F_D}$ is the labels (affected packages) of these vulnerabilities, and $\mathcal{L_D}$ is naturally defined as $\mathcal{F_D}(V_D)$.
The target of existing approaches is to learn the correlation from a given dataset $\mathcal{F^{'}} \sim \mathcal{F_D}$.



\subsection{Existing Ranking Approaches}
Conventional approaches model this task as a ranking task while all of these approaches face the scalability challenge.


\noindent \textbf{Ranking Approaches:}
They highly depend on the training data. For example, existing approaches use trained LightXML~\cite{lightxml} and ZestXML~\cite{chronos} as their classification models, which are limited to only seen libraries (or libraries whose names are close to seen labels), thus resulting in scalability limitations.
\begin{equation*}
\mathcal{F}_{classification}(\mathcal{V}) \subseteq \mathcal{L_D} \mbox{ \textbf{while} } \mathcal{F}(\mathcal{V}) \not\subseteq \mathcal{L_D}.
\end{equation*}

\noindent \textbf{Reranking Approaches:}
They need to correlate the input vulnerability description with all its candidate libraries. 
Specifically, they take a pair of one vulnerability $v$ and one library $l$ and output the likelihood of whether $l$ is affected by $v$: $\mathcal{F}_{IR}: \mathcal{V} \times \mathcal{L} \rightarrow [0,1]$.

Considering the large number of packages (e.g., 435,642 in Maven and 506,848 in Pypi) and vulnerabilities (more than 200,000 per year~\cite{nvd2022report}), existing IR approaches face high efficiency and resource costs.
Even though VulLibMiner~\cite{vullibminer}, a representative IR approach, uses a lightweight filter to screen out 512 candidates for comparison, it is still time-consuming (e.g., 10 minutes per vulnerability) to query a deep-learning model (or LLMs) for 512 times.

\subsection{Our Motivation}
To address the scalability problem, in this paper, we propose to model this task as a generation task as generation approaches have shown better effectiveness than IR/classification in other NLP tasks~\cite{mao2020generation, ye2020leveraging}.

\noindent \textbf{A Generation Task:}
It is formally defined as $\mathcal{F}_{Generation}: \mathcal{V} \rightarrow \mathcal{T}$ where $T$ is the textual response of generative pre-trained language models (e.g., LLMs).
Then we can filter the targeted names of affected packages by a lightweight filter, e.g., regular expressions.
The rationale behind our modeling is to address the scalability limitations by generation instead of IR/classification.

When compared with classification approaches, the output space of $\mathcal{T}$ includes the space of all existing library names (and even non-existing ones): 
\begin{equation*}
    \mathcal{L_D} \subseteq \mathcal{L} \subseteq \mathcal{T}.
\end{equation*}

When compared with IR approaches, a generative approach is invoked only once, thus making it possible to adapt LLMs within acceptable efficiency and resource costs.


\subsection{Challenges of Adopting LLMs}
\label{sec:empirical_study}

Before employing LLMs to generate the names of affected libraries, we conduct an empirical study to investigate the challenges when directly querying LLMs.
Specifically, we query ChatGPT with the descriptions of 2,789 vulnerabilities collected in a recent work~\cite{vullibminer}, and ChatGPT outputs the correct library names (exactly matching) in only 1,166 of them.
We conduct case studies on the rest 1,623 vulnerabilities to investigate the reasons for ChatGPT's incorrect responses.
Table~\ref{tab: fault case study} shows the classified reasons for ChatGPT's incorrect response.

In the former three categories of incorrect responses, which count for 64\%, ChatGPT mainly encounters non-existing library names. 
Although ChatGPT's responses share a large portion of common tokens with their corresponding ground truths, there are still slight differences between them.
For example, in CVE-2020-2167, the affected library is \CodeIn{com.openshift.jenkins:openshift-pipeline} while LLMs might change the group ID into \CodeIn{com.openshift.jenkins}, which is not an existing library.

As for the latter two categories, which count for 36\%, ChatGPT faces the challenge of lacking sufficient domain knowledge, thus resulting in misleading names (or even no structural names).
For example, in CVE-2020-11974, the description mentions both \CodeIn{DolphinScheduler} and \CodeIn{mysql} while ChatGPT incorrectly captures \CodeIn{mysql} as the affected package.


==> backup/conclusion-backup.tex <==
\section{Conclusion}\label{sec:conclusion}
In this paper, we have presented our work, \detector{}, the first generative approach to generate vulnerable third-party libraries via LLMs, thus reducing the scalability challenge of existing ranking approaches.
\detector{} is highly effective, achieving an accuracy of 0.806 while the best of SOTA approaches achieves only 0.669.
\detector{} includes a RAG technique and local search algorithm to improve the effectiveness of \detector{} by 8.9\% and 3.0\% on average, respectively.
\detector{} achieves better trade-offs between efficiency and accuracy than both existing and future ranking approaches.
Additionally, \detector{} has shown high value to security practice. 
We have submitted 28 pairs of <vulnerability, affected package> to GitHub advisory, and 22 of them have been accepted and merged.

==> backup/evaluation-backup.tex <==




















% % \subsubsection{Methodology}
% We evaluate the effectiveness of \detector{} on three testing sets from the perspective of the preceding three metrics, $precision@1$, $recall@1$, and $F1@1$.
% Note that these evaluation metrics cannot achieve 1.0 due to the various numbers of vulnerabilities' affected packages, we also include the ground truth results as the maximum values of these metrics.
% In this research question, we feed only one recommended package from VulLibMiner as a basic configuration.

% Similar to some baseline approaches, such as LightXML~\cite{lightxml} and FastXML~\cite{fastxml}, we also evaluate the effectiveness of \detector{} when it only outputs the package names in the top packages.
% Top packages are defined as those that have already been affected by vulnerabilities: $\mathcal{L} = \mathcal{L}_{test}$.
% Thus, we conduct evaluations by restricting the search space of post-processing as the top packages.


% \subsubsection{General Results}
% The upper part of Table~\ref{tab: baseline cmp} shows the Top1 values of precision, recall, and F1 score of \detector{} when generating vulnerable package names from all Java packages in Maven.
% We show that \detector{} achieves substantially high performance on all three metrics on the raw testing set.
% Specifically, the highest F1@1 of \detector{} is 0.626 while the ground truth of F1@1 is only 0.867.
% Table~\ref{tab: baseline cmp} also shows that there is no substantial difference between the performance of various base models before supervised fine-tuning (LLaMa-7B/13B, unsupervised fine-tuning or not).
% The difference between the maximum and minimum values of F1@1 on the raw testing set is less than 0.02.

% When compared with baseline approaches, the F1@1 of Chronos and VulLibMiner are 0.360 and 0.542, respectively.
% This result indicates that \detector{} outperforms them by 73.9\% and 15.5\%.
% With the help of input augmentation and post-processing, \detector{} can utilize LLMs to comprehend the descriptions of vulnerabilities and directly generate the vulnerable packages.


% \subsubsection{Results on the zero-shot testing set}
% Table~\ref{tab: baseline cmp} also includes the Top1 values of three metrics on the zero-shot testing set, $\mathcal{V}_{test}$.
% From this table, \detector{} also achieves a high F1@1 value of 0.540 on the zero-shot testing set.

% When compared with baseline approaches, the F1@1 of Chronos and VulLibMiner are 0.000 and 0.417, which is substantially less than that of \detector{}.
% The main reason for Chronos's low F1@1 is that it represents the package names based on the TF-IDF frequency to identify zero-shot packages while Java package names are much longer and complicated, thus being difficult to distinguish.
% For example, there are 1,208 Java packages with the same group id, \CodeIn{org.jenkins-ci.plugins}, and packages containing such a long group id tend to have similar TF-IDF representation.
% The main reason for \detector{}'s higher F1@1 is that \detector{} combines its prior knowledge with the recommended packages, thus generating more accurate results.

% % generate package names from those with similar functionalities instead of all packages 
% % combines the recommended packages with knowledge
% % takes advantage of the recommended packages and generates responses from all related packages while VulLibMiner separately correlates each package with a given vulnerability.


% \subsubsection{Results post-processed among top packages}

% The results are shown in the lower part of Table~\ref{tab: baseline cmp}.
% We show that focusing on the top packages can further improve the effectiveness of identifying vulnerable packages.
% The F1@1 of \detector{} is 0.690, 0.644, and 0.715 in $\mathcal{V}_{test}$, $\mathcal{V}_{zero}$, and $\mathcal{V}_{full}$, respectively.

% Focusing on the top packages can be practical in some cases.
% For example, developers might not concern about vulnerable packages not being used in their projects. 
% Therefore, we also show the effectiveness of identifying vulnerable packages among the top packages in this subsection.
% Thus developers can use \detector{} based on their requirements.



% \myfindings[1]{\detector{} can effectively identify vulnerable packages (including zero-shot packages) better than the SOTA approaches. If we focus on top packages, \detector{} achieves even higher performance.}

% \subsection{\textbf{RQ2}: To what extent can our RAG technique help generate vulnerable packages?}~\label{sec: rq2}

% % \subsubsection{Methodology}
% We evaluate the effectiveness of \detector{} with various recommended packages to see input augmentation's benefits on \detector{}.
% In this research question, we evaluate the base model of LLaMa-13B without unsupervised fine-tuning because its effectiveness is quite similar to other base models.
% Specifically, we use TF-IDF and VulLibMiner to recommend at most three packages.

% \subsubsection{Metrics}
% Considering the number of recommended packages, we use the metrics F1@k (k=1,2,3) instead of only F1@1 to see whether more recommended packages improve \detector{}'s Topk metrics.

% To directly show how \detector{} utilizes the recommended packages, we use another perspective of metrics, the relative precision when \detector{} accepts or rejects the recommended packages.
% It is formally defined as:
% \begin{equation}
%     \begin{aligned}
%         Accept &:= \{v| predict_m(v) = predict_r(v) \} \\
%         Reject &:= \{v| predict_m(v) \not= predict_r(v) \} \\
%         R_{Accept} &:= \#Accept / (\# Accept + \# Reject) \\
%         R^{Model}_{Accept} &:= \mathop{Avg.}\limits_{v \in Accept} precison@1(v) (\mbox{\detector{}})  \\
%         R^{Model}_{Reject} &:= \mathop{Avg.}\limits_{v \in Reject} precison@1(v) (\mbox{\detector{}})  \\
%         R^{Rec}_{Reject} &:= \mathop{Avg.}\limits_{v \in Reject} precison@1(v) (\mbox{Recommend}) \\
%     \end{aligned}
% \end{equation}

% \subsubsection{General Results}
% Table~\ref{tab: various recommend} shows the F1@k results of \detector{} with various recommended packages.
% From this table, we show that the recommended packages increase the effectiveness of \detector{} in terms of F1@1 from 0.593 to 0.626 on the testing set.
% However, the recommended packages do not substantially increase the F1@2 and F1@3.
% The main reason is that \detector{} tends to generate only one vulnerable Java package because each Java vulnerability affects less than two packages on average~\cite{vullibminer}.
% On the contrary, baseline approaches identify vulnerable packages based on a probability threshold, thus outputting a large list of packages.


% \begin{table*}[t]
% \centering
% \caption{F1@k of \detector{} with Various Recommended packages (LLaMa-13B without Unsupervised Fine-Tuning)}
% \label{tab: various recommend}
% \begin{tabular}{llccccccccc}
% \toprule
% \multicolumn{2}{c}{\multirow{2}{*}{Approach}}                   & \multicolumn{3}{c}{F1@1}      & \multicolumn{3}{c}{F1@2}      & \multicolumn{3}{c}{F1@3}      \\
% \cmidrule(lr){3-5}\cmidrule(lr){6-8}\cmidrule(lr){9-11}
% \multicolumn{2}{c}{}                                            & Raw   & Zero-shot & Full-shot & Raw   & Zero-shot & Full-shot & Raw   & Zero-shot & Full-shot \\
% \midrule
% \multicolumn{2}{c}{Ground Truth}                                & 0.867 & 0.931     & 0.840     & 0.792 & 0.746     & 0.807     & 0.677 & 0.704     & 0.602     \\
% \multicolumn{2}{c}{Chronos}                                     & 0.360 & 0.000     & 0.505     & 0.292 & 0.000     & 0.407     & 0.247 & 0.000     & 0.344     \\
% \multicolumn{2}{c}{VulLibMiner}                                 & 0.561 & 0.507     & 0.581     & 0.486 & 0.395     & 0.519     & 0.418 & 0.313     & 0.457     \\
% \midrule
% \multicolumn{2}{c}{\makecell[l]{VulLibGen (None)}}                    & 0.593 & 0.394     & 0.670     & 0.502 & 0.290     & 0.584     & 0.411 & 0.226     & 0.483     \\
% \midrule
% \multirow{3}{*}{\makecell[l]{VulLibGen (recom-\\ mended by TF-IDF )}}      & 1 Lib & 0.604 & 0.446     & 0.664     & 0.491 & 0.298     & 0.565     & \textbf{0.417} & 0.252     & \textbf{0.480}     \\
%                                                          & 2 Libs & 0.597 & 0.443     & 0.656     & 0.507 & 0.309     & 0.583     & 0.410 & 0.233     & 0.477     \\
%                                                          & 3 Libs & 0.602 & 0.445     & 0.663     & 0.493 & 0.323     & 0.558     & 0.408 & 0.250     & 0.469     \\
% \midrule
% \multirow{3}{*}{\makecell[l]{VulLibGen (recom-\\ mended by VulLibMiner)}} & 1 Lib & \textbf{0.626} & 0.483     & \textbf{0.681}     & \textbf{0.508} & 0.351     & \textbf{0.567}     & 0.416 & 0.268     & 0.473     \\
%                                                          & 2 Libs & 0.618 & \textbf{0.547}     & 0.644     & 0.497 & 0.368     & 0.546     & 0.406 & 0.284     & 0.453     \\
%                                                          & 3 Libs & 0.612 & 0.546     & 0.636     & 0.499 & \textbf{0.383}     & 0.543     & 0.405 & \textbf{0.293}     & 0.448     \\
% \bottomrule
% \end{tabular}
% \end{table*}


% \subsubsection{Improvement in identifying zero-shot packages}
% Table~\ref{tab: various recommend} shows \detector{}'s F1@k results in terms of identifying full-shot and zero-shot packages.
% We show that the Topk F1 scores on the full-shot testing set vary only a little upon different recommended packages.
% For example, the difference between the maximum and minimum values of F1@1 on the full-shot testing set is less than 0.04.
% On the contrary, the recommended packages substantially increase the F1@1 on the zero-shot testing set by 39\% (from 0.394 to 0.547).
% Additionally, recommended packages with higher quality (e.g., from no recommended packages to TF-IDF, or from TF-IDF to VulLibMiner) also help \detector{} to identify zero-shot packages.
% For example, the F1@1 increases by 8\% on average (upon Topk recommended packages) when we use the recommended results from VulLibMiner instead of TF-IDF.
% The main reason for this improvement is that zero-shot packages are difficult for LLMs to identify, and input augmentation provides examples of packages whose functionalities are likely to be affected by a given vulnerability.
% Thus, \detector{} can generate package names from those with similar functionalities instead of all packages.


% % the recommended packages enable them to correlate the knowledge of the input vulnerability with a small subset of packages that are similar to the recommended ones in functionalities.


% \subsubsection{Results of relative precision}
% Table~\ref{tab: hit rate} shows the results of four relative precision metrics.
% This table shows that \detector{} can judge the quality of recommended packages.
% The $R_{Accept}$ increases by 283\% on average (upon Topk) from TF-IDF to VulLibMiner.
% Additionally, we also show that \detector{} can determine whether the recommended results are correct or not.
% Here we take the Top1 recommended package from VulLibMiner as an example.
% The $R^{Model}_{Accept}$ equals 83\%, indicating that the recommended results are likely to be correct when they are accepted.
% Additionally, $R^{Model}_{Reject}$ equals 41\% while $R^{Rec}_{Reject}$ equals 13\%, indicating that the output of \detector{} is more likely to be correct than the recommended packages when \detector{} rejects them.
% Thus, we can make the conclusion that \detector{} can accept correct recommended packages while generating better results based on incorrect ones.



% \begin{table}[t]
% \centering
% \caption{Results of Relative Precision (LLaMa-13B without Unsupervised Fine-Tuning)}
% \label{tab: hit rate}
% \begin{tabular}{lrrrrrr}
% \toprule
% \multirow{2}{*}{Metric}    & \multicolumn{3}{c}{TF-IDF} & \multicolumn{3}{c}{VulLibMiner} \\
%     & Top1    & Top2    & Top3   & Top1      & Top2     & Top3     \\
% \midrule
% $R_{Accept}$    & 18\%    & 25\%    & 31\%   & 55\%      & 77\%     & 73\%     \\
% $R^{Model}_{Accept}$       & 79\%    & 73\%    & 74\%   & 83\%      & 72\%     & 71\%     \\
% $R^{Model}_{Reject}$      & 58\%    & 57\%    & 57\%   & 41\%      & 31\%     & 38\%     \\
% $R^{Rec}_{Reject}$      & 4\%    & 3\%    & 4\%   & 13\%      & 9\%     & 7\%     \\
%                                % Incorrect & 38\%    & 39\%    & 39\%   & 45\%      & 61\%     & 55\%     \\
% \bottomrule
% \end{tabular}
% \end{table}


% \myfindings[2]{Input augmentation substantially increases the average F1@1 on identifying zero-shot packages by 39\%.
% Additionally, \detector{} can judge whether these recommended packages are correct and generate better results based on the incorrect ones.}

% \begin{table*}[t]
%     \centering
%     \caption{F1@1 of \detector{} Before and After Post-Processing}
%     \label{tab: post-processing}
%     \begin{tabular}{ccccccrcrcr}
%     \toprule
%     \multirow{2}{*}{Base   Model}                              &  \multicolumn{1}{c}{\multirow{2}{*}{\makecell[c]{Recommend\\ (One package)}}} & \multicolumn{3}{c}{Before Post-processing(F1@1)}  & \multicolumn{6}{c}{After Post-processing(F1@1)}                                            \\
%     \cmidrule(lr){3-5}\cmidrule(lr){6-11}
%                                                                &                                                   & Raw   & Zero-shot & Full-shot & Raw   &  \multicolumn{1}{c}{$\uparrow$}      & Zero-shot &     \multicolumn{1}{c}{$\uparrow$}     & Full-shot &     \multicolumn{1}{c}{$\uparrow$}     \\
%     \midrule
%     % \multirow{3}{*}{\makecell[c]{LLaMa-13B With\\ Maven Corpus}}    & None                                    & 0.541 & 0.286     & 0.640     & 0.596 & (10\%) & 0.420     & (47\%) & 0.664     & (4\%)   \\
%     % & \multirow{1}{*}{TF-IDF}                                            & 0.557 & 0.306     & 0.654     & 0.602 & (8\%)  & 0.441     & (44\%) & 0.664     & (2\%) \\
%     %                                                            & \multirow{1}{*}{VulLibMiner}                                       & 0.598 & 0.477     & 0.645     & 0.615 & (3\%)  & 0.516     & (8\%) & 0.652     & (1\%) \\
%     % \midrule
%     \multirow{3}{*}{\makecell[c]{LLaMa-13B Without\\   Maven Corpus}}  &   None                                 & 0.524 & 0.214     & 0.646     & 0.593 & (13\%) & 0.394     & (84\%) & 0.670     & (4\%) \\
%     & \multirow{1}{*}{TF-IDF}                                            & 0.551 & 0.282     & 0.656     & 0.604 & (10\%) & 0.446     & (58\%) & 0.664     & (1\%) \\
%     & \multirow{1}{*}{VulLibMiner}                                       & 0.595 & 0.399     & 0.671     & 0.626 & (5\%)  & 0.483     & (21\%) & 0.681     & (1\%) \\
%     \bottomrule
%     \end{tabular}
%     \end{table*}


% \subsection{\textbf{RQ3}: To what extent can post-processing help \detector{} address hallucinations?}
% We evaluate the effectiveness of \detector{} before and after post-processing from the perspective of F1@1 to show the benefits of post-processing.
% As shown in Section~\ref{sec: rq2}, the number of recommended packages does not affect the effectiveness of \detector{}, so we evaluate \detector{} on the LLaMa-13B model with one recommended package from TF-IDF and VulLibMiner in this research question. 

% \subsubsection{General Results}
% Table~\ref{tab: post-processing} shows the F1@1 of \detector{} before and after processing.
% From this table, we show that the benefits of our post-processing technique range from 3\% to 13\%.
% Additionally, the improvement of the base mode with unsupervised fine-tuning (7\% on average) is relatively less than that without unsupervised fine-tuning (9.3\% on average).
% The main reason for this difference is that both unsupervised fine-tuning and post-processing aim at addressing hallucinations, and their improvement might be overlapped.

% Table~\ref{alg: post-processing} also shows that the improvement on the full-shot testing set is limited (less than 4\%).
% However, the improvement on the zero-shot testing set can be substantially high, especially when given low-quality recommended results. 
% For example, the improvement of \detector{} with TF-IDF recommendation or no recommendation is larger than 44\% while the improvement of \detector{} with VulLibMiner recommendation is 8\% and 21\%.

% \subsubsection{A case study}
% Table~\ref{tab: case2} shows an example result of CVE-2020-2311 to show how post-processing helps \detector{}.
% The targeted vulnerable package is \CodeIn{maven:io.jenkins.plugins:aws-global-\\ configuration}.
% Although The recommended package is correct, the output of \detector{} changes its group id from \CodeIn{io.jenkins.plugins} to \CodeIn{org.jenkins-ci.plugins}.
% The main reason for this change is that there are only 2,34 Java packages with the former group id and 1,208 Java packages with the latter group id.
% Thus, \detector{} is likely to mix up these two similar group ids.
% However, our post-processing algorithm notices that the former group id with the given artifact id cannot be concatenated into an existing package name, and the former group id has a minimal Levenshitein distance from the latter one among those containing this artifact id.



% \subsubsection{Correctness of group ids and artifact ids}
% To directly shows how much portion of generated package names is revised during post-processing, we further analyze the correctness of each component (i.e., group ids and artifact ids) of generated package names.
% Table~\ref{tab: existing component} shows the results of their correctness.
% We show that about 78\% of the package names generated by \detector{} belong to existing packages.
% Among the 22\% non-existing results, non-existing artifact ids contribute to most of them.
% Generating existing artifact ids is difficult because the number of existing artifact ids (274,232) is larger than the number of existing group ids (53,074). 

    
% \begin{table}[t]
% \centering
% \caption{Portions of Various Faults}
% \label{tab: existing component}
% \begin{tabular}{ccccc}
% \toprule
% \multicolumn{1}{c}{Model}                       & \multicolumn{1}{c}{\makecell[c]{IR package\\ Resource}} & \makecell[c]{Existing\\ package\\ Name} & \makecell[c]{Existing\\ GroupID} & \makecell[c]{Existing\\ ArtifactID} \\
% \midrule
% \multirow{4}{*}{ChatGPT} & \multicolumn{1}{c}{None}                & 71.7\%               & 92.3\%          & 76.6\%             \\
%                                            & \multirow{1}{*}{TF-IDF}              & 77.3\%               & 96.2\%          & 81.0\%             \\
%                                            & \multirow{1}{*}{BERT}         & 82.8\%               & 97.8\%          & 85.6\%             \\
% \cmidrule(lr){2-5}
% & Average  & 77.2\% & 95.4\% & 81.0\% \\
% \midrule
% \multirow{4}{*}{GPT4} & \multicolumn{1}{c}{None}                & 71.7\%               & 92.3\%          & 76.6\%             \\
%                                            & \multirow{1}{*}{TF-IDF}              & 77.3\%               & 96.2\%          & 81.0\%             \\
%                                            & \multirow{1}{*}{BERT}         & 82.8\%               & 97.8\%          & 85.6\%             \\
% \cmidrule(lr){2-5}
% & Average  & 77.2\% & 95.4\% & 81.0\% \\
% \midrule
% \multirow{4}{*}{LLaMa} & \multicolumn{1}{c}{None}                & 71.7\%               & 92.3\%          & 76.6\%             \\
%                                            & \multirow{1}{*}{TF-IDF}              & 77.3\%               & 96.2\%          & 81.0\%             \\
%                                            & \multirow{1}{*}{BERT}         & 82.8\%               & 97.8\%          & 85.6\%             \\
% \cmidrule(lr){2-5}
% & Average  & 77.2\% & 95.4\% & 81.0\% \\
% \midrule
% \multirow{4}{*}{Vicuna} & \multicolumn{1}{c}{None}                & 71.7\%               & 92.3\%          & 76.6\%             \\
%                                            & \multirow{1}{*}{TF-IDF}              & 77.3\%               & 96.2\%          & 81.0\%             \\
%                                            & \multirow{1}{*}{BERT}         & 82.8\%               & 97.8\%          & 85.6\%             \\
% \cmidrule(lr){2-5}
% & Average  & 77.2\% & 95.4\% & 81.0\% \\
% \bottomrule
% \end{tabular}
% \end{table}

% \begin{table*}[t]
% \begin{tabular}{cccccccccccc}
% \multirow{2}{*}{Model}   & IR package & \multicolumn{5}{c}{Fault Proportion   (Before Fixing)} & \multicolumn{5}{c}{Fault Proportion   (After Fixing)} \\
%                          & Resource   & Type1     & Type2     & Type3    & Type4    & Type5    & Type1     & Type2    & Type3    & Type4    & Type5    \\
% \multirow{3}{*}{ChatGPT} & None       & 12.34\%   & 12.34\%   & 12.34\%  & 12.34\%  & 12.34\%  & 12.34\%   & 12.34\%  & 12.34\%  & 12.34\%  & 12.34\%  \\
%                          & TF-IDF     & 12.34\%   & 12.34\%   & 12.34\%  & 12.34\%  & 12.34\%  & 12.34\%   & 12.34\%  & 12.34\%  & 12.34\%  & 12.34\%  \\
%                          & BERT       & 12.34\%   & 12.34\%   & 12.34\%  & 12.34\%  & 12.34\%  & 12.34\%   & 12.34\%  & 12.34\%  & 12.34\%  & 12.34\%  \\
% \multirow{3}{*}{GPT4}    & None       & 12.34\%   & 12.34\%   & 12.34\%  & 12.34\%  & 12.34\%  & 12.34\%   & 12.34\%  & 12.34\%  & 12.34\%  & 12.34\%  \\
%                          & TF-IDF     & 12.34\%   & 12.34\%   & 12.34\%  & 12.34\%  & 12.34\%  & 12.34\%   & 12.34\%  & 12.34\%  & 12.34\%  & 12.34\%  \\
%                          & BERT       & 12.34\%   & 12.34\%   & 12.34\%  & 12.34\%  & 12.34\%  & 12.34\%   & 12.34\%  & 12.34\%  & 12.34\%  & 12.34\%  \\
% \multirow{3}{*}{LLaMa}   & None       & 12.34\%   & 12.34\%   & 12.34\%  & 12.34\%  & 12.34\%  & 12.34\%   & 12.34\%  & 12.34\%  & 12.34\%  & 12.34\%  \\
%                          & TF-IDF     & 12.34\%   & 12.34\%   & 12.34\%  & 12.34\%  & 12.34\%  & 12.34\%   & 12.34\%  & 12.34\%  & 12.34\%  & 12.34\%  \\
%                          & BERT       & 12.34\%   & 12.34\%   & 12.34\%  & 12.34\%  & 12.34\%  & 12.34\%   & 12.34\%  & 12.34\%  & 12.34\%  & 12.34\%  \\
% \multirow{3}{*}{Vicuna}  & None       & 12.34\%   & 12.34\%   & 12.34\%  & 12.34\%  & 12.34\%  & 12.34\%   & 12.34\%  & 12.34\%  & 12.34\%  & 12.34\%  \\
%                          & TF-IDF     & 12.34\%   & 12.34\%   & 12.34\%  & 12.34\%  & 12.34\%  & 12.34\%   & 12.34\%  & 12.34\%  & 12.34\%  & 12.34\%  \\
%                          & BERT       & 12.34\%   & 12.34\%   & 12.34\%  & 12.34\%  & 12.34\%  & 12.34\%   & 12.34\%  & 12.34\%  & 12.34\%  & 12.34\% 
% \end{tabular}
% \end{table*}



% \myfindings[3]{Post-processing substantially increases the
% average F1@1 by 9.3\% on average.}

% \subsection{\textbf{RQ4}: How efficiently can \detector{} identify vulnerable Java packages?}

% This research question evaluates the runtime overhead of \detector{}.
% We measure the end-to-end time of \detector{}'s each component.
% We train 20 epochs for each model used in LightXML and 30 epochs for VulLibMiner until their training losses converge.
% The training details of \detector{} are listed in Table~\ref{tab: hyper parameter}.


% \subsubsection{General results}
% The evaluation result is shown in Table~\ref{tab: time}.
% Although \detector{} costs hundreds of hours for unsupervised fine-tuning, this stage of fine-tuning can be skipped as it does not mainly contribute to the effectiveness of \detector{}.
% For the time consumption for supervised fine-tuning, the maximum time cost is less than 36 hours, which is acceptable when compared with baseline approaches.
% As for the time consumption for prediction and post-processing, it costs less than 1 hour for 633 vulnerabilities in the testing set.
% Thus, the end-to-end time consumption for \detector{} to identify a given vulnerability is less than 6 seconds on average.
% In general, it is practical for \detector{} to identify the affected packages of vulnerabilities.

% \begin{table}[t]
% \centering
% \caption{Time Consumption of \detector{} and Baselines}
% \label{tab: time}
% \begin{tabular}{llrrr}
% \toprule
% \multicolumn{2}{l}{Approach}                          & Train (h) & Pred. (min) & Post. (min) \\
% \midrule
% \multicolumn{2}{l}{LightXML}                          & 6.30      & 2.14        & -               \\
% \multicolumn{2}{l}{Chronos}                           & 1.19      & 1.12        & 7.34            \\
% \multicolumn{2}{l}{VulLibMiner}                       & 17.00     & 2.63        & -               \\
% % \midrule
% \multicolumn{2}{l}{\detector{}-max}                         & 35.50     & 39.35       & 8.45            \\
% \cmidrule(lr){1-2}\cmidrule(lr){3-5}
% \multirow{2}{*}{\makecell[l]{Unsupervised\\ Fine-tuning}} & 7B      & 276.02    & -           & -               \\
%                                             & 13B     & 805.30    & -           & -               \\
% \cmidrule(lr){1-2}\cmidrule(lr){3-5}
% \multirow{2}{*}{\makecell[l]{Raw LLaMa}}        & 7B      & -         & 270.30      & -               \\
%                                             & 13B     & -         & 301.27      & -               \\
% \cmidrule(lr){1-2}\cmidrule(lr){3-5}
% \multirow{4}{*}{\makecell[l]{Supervised\\ Fine-Tuning}}   & 7B-min  & 32.92     & 25.27       & 3.93            \\
%                                             & 7B-max  & 35.50     & 34.20       & 9.15            \\
%                                             & 13B-min & 30.45     & 29.20       & 3.62            \\
%                                             & 13B-max & 31.17     & 39.35       & 8.45            \\
% \bottomrule
% \end{tabular}
%  \begin{tablenotes}
%     \item Here \CodeIn{-max} and \CodeIn{-min} indicate the maximum and minimum time consumption under various configurations, respectively.
%  \end{tablenotes}
% \end{table}


% \myfindings[4]{The training time consumption of \detector{} is 35.5 hours and it identifies vulnerable packages in 6 seconds per vulnerability, which is acceptable in practice.}


% \subsection{\textbf{RQ5}: How much benefit can our industrial partner (and security practice) gain from our approach?}

% \subsubsection{Methodology}

% To evaluate \detector{}'s impact on our industrial partner

% To evaluate \detector{}'s impact on our security practice, we take \detector{} as an oracle to identify <vulnerability, package> pairs as complements of one open-sourced vulnerability database, GitHub Advisory~\cite{githubAD}.
% Note that there are a large amount of Java vulnerabilities besides those included in VulLib and the number of vulnerabilities is rapidly increasing. In this research question, we conduct an empirical study by answering the following two sub-questions:


% \myfindings[4]{\detector{} substantially reduces the manual costs of identifying the affected packages of vulnerabilities.
% Additionally, we demonstrate \detector{}'s high value of security practice by submitting 25 of the identified <vulnerability, package> pairs to GitHub Advisory, and 22 of them are accepted.}

% \begin{table}[t]
% \centering
% \caption{The Statistics of Dataset VulLib}
% \label{tab: dataset info}
% \begin{tabular}{lrc|rc}
% \toprule
% VulLib     & \#$\mathcal{V}$ & \#$\mathcal{V}_{zero}$ & \#$\mathcal{L}$ & \#$\mathcal{L}_{zero}$ \\ 
% \midrule
% Training   & 1,860               & -                           & 1,509               & -                          \\
% Validation & 620                 & 233 (37.58\%)               & 663                 & 325 (49.02\%)              \\
% Testing    & 633                 & 228 (36.02\%)               & 676                 & 307 (45.41\%)              \\ 
% \midrule
% Total      & 3,113               & -                           & 2,095               & -                         \\
% \bottomrule
% \end{tabular}
% \end{table}

% \begin{table*}[t]
% \centering
% \caption{Comparison of \detector{}'s Effectiveness (Top1) with the SOTA Approaches}
% \label{tab: baseline cmp}
% \begin{tabular}{ccllllllllll}
% \toprule
% \multirow{2}{*}{\makecell[l]{Search\\   Space}} & \multirow{2}{*}{Approach}                                                       & \multicolumn{1}{c}{\multirow{2}{*}{Model}} & \multicolumn{3}{c}{Raw} & \multicolumn{3}{c}{Zero-shot} & \multicolumn{3}{c}{Full-Shot} \\
% \cmidrule(lr){4-6}\cmidrule(lr){7-9}\cmidrule(lr){10-12}
%                                                 &                                                                                 & \multicolumn{1}{c}{}                       & Prec.  & Rec.   & F1    & Prec.    & Rec.     & F1      & Prec.    & Rec.     & F1      \\
% \midrule
% \multicolumn{1}{l}{}                            & \multicolumn{1}{l}{Ground Truth} & -                                                                                          & 1.000  & 0.765  & 0.867 & 1.000    & 0.871    & 0.931   & 1.000    & 0.723    & 0.840   \\
% \multirow{6}{*}{Maven}                          & \multicolumn{1}{l}{Chronos}                                                     & ZestXML                                    & 0.416  & 0.318  & 0.360 & 0.000    & 0.000    & 0.000   & 0.583    & 0.445    & 0.505   \\
%                                                 & \multicolumn{1}{l}{VulLibMiner}                                                 & BERT-FNN                                   & 0.544  & 0.497  & 0.561 & 0.431    & 0.485    & 0.507   & 0.689    & 0.502    & 0.581   \\
% \cmidrule(lr){2-12}
%                                                 & \multirow{2}{*}{\makecell[l]{\detector{}   (with\\ Unsupervised Fine-Tuning)}}    & LLaMa-7B                                   & 0.699  & 0.545  & 0.612 & 0.513    & 0.471    & 0.491   & 0.773    & 0.574    & 0.658   \\
%                                                 &                                                                                 & LLaMa-13B                                  & 0.697  & 0.550  & 0.615 & 0.544    & 0.496    & 0.516   & 0.758    & 0.572    & 0.652   \\
% \cmidrule(lr){2-12}
%                                                 & \multirow{2}{*}{\makecell[l]{\detector{}   (without\\ Unsupervised Fine-Tuning)}} & LLaMa-7B                                   & 0.703  & 0.548  & 0.616 & 0.563    & 0.520    & \textbf{0.540}   & 0.758    & 0.560    & 0.644   \\
%                                                 &                                                                                 & LLaMa-13B                                  & 0.720  & 0.554  & \textbf{0.626} & 0.506    & 0.461    & 0.483   & 0.805    & 0.591    & \textbf{0.681}   \\
% \midrule
% \multirow{5}{*}{Top-Lib}                        & \multicolumn{1}{l}{LightXML}                                                    & LightXML                                   & 0.444  & 0.328  & 0.377 & 0.000    & 0.000    & 0.000   & 0.665    & 0.438    & 0.528   \\
% \cmidrule(lr){2-12}
%                                                 & \multirow{2}{*}{\makecell[l]{\detector{}   (with\\ Unsupervised Fine-Tuning)}}    & LLaMa-7B                                   & 0.791  & 0.612  & 0.690 & 0.675    & 0.598    & 0.634   & 0.837    & 0.617    & 0.710   \\
%                                                 &                                                                                 & LLaMa-13B                                  & 0.781  & 0.607  & 0.683 & 0.656    & 0.585    & 0.618   & 0.830    & 0.616    & 0.707   \\
% \cmidrule(lr){2-12}
%                                                 & \multirow{2}{*}{\makecell[l]{\detector{} (without\\ Unsupervised Fine-Tuning)}} & LLaMa-7B                                   & 0.788  & 0.611  & 0.688 & 0.675    & 0.615    & \textbf{0.644}   & 0.832    & 0.609    & 0.703   \\
%                                                 &                                                                                 & LLaMa-13B                                  & 0.793  & 0.609  & \textbf{0.689} & 0.656    & 0.583    & 0.617   & 0.847    & 0.619    & \textbf{0.715}   \\
% \bottomrule
% \end{tabular}
% \end{table*}

% \begin{table}[t]
% \centering
% \caption{Parameters Used in Fine-Tuning LLMs}
% \label{tab: hyper parameter}
% % \begin{tabular}{ll}
% \begin{tabular}{l|l}
% \toprule
% Parameters           & Parameters           \\
% \midrule
% Train Batch Size : 4 & Learning Rate : 2e-5      \\
% Evaluation Batch Size : 4 & Weight Decay  : 0.00        \\
% Learning Rate schedule : Cosine    & Warmup Ratio  : 0.03         \\
% \bottomrule
% \end{tabular}
% \end{table}




% \begin{table*}[t]
% \begin{tabular}{cccccccccccc}
% \multirow{2}{*}{Model}   & IR package & \multicolumn{5}{c}{Fault Proportion   (Before Fixing)} & \multicolumn{5}{c}{Fault Proportion   (After Fixing)} \\
%                          & Resource   & Type1     & Type2     & Type3    & Type4    & Type5    & Type1     & Type2    & Type3    & Type4    & Type5    \\
% \multirow{3}{*}{ChatGPT} & None       & 12.34\%   & 12.34\%   & 12.34\%  & 12.34\%  & 12.34\%  & 12.34\%   & 12.34\%  & 12.34\%  & 12.34\%  & 12.34\%  \\
%                          & TF-IDF     & 12.34\%   & 12.34\%   & 12.34\%  & 12.34\%  & 12.34\%  & 12.34\%   & 12.34\%  & 12.34\%  & 12.34\%  & 12.34\%  \\
%                          & BERT       & 12.34\%   & 12.34\%   & 12.34\%  & 12.34\%  & 12.34\%  & 12.34\%   & 12.34\%  & 12.34\%  & 12.34\%  & 12.34\%  \\
% \multirow{3}{*}{GPT4}    & None       & 12.34\%   & 12.34\%   & 12.34\%  & 12.34\%  & 12.34\%  & 12.34\%   & 12.34\%  & 12.34\%  & 12.34\%  & 12.34\%  \\
%                          & TF-IDF     & 12.34\%   & 12.34\%   & 12.34\%  & 12.34\%  & 12.34\%  & 12.34\%   & 12.34\%  & 12.34\%  & 12.34\%  & 12.34\%  \\
%                          & BERT       & 12.34\%   & 12.34\%   & 12.34\%  & 12.34\%  & 12.34\%  & 12.34\%   & 12.34\%  & 12.34\%  & 12.34\%  & 12.34\%  \\
% \multirow{3}{*}{LLaMa}   & None       & 12.34\%   & 12.34\%   & 12.34\%  & 12.34\%  & 12.34\%  & 12.34\%   & 12.34\%  & 12.34\%  & 12.34\%  & 12.34\%  \\
%                          & TF-IDF     & 12.34\%   & 12.34\%   & 12.34\%  & 12.34\%  & 12.34\%  & 12.34\%   & 12.34\%  & 12.34\%  & 12.34\%  & 12.34\%  \\
%                          & BERT       & 12.34\%   & 12.34\%   & 12.34\%  & 12.34\%  & 12.34\%  & 12.34\%   & 12.34\%  & 12.34\%  & 12.34\%  & 12.34\%  \\
% \multirow{3}{*}{Vicuna}  & None       & 12.34\%   & 12.34\%   & 12.34\%  & 12.34\%  & 12.34\%  & 12.34\%   & 12.34\%  & 12.34\%  & 12.34\%  & 12.34\%  \\
%                          & TF-IDF     & 12.34\%   & 12.34\%   & 12.34\%  & 12.34\%  & 12.34\%  & 12.34\%   & 12.34\%  & 12.34\%  & 12.34\%  & 12.34\%  \\
%                          & BERT       & 12.34\%   & 12.34\%   & 12.34\%  & 12.34\%  & 12.34\%  & 12.34\%   & 12.34\%  & 12.34\%  & 12.34\%  & 12.34\% 
% \end{tabular}
% \end{table*}



% \begin{table}[t]
% \centering
% \caption{Portions of Various Faults}
% \label{tab: existing component}
% \begin{tabular}{ccccc}
% \toprule
% \multicolumn{1}{c}{Model}                       & \multicolumn{1}{c}{\makecell[c]{IR package\\ Resource}} & \makecell[c]{Existing\\ package\\ Name} & \makecell[c]{Existing\\ GroupID} & \makecell[c]{Existing\\ ArtifactID} \\
% \midrule
% \multirow{4}{*}{ChatGPT} & \multicolumn{1}{c}{None}                & 71.7\%               & 92.3\%          & 76.6\%             \\
%                                            & \multirow{1}{*}{TF-IDF}              & 77.3\%               & 96.2\%          & 81.0\%             \\
%                                            & \multirow{1}{*}{BERT}         & 82.8\%               & 97.8\%          & 85.6\%             \\
% \cmidrule(lr){2-5}
% & Average  & 77.2\% & 95.4\% & 81.0\% \\
% \midrule
% \multirow{4}{*}{GPT4} & \multicolumn{1}{c}{None}                & 71.7\%               & 92.3\%          & 76.6\%             \\
%                                            & \multirow{1}{*}{TF-IDF}              & 77.3\%               & 96.2\%          & 81.0\%             \\
%                                            & \multirow{1}{*}{BERT}         & 82.8\%               & 97.8\%          & 85.6\%             \\
% \cmidrule(lr){2-5}
% & Average  & 77.2\% & 95.4\% & 81.0\% \\
% \midrule
% \multirow{4}{*}{LLaMa} & \multicolumn{1}{c}{None}                & 71.7\%               & 92.3\%          & 76.6\%             \\
%                                            & \multirow{1}{*}{TF-IDF}              & 77.3\%               & 96.2\%          & 81.0\%             \\
%                                            & \multirow{1}{*}{BERT}         & 82.8\%               & 97.8\%          & 85.6\%             \\
% \cmidrule(lr){2-5}
% & Average  & 77.2\% & 95.4\% & 81.0\% \\
% \midrule
% \multirow{4}{*}{Vicuna} & \multicolumn{1}{c}{None}                & 71.7\%               & 92.3\%          & 76.6\%             \\
%                                            & \multirow{1}{*}{TF-IDF}              & 77.3\%               & 96.2\%          & 81.0\%             \\
%                                            & \multirow{1}{*}{BERT}         & 82.8\%               & 97.8\%          & 85.6\%             \\
% \cmidrule(lr){2-5}
% & Average  & 77.2\% & 95.4\% & 81.0\% \\
% \bottomrule
% \end{tabular}
% \end{table}



==> backup/intro-backup-1.tex <==
\begin{figure}[h]
\centering
\includegraphics[width=1\linewidth]{figures/vulnerability-report.drawio.pdf}
\caption{GitHub Advisory Report for CVE-2020-2318}
\label{fig: case}
\end{figure}

\section{Introduction}~\label{sec:intro}
With the increasing usage of third-party software packages, their security vulnerabilities pose great challenges to software and network systems.
A recent study~\cite{wang2020empirical} shows that 84\% third-party packages contain vulnerabilities and 60\% of them are high-risk ones.
To avoid potential risks posed by these vulnerabilities, developers maintain vulnerability databases, e.g., the National Vulnerability Database (NVD)~\cite{nvd} and GitHub Advisory~\cite{githubAD} for reference.
These databases help developers realize and deploy vulnerability patches.
Figure~\ref{fig: case} shows an example report of one vulnerability, CVE-2020-2318~\footnote{https://github.com/advisories/GHSA-485q-v457-3p58}.
It includes the affected package \CodeIn{org.jenkins-ci.plugins:mailcommander} and its corresponding versions.
The field of affected packages is specified by the developers who create this CVE. However, recent studies show that more than half of vulnerability reports have missing or incorrect package information~\cite{lightxml,viem}.
% \xueqing{can we say the package information is incorrect?}
% \tianyu{I think it's better not to mention incorrect, otherwise, our ground truth of labels might be challenged.}
To this end, the databases hire human maintainers to manually complete or validate the package information, e.g., maintainers from the GitHub advisory database~\cite{githubReview}.
% \xueqing{replace reference inproceedings with misc}.
% \xueqing{Add citation to show that NVD or GitHub advisory packages are verified}.
Nevertheless, manual validation requires high manual efforts~\cite{lightxml,vullibminer}, which underscores the need for automatic automatically identification. 





Existing work on vulnerable package identification~\cite{fastxml, viem, lightxml, chronos, vullibminer} focuses on the ranking approach, i.e., given the description as the query, rank the most similar package name from an existing list of package names of the corresponding ecosystem (e.g., PyPI, Maven). Since the ranking approach requires one to compute the similarity with each package, the inference cost is linear to the number of candidate package names. Due to the large number of candidate packages in software ecosystems (e.g, Java has 435k packages), existing approaches only resort to relatively smaller models such as non-neural-network models~\cite{fastxml}, logistic regression~\cite{zestxml,chronos}, or BERT~\cite{lightxml,vullibminer}. Without leveraging larger models, they typically suffer from low accuracies. 


% However, these approaches face the scalability problem due to the large number of third-party packages (e.g., more than 500 thousand).
% Now that it is time-consuming to correlate each package with a given vulnerability description, a large portion of existing approaches use only lightweight models, such as FastXML~\cite{fastxml} and ZestXML~\cite{chronos} to rank these packages, thus leading to low accuracies.
% Although other approaches~\cite{vullibminer} adopt reranking models after the lightweight ranking model, the number of candidate packages (e.g., 512) still leads to a heavy burden of time and computation resources, especially when adopting large language models (LLMs).

% Specifically, both of these approaches are limited to their training set~\cite{fernandez2011semantically}.
% Thus, they are ineffective in identifying unseen vulnerable libraries during training.

In this paper, we investigate an alternative approach for vulnerable package identification.
% \xueqing{I named the task vulnerable package identification, please check}.
Given the description, our approach will \emph{generate}, rather than rank the package names. As a result, our approach can scale to larger models as the inference requires invoking the model only once. Nevertheless, text generation suffers from challenges such as hallucination~\cite{ji2023survey} which may affect the accuracy. To understand the feasibility of the generative approach, we first conduct a pilot study on how ChatGPT output for this task. We observe that with 42\% probability, the raw output correctly matches the ground truth. Among the incorrect outputs, 22.4\% can be fixed by matching the output with the closest existing package.
% \xueqing{Check if this statement is true}.
%(3) Among the rest incorrect names, ChatGPT captures incorrect keywords or fails to capture keywords from vulnerability descriptions due to its lack of knowledge.

% From the results of the preceding empirical study, we categorize two main challenges that lead to incorrectly generated names.
% First, LLMs lack sufficient domain knowledge of these affected libraries.
% For example, a Java package's name consists of both group IDs and artifact IDs while the group ID might be neglected in a vulnerability description.
% Therefore, LLMs need to generate the correct group ID based on their domain knowledge.
% Second, LLMs might output non-existing package names.
% Note that LLMs generate the names of affected packages from only vulnerability descriptions, so the output names might have more/fewer tokens, e.g., \CodeIn{core} or \CodeIn{framework}, which are widely used in the names of Java packages.

After observing the pilot study results, we propose the \detector{} framework for vulnerable package identification based on LLM generation. First, we leverage supervised fine-tuning and retrieval-augmented generation (RAG) to bridge the knowledge gap of LLM in the security vulnerability domain. For RAG, we leverage the fine-tuned BERT model to retrieve the top-k package names and append them to the prompt to the LLM. Second, we design a local search algorithm to match the generation result with the existing package names, so the output package must exist. 


% To address the preceding challenges, we design three techniques to address the preceding challenges.
% First, we design a retrieval augmented generation (RAG) technique that provides domain knowledge into the inputs of LLMs before generation.
% Specifically, we add the names of affected libraries generated by IR approaches as they might be similar to the targeted library names.
% Second, we design a constrained decoding algorithm during generation.
% We collect package names from ecosystems of each programming language and require the output of LLMs to include at least one of them, thus avoiding non-existing package names.
% This technique modifies the decoding layer of LLMs and can be applied to only open-source LLMs.
% Third, we design a local search algorithm after generation.
% It directly searches the closest package name for each generated name, thus also avoiding non-existing package names.
% This technique is non-intrinsic and can be applied to both commercial and open-source LLMs.


We evaluate \detector{} on four software ecosystems (Java, JS, Python, Go). First, we observe that the accuracy of \detector{} (using Vicuna and Llama 13B) significantly outperforms the ranking-based approaches~\cite{fastxml,lightxml,chronos,vullibminer}, while the inference cost is comparable. Second, our ablation studies show that supervised fine-tuning (SFT), RAG and local search all improve the accuracy of \detector{}. In particular, due to the lack of SFT, the larger ChatGPT and GPT-4 models underperform the smaller \detector{} model (using Vicuna-13B). Third, to examine \detector{}'s performance in the real-world setting, we randomly sample a subset of the vulnerability descriptions in Java and JS, use \detector{} to generate the package names, and submit the generated names to GitHub Advisory. Among the 28 submitted <vulnerability, affected package> pairs, 22 are accepted and merged. This result highlights the real-world performance of \detector{} in automatically identifying affected package names. 

% We evaluate \detector{} using four state-of-the-art/practice (SOTA) approaches (FastXML~\cite{fastxml}, LightXML~\cite{lightxml}, Chronos~\cite{chronos}, and VulLibMiner~\cite{vullibminer}) that identify vulnerable libraries on the dataset of GitHub Advisory.
% Our evaluation results show that:
% (1) \detector{} is highly effective, achieving an accuracy of 0.806 while the best of SOTA approaches achieves only 0.669.
% (2) Our RAG technique and local search algorithm can boost the effectiveness of \detector{} by 8.9\% and 3.0\% on average, respectively.
% (3) \detector{} achieves better trade-offs between efficiency and accuracy than both existing and future ranking approaches.
% (4) \detector{} brings high value to security practice. 
% We have submitted 28 pairs of <vulnerability, affected package> to GitHub advisory, and 22 of them have been accepted and merged.
% We submit 25 vulnerabilities' affected libraries to GitHub advisory and 18 of them are accepted and merged.
% (5) Although fine-tuned open-source LLMs achieve similar effectiveness with ChatGPT/GPT4, they might face the limitation of overfitting, which can be alleviated by larger open-source LLMs.\tianyu{is it necessary to keep (5)?}



% Existing approaches~\cite{fastxml, viem, lightxml, chronos, vullibminer} model this task as an information retrieval (IR) task or a classification task.
% For example, they take the description field \CodeIn{``Jenkins Mail Commander Plugin for Jenkins-ci Plugin 1.0.0 and earlier stores passwords unencryted $\dots$''} as inputs and their targeted outputs, are the field of affected libraries, e.g., \CodeIn{maven:org.jenkins-ci.plugins:mailcommander}.
% However, these approaches face the scalability problem as it is unavoidable for IR/classification approaches.
% Specifically, both of these approaches are limited to their training set~\cite{fernandez2011semantically}.
% Thus, they are ineffective in identifying unseen vulnerable libraries during training.

% To address the scalability problem, in this paper, we propose to model this task as a generation task, thus utilizing the tremendous capabilities of Large Language Models (LLMs) in comprehending vulnerability descriptions.
% Here, we collect the dataset from the reviewed reports in GitHub Advisory.
% The affected libraries in each report are submitted by library developers and users, and they are manually validated by the maintainers of GitHub Advisory.
% Therefore, the ground truth of this dataset is reliable.
% Specifically, the number of Java, JavaScript, Python, and Go vulnerabilities are 4308, 3193, 2237, and 1351, respectively.


% Before employing LLMs for this task, we conduct an empirical study on the results when directly querying ChatGPT, revealing two main categories of challenges faced by LLMs.
% First, LLMs lack sufficient domain knowledge of these affected libraries.
% For example, in CVE-2022-24197, the affected library is \CodeIn{maven:com.itextpdf:itext7-core} while its description only mentions the affected library's artifact ID \CodeIn{itext7-core}, and its group ID \CodeIn{com.itextpdf} is neglected. 
% This group ID can be complemented based on the domain knowledge that only \CodeIn{itext7-core} corresponds to only one group ID \CodeIn{com.itextpdf}.
% Second, LLMs might output non-existing library names.
% For example, in CVE-2020-2167, the affected library is \CodeIn{maven:com.openshift.jenkins:openshift-pipeline} while LLMs might change the group ID into \CodeIn{com.openshift.jenkins}, which is not an existing library.
% % \tianyu{I also consider the reason that there might exist vulnerabilities whose descriptions are incomplete. (in the following comments in the source code)
% % However, this reason might be similar to 'lack of domain knowledge'}
% % First, the information in vulnerability reports might be incomplete. 
% % For example, in CVE-2017-1000406, the affected library is \CodeIn{maven:org.opendaylight.integration:distribution-karaf} while token \CodeIn{distribution} does not occur in its description.
% % Thus, even human experts cannot identify the correct names of affected libraries.


% To address the preceding challenges, we design two categories of techniques to address the preceding challenges.
% First, we design a retrieval augmented generation (RAG) technique that provides domain knowledge into the inputs of LLMs. 
% Specifically, we add the names of affected libraries generated by IR approaches as they might be similar to the targeted library names.
% Second, we design a constrained decoding algorithm and a local search algorithm to reduce non-existing outputs.
% Specifically, the constrained decoding algorithm is more effective while the local search algorithm is non-intrinsic and can be applied in commercial LLMs, e.g., ChatGPT/GPT4.
% Both algorithms utilize the database of all library names (e.g., those in Maven or Pypi) to ensure that the output of \detector{} is an existing library name.


% We evaluate \detector{} using three state-of-the-art/practice (SOTA) approaches (LightXML~\cite{lightxml}, Chronos~\cite{chronos}, and VulLibMiner~\cite{vullibminer}) that identify vulnerable libraries on the dataset of GitHub Advisory.
% Our evaluation results show that:
% (1) \detector{} is highly effective, achieving an accuracy of 0.80 while the best of SOTA approaches achieves only 0.669.
% (2) Our RAG technique can boost the effectiveness of both ChatGPT/GPT4 and open-source LLMs by at least 12\%.
% (3) Both our constrained decoding and local search algorithms can effectively reduce incorrect/non-existing outputs by at least 5.4\%.
% (4) \detector{} brings high value to security practice. We submit 25 vulnerabilities' affected libraries to GitHub advisory and 18 of them are accepted and merged.
% (5) Although fine-tuned open-source LLMs achieve similar effectiveness with ChatGPT/GPT4, they might face the limitation of overfitting, which can be alleviated by larger open-source LLMs.


% 一个建议的intro提纲：
% 1. CVE问题的重要性（为什么需要自动预测，可以帮助及时修补？）
% 2.当前解决方案的不足（scalability）
% 3.我们提出用generation来解决scalability问题，介绍一下GitHub advisory数据集以及为什么ground truth是准确的，3.但是generation存在挑战：一个是有的example input信息不全（所以即使human expert也很难做到100%），一个是llm缺乏domain knowledge 
% 4.做一个empirical study发现input信息不全的现象只占少数。同时针对以上挑战，设计了几个方法：fine tuning，rag，constrained decoding，post processing，讨论一下它们为什么有可能解决generation的挑战。
% 5. 总结实验结果，讨论可能存在的limitation，比如fine tuning可能存在overfitting，future work如何弥补这些limitation


% To avoid potential risks posed by vulnerabilities in third-party libraries, security researchers maintain databases containing vulnerability reports, e.g., the National Vulnerability Database (NVD)~\cite{nvd}. 
% A vulnerability report in NVD includes a vulnerability's identification number in the entry of Common Vulnerability Enumeration (CVE), its description, and the name list of libraries affected by the vulnerability  (a.k.a. vulnerable libraries).
% Application developers can identify vulnerable libraries by directly querying each description and CPE entry with the name of each used library. 
% However, recent studies on about 200,000 vulnerability reports in NVD show that 53.3\% of the vulnerability reports in NVD do not mention any affected libraries~\cite{lightxml} and 59.82\% of the included vulnerable libraries are incomplete or incorrect~\cite{viem}.


% To address the preceding issue, existing approaches~\cite{viem, anwar2021cleaning, jo2022vulcan, kuehn2021ovana, fastxml, lightxml, chronos, vullibminer} fall into three main categories.
% First, named-entity-recognition (NER) approaches~\cite{viem, anwar2021cleaning, jo2022vulcan, kuehn2021ovana} use NER models to extract the mentioned library entities from vulnerability descriptions, and then match these entities with a dictionary of library names.
% Second, extreme multi-label learning (XML) approaches~\cite{fastxml, lightxml, chronos} use deep-learning classification models to assign a set of labels (i.e., vulnerable libraries) to a given vulnerability by training on labeled datasets.
% Third, entity-linking approaches~\cite{vullibminer} take library descriptions as inputs besides the description of a given vulnerability, thus achieving higher accuracy than NER and XML approaches.

% Although existing approaches make efforts to identify vulnerable libraries, they still suffer from highly inaccurate results.
% Existing NER and XML approaches cannot distinguish vulnerable libraries with similar names, such as ``org.jenkins-ci.plugins:mailer'' and ``org.jenkins-ci.plugins:mailcommander''.
% However, these libraries are not affected together by one vulnerability due to their different functionalities and scopes.
% Existing entity-linking approaches use TF-IDF techniques to reduce the number of libraries for comparison, and yet suffer from false negatives (i.e., some vulnerable libraries are missed) and thus low accuracy.
% Considering the large number of collected libraries (e.g., 310,844 in Maven) for comparison compared, this step cannot be avoided; otherwise, it might cost them two years to identify all vulnerable libraries~\cite{vullibminer}.




% To overcome the preceding limitations, we propose \detector{}, the first generative approach to generate the affected libraries of a given vulnerability.
% \detector{} is effective to generate the name list of vulnerable libraries (out of all the existing libraries) by utilizing the recent enormous advances in Large Language Models (LLMs) with two stages of fine-tuning.
% The rationale behind this step is that LLMs can correlate the input vulnerability description to vulnerable libraries based on their prior knowledge of these libraries, e.g., their functionalities, usages, and even history issues.
% With prior knowledge, \detector{} avoids the high cost of correlating one vulnerability description with each library.
% Specifically, we conduct unsupervised fine-tuning on maven~\cite{maven} corpus to fine-tune raw LLaMa models to activate their prior knowledge of Java libraries.
% The input of this stage is one library's description, and its targeted output is its library name.
% Then, we conduct supervised fine-tuning on labeled datasets to enhance the ability to identify vulnerable libraries.
% The input of this stage is a vulnerability description and its targeted output is a name list of vulnerable libraries affected by this vulnerability.

% Since we use fine-tuned LLMs to generate the affected library names of a given vulnerability, there are two main challenges that decrease LLMs' effectiveness.
% First, LLMs face the difficulty of low accuracy when identifying zero-shot libraries because they have no prior knowledge of how these libraries are affected by vulnerabilities.
% Similar to XML approaches, LLMs tend to output incorrect libraries that have already been affected by other vulnerabilities during training and fine-tuning.
% Second, LLMs face hallucinations, i.e., generating plausible-looking library names that are non-existing.
% For example, they might mix up two similar library names and lack part of the library names.



% To address the preceding challenges, we design two specialized techniques during supervised fine-tuning to improve the effectiveness by addressing the preceding challenges.
% To help identify zero-shot libraries, we design an input augmentation technique, which feeds the names of vulnerable libraries (a.k.a., recommended libraries) identified by the SOTA approach~\cite{vullibminer} to \detector{} as input.
% This technique provides examples of libraries whose functionalities are likely to be affected by a given vulnerability.
% Thus, \detector{} can generate library names from those with similar functionalities instead of all libraries when \detector{} has no prior knowledge of how these zero-shot libraries are affected by vulnerabilities.
% To address \detector{}'s hallucinations, we design our post-processing technique based on the Levenshtein distance~\cite{levenshtein} to obtain existing Java library names from the response of LLMs.
% We find that \detector{} can generate the components of the targeted library names (i.e., the targeted functionalities and scopes), and make mistakes when jointing these components of library names, thus leading to hallucinations.
% Therefore, hallucination library names are close to the targeted names of vulnerable libraries, and their closest library names tend to be the targeted names.


% We evaluate \detector{} using three state-of-the-art/practice approaches (LightXML~\cite{lightxml}, Chronos~\cite{chronos}, and VulLibMiner~\cite{vullibminer}) that identify vulnerable libraries on an open-source dataset (VulLib)~\cite{vullib}.
% Our evaluation results show a number of findings to demonstrate our \detector{} approach’s effectiveness and efficiency.
% Given the ground truth score of 0.840, \detector{} effectively achieves the F1@1 score of 0.626 while the state-of-the-art/practice (SOTA) approaches achieve only 0.561.
% Specifically, the post-processing technique helps \detector{} achieve an average improvement of F1@1 by 9.3\%, and the input augmentation technique helps \detector{} achieve an average improvement of F1@1 by 39\% in identifying zero-shot libraries.
% Additionally, \detector{} is highly efficient, identifying one vulnerability in less than 6 seconds.


% In summary, this paper makes the following main contributions:
% \begin{itemize}
% \item  We propose, \detector{}, the first generative approach for identifying vulnerable libraries via Large Language Models.
% \item  We design an input augmentation technique and a post-processing technique to help identify zero-shot libraries and help address hallucinations.
% \item  We conduct a comprehensive evaluation demonstrating the effectiveness and efficiency of \detector{}, increasing the F1@1 of 0.626 while the state-of-the-art/practice (SOTA) approaches achieve only 0.561.
% \end{itemize}



==> backup/intro-backup-2.tex <==
\begin{figure}[h]
\centering
\includegraphics[width=1\linewidth]{figures/vulnerability-report.drawio.pdf}
\caption{GitHub Advisory Report for \href{https://github.com/advisories/GHSA-485q-v457-3p58}{CVE-2020-2318}}
\label{fig: case}
\end{figure}

\section{Introduction}~\label{sec:intro}
With the increasing usage of third-party software packages, their security vulnerabilities pose great challenges to software and network systems.
A recent study~\cite{wang2020empirical} shows that 84\% third-party packages contain vulnerabilities and 60\% of them are high-risk ones.
To avoid potential risks posed by these vulnerabilities, security practitioners maintain vulnerability databases for reference, e.g., the National Vulnerability Database (NVD)~\cite{nvd} and GitHub Advisory~\cite{githubAD}.
These databases help developers realize and deploy vulnerability patches.
Figure~\ref{fig: case} shows an example report of one vulnerability, \href{https://github.com/advisories/GHSA-485q-v457-3p58}{CVE-2020-2318}.
The vulnerability's affected packages include  \CodeIn{org.jenkins-ci.plugins:mailcommander} and its corresponding versions.
The field of affected packages is specified by the developers who create this CVE. However, recent studies~\cite{lightxml,viem} show that in more than half of vulnerability reports, this field is missing or incorrect.
To alleviate this problem, human maintainers manually complete or validate the affected-package information in databases such as GitHub Advisory~\cite{githubReview}.
However, manual completion or validation requires high manual efforts~\cite{lightxml,vullibminer}, underscoring the need for automatic identification. 



Existing work suffers from low accuracy due to two factors. First, most existing work uses s

Existing work on automatic identification of vulnerable packages~\cite{fastxml, viem, lightxml, chronos, vullibminer} propose  ranking approaches\footnote{\xueqing{classification which can be seen as ranking approach}} that,  given the vulnerability description as the query, rank the most similar package name from an existing list of package names of the corresponding ecosystem (e.g., PyPI, Maven). Since a ranking approach requires one to compute the description's similarity with each package, the time cost is typically large, e.g., Java has 435k packages. To the best of our knowledge, most existing approaches focus on relatively smaller models such as non-neural-network models~\cite{fastxml}, logistic regression~\cite{zestxml,chronos}, or BERT~\cite{lightxml,vullibminer}. Without leveraging larger models, they typically suffer from low accuracies. 


To address the low accuracy issue, in this paper, we propose to first leverage large language models (i.e., 7B models and larger) for vulnerable package identification. Given the description, our approach will \emph{generate}, rather than rank the package names. As a result, our approach can scale to larger models since this approach requires invoking the model inference only once. However, it is unclear whether the generative approach is effective for this task. On the one hand, the description often does not include the full information about the package name (Section~\ref{sec: empirical_study}); on the other hand, the task requires the generated package name to exactly match the ground truth and previous work finds this to be challenging for LLMs~\cite{liu2023codegen4libs}. To understand the potential of the generative approach, we conduct a pilot study on the errors made by ChatGPT raw output for this task. The study shows that ChatGPT raw output has a reasonable accuracy; however, for some vulnerabilities, ChatGPT lacks the domain knowledge for generation; for other vulnerabilities, the generated package names do not exist. 
Based on the study results, we propose the following \detector{} framework. First, we leverage supervised fine-tuning, in-context learning, and retrieval-augmented generation (RAG) to bridge the knowledge gap of LLM in the security vulnerability domain. For RAG, we leverage the fine-tuned BERT model to retrieve the top-k package names and append them to the prompt to the LLM. Second, we design a local search algorithm to match the generation result with the existing package names, so the output package must exist. 



We evaluate \detector{} on four software ecosystems (Java, JS, Python, Go). First, we observe that the accuracy of \detector{} (using Vicuna and Llama 13B) significantly outperforms the ranking-based approaches~\cite{fastxml,lightxml,chronos,vullibminer} and the computational time cost is comparable. In particular, \detector{} using Vicuna-13B outperforms the larger ChatGPT and GPT-4 models by employing SFT. Second, our ablation studies show that supervised fine-tuning (SFT), RAG and local search all improve the accuracy of \detector{}. Third, to examine \detector{}'s performance in the real-world setting, we randomly sample a subset of the vulnerability descriptions in Java and JS, use \detector{} to generate the package names, and submit the generated names to GitHub Advisory. Among the 28 submitted <vulnerability, affected package> pairs, 22 are accepted and merged. This result highlights the real-world performance of \detector{} in automatically generating the names of affected packages. 


==> backup/intro-backup-3.tex <==
\begin{figure}[h]
\centering
\includegraphics[width=1\linewidth]{figures/vulnerability-report.drawio.pdf}
\caption{GitHub Advisory Report for \href{https://github.com/advisories/GHSA-485q-v457-3p58}{CVE-2020-2318}}
\label{fig: case}
\end{figure}

\section{Introduction}~\label{sec:intro}
With the increasing usage of third-party software packages, their security vulnerabilities pose great challenges to software and network systems.
A recent study~\cite{wang2020empirical} shows that 84\% third-party packages contain vulnerabilities and 60\% of them are high-risk ones.
To avoid potential risks posed by these vulnerabilities, security practitioners maintain vulnerability databases for reference, e.g., the National Vulnerability Database (NVD)~\cite{nvd} and GitHub Advisory~\cite{githubAD}.
These databases help developers realize and deploy vulnerability patches.
Figure~\ref{fig: case} shows an example report of one vulnerability, \href{https://github.com/advisories/GHSA-485q-v457-3p58}{CVE-2020-2318}.
The vulnerability's affected packages include  \CodeIn{org.jenkins-ci.plugins:mailcommander} and its corresponding versions.
The field of affected packages is specified by the developers who create this CVE. However, recent studies~\cite{lightxml,viem} show that in more than half of vulnerability reports, this field is missing or incorrect.
% \xueqing{can we say the package information is incorrect?}
% \tianyu{I think it's better not to mention incorrect, otherwise, our ground truth of labels might be challenged.}
To alleviate this problem, human maintainers manually complete or validate the affected-package information in databases such as GitHub Advisory~\cite{githubReview}.
% \xueqing{replace reference inproceedings with misc}.
% \xueqing{Add citation to show that NVD or GitHub advisory packages are verified}.
However, manual completion or validation requires high manual efforts~\cite{lightxml,vullibminer}, underscoring the need for automatic identification. 

% \xueqing{Explain how is smaller model used -> low accuracy -> leverage LLM's potential, LLM will keep improving-> if we use it the same way as smaller models, cost is high -> to leverage LLM wo high cost, propose the generative approach}

Existing work on automatic identification of vulnerable packages~\cite{fastxml, viem, lightxml, chronos, vullibminer} suffers from lower accuracies while requiring a linear time cost to the number of packages~\cite{chronos,vullibminer}. The reason for the lower accuracies is partly because existing work only investigates approaches using smaller models such as logistic regression and BERT~\cite{fastxml,zestxml,chronos,lightxml,vullibminer}. Regarding the time cost, given a vulnerability description (Figure~\ref{fig: case}), existing work computes a similarity score between the vulnerability description and each package's text description from the ecosystem (e.g., PyPI, Maven), and then they rank all package based on this score. As a result, the time cost for identifying each vulnerability = the number of candidate packages $\times$ the cost of each model inference (e.g., BERT). 

To improve the accuracy of vulnerable package identification, we investigate the potential of large language models (LLMs). In particular, we propose a framework \detector{} which uses LLMs to \emph{generate} instead of rank the affected package names. When using LLMs, we cannot directly adopt previous work's ranking approach, since the number of candidate packages (e.g., Java has 435k packages) and the inference cost of LLMs are both high. In contrast, the generative approach invokes the model inference only once.

To improve the accuracy of the generation, \detector{} aims to address two issues with the generative approach. First, the LLM may lack the domain knowledge required to generate the target package. The reason is that the LLM's input vulnerability description often does not contain the full information of the package name, it thus requires the LLM to infer the missing information from the domain knowledge. Second, a previous study shows that the LLM may generate package names that do not exist. 

To address the preceding issues, our approach leverages the following techniques. First, to enhance the domain knowledge of LLMs, we employ supervised fine-tuning, in-context learning, and retrieval-augmented generation (RAG). Second, to ensure the generated package exists, we propose a post-processing algorithm to match the generation output with the closest existing package name. Our algorithm design is based on an empirical study of the errors of the raw output of ChatGPT. 

% Existing work on automatic identification of vulnerable packages~\cite{fastxml, viem, lightxml, chronos, vullibminer} propose  ranking approaches\footnote{\xueqing{classification which can be seen as ranking approach}} that,  given the vulnerability description as the query, rank the most similar package name from an existing list of package names of the corresponding ecosystem (e.g., PyPI, Maven). Since a ranking approach requires one to compute the description's similarity with each package, the time cost is typically large, e.g., Java has 435k packages. To the best of our knowledge, most existing approaches focus on relatively smaller models such as non-neural-network models~\cite{fastxml}, logistic regression~\cite{zestxml,chronos}, or BERT~\cite{lightxml,vullibminer}. Without leveraging larger models, they typically suffer from low accuracies. 


% However, these approaches face the scalability problem due to the large number of third-party packages (e.g., more than 500 thousand).
% Now that it is time-consuming to correlate each package with a given vulnerability description, a large portion of existing approaches use only lightweight models, such as FastXML~\cite{fastxml} and ZestXML~\cite{chronos} to rank these packages, thus leading to low accuracies.
% Although other approaches~\cite{vullibminer} adopt reranking models after the lightweight ranking model, the number of candidate packages (e.g., 512) still leads to a heavy burden of time and computation resources, especially when adopting large language models (LLMs).

% Specifically, both of these approaches are limited to their training set~\cite{fernandez2011semantically}.
% Thus, they are ineffective in identifying unseen vulnerable libraries during training.

% To address the low accuracy issue, in this paper, we propose to first leverage large language models (i.e., 7B models and larger) for vulnerable package identification. Given the description, our approach will \emph{generate}, rather than rank the package names. As a result, our approach can scale to larger models since this approach requires invoking the model inference only once. However, it is unclear whether the generative approach is effective for this task. On the one hand, the description often does not include the full information about the package name (Section~\ref{sec: empirical_study}); on the other hand, the task requires the generated package name to exactly match the ground truth and previous work finds this to be challenging for LLMs~\cite{liu2023codegen4libs}. To understand the potential of the generative approach, we conduct a pilot study on the errors made by ChatGPT raw output for this task. The study shows that ChatGPT raw output has a reasonable accuracy; however, for some vulnerabilities, ChatGPT lacks the domain knowledge for generation; for other vulnerabilities, the generated package names do not exist. 
%Based on the study results,
% \xueqing{I named the task vulnerable package identification, please check}.
% Nevertheless, text generation suffers from challenges such as hallucination~\cite{ji2023survey} which may affect the accuracy. To understand the feasibility of the generative approach, we first conduct a pilot study on how ChatGPT output for this task. We observe that with 42\% probability, the raw output correctly matches the ground truth. Among the incorrect outputs, 22.4\% can be fixed by matching the output with the closest existing package.
% \xueqing{Check if this statement is true}.
%(3) Among the rest incorrect names, ChatGPT captures incorrect keywords or fails to capture keywords from vulnerability descriptions due to its lack of knowledge.
% From the results of the preceding empirical study, we categorize two main challenges that lead to incorrectly generated names.
% First, LLMs lack sufficient domain knowledge of these affected libraries.
% For example, a Java package's name consists of both group IDs and artifact IDs while the group ID might be neglected in a vulnerability description.
% Therefore, LLMs need to generate the correct group ID based on their domain knowledge.
% Second, LLMs might output non-existing package names.
% Note that LLMs generate the names of affected packages from only vulnerability descriptions, so the output names might have more/fewer tokens, e.g., \CodeIn{core} or \CodeIn{framework}, which are widely used in the names of Java packages.



% To address the preceding challenges, we design three techniques to address the preceding challenges.
% First, we design a retrieval augmented generation (RAG) technique that provides domain knowledge into the inputs of LLMs before generation.
% Specifically, we add the names of affected libraries generated by IR approaches as they might be similar to the targeted library names.
% Second, we design a constrained decoding algorithm during generation.
% We collect package names from ecosystems of each programming language and require the output of LLMs to include at least one of them, thus avoiding non-existing package names.
% This technique modifies the decoding layer of LLMs and can be applied to only open-source LLMs.
% Third, we design a local search algorithm after generation.
% It directly searches the closest package name for each generated name, thus also avoiding non-existing package names.
% This technique is non-intrinsic and can be applied to both commercial and open-source LLMs.


Our evaluation of \detector{} shows three main findings. First, we observe that the accuracy of \detector{} significantly outperforms existing approaches~\cite{fastxml,lightxml,chronos,vullibminer} and the computational time cost is comparable. In particular, \detector{} using Vicuna-13B outperforms the larger ChatGPT and GPT-4 models by employing supervised fine-tuning (SFT). Second, our ablation studies show that SFT, RAG and local search all improve the accuracy of \detector{}. Third, \detector{} provides high value to security practice: we have submitted 28 pairs of <vulnerability, generated affected package> to GitHub Advisory, 22 of them are accepted and merged. 

% To examine \detector{}'s performance in the real-world setting, we further randomly sample a subset of the vulnerability descriptions in Java and JS, use \detector{} to generate the package names, and submit the generated names to GitHub Advisory. Among the 28 submitted <vulnerability, affected package> pairs, 22 are accepted and merged. This result highlights the real-world performance of \detector{} in automatically generating the names of affected packages. 

% We evaluate \detector{} using four state-of-the-art/practice (SOTA) approaches (FastXML~\cite{fastxml}, LightXML~\cite{lightxml}, Chronos~\cite{chronos}, and VulLibMiner~\cite{vullibminer}) that identify vulnerable libraries on the dataset of GitHub Advisory.
% Our evaluation results show that:
% (1) \detector{} is highly effective, achieving an accuracy of 0.806 while the best of SOTA approaches achieves only 0.669.
% (2) Our RAG technique and local search algorithm can boost the effectiveness of \detector{} by 8.9\% and 3.0\% on average, respectively.
% (3) \detector{} achieves better trade-offs between efficiency and accuracy than both existing and future ranking approaches.
% (4) \detector{} brings high value to security practice. 
% We have submitted 28 pairs of <vulnerability, affected package> to GitHub advisory, and 22 of them have been accepted and merged.
% We submit 25 vulnerabilities' affected libraries to GitHub advisory and 18 of them are accepted and merged.
% (5) Although fine-tuned open-source LLMs achieve similar effectiveness with ChatGPT/GPT4, they might face the limitation of overfitting, which can be alleviated by larger open-source LLMs.\tianyu{is it necessary to keep (5)?}



% Existing approaches~\cite{fastxml, viem, lightxml, chronos, vullibminer} model this task as an information retrieval (IR) task or a classification task.
% For example, they take the description field \CodeIn{``Jenkins Mail Commander Plugin for Jenkins-ci Plugin 1.0.0 and earlier stores passwords unencryted $\dots$''} as inputs and their targeted outputs, are the field of affected libraries, e.g., \CodeIn{maven:org.jenkins-ci.plugins:mailcommander}.
% However, these approaches face the scalability problem as it is unavoidable for IR/classification approaches.
% Specifically, both of these approaches are limited to their training set~\cite{fernandez2011semantically}.
% Thus, they are ineffective in identifying unseen vulnerable libraries during training.

% To address the scalability problem, in this paper, we propose to model this task as a generation task, thus utilizing the tremendous capabilities of Large Language Models (LLMs) in comprehending vulnerability descriptions.
% Here, we collect the dataset from the reviewed reports in GitHub Advisory.
% The affected libraries in each report are submitted by library developers and users, and they are manually validated by the maintainers of GitHub Advisory.
% Therefore, the ground truth of this dataset is reliable.
% Specifically, the number of Java, JavaScript, Python, and Go vulnerabilities are 4308, 3193, 2237, and 1351, respectively.


% Before employing LLMs for this task, we conduct an empirical study on the results when directly querying ChatGPT, revealing two main categories of challenges faced by LLMs.
% First, LLMs lack sufficient domain knowledge of these affected libraries.
% For example, in CVE-2022-24197, the affected library is \CodeIn{maven:com.itextpdf:itext7-core} while its description only mentions the affected library's artifact ID \CodeIn{itext7-core}, and its group ID \CodeIn{com.itextpdf} is neglected. 
% This group ID can be complemented based on the domain knowledge that only \CodeIn{itext7-core} corresponds to only one group ID \CodeIn{com.itextpdf}.
% Second, LLMs might output non-existing library names.
% For example, in CVE-2020-2167, the affected library is \CodeIn{maven:com.openshift.jenkins:openshift-pipeline} while LLMs might change the group ID into \CodeIn{com.openshift.jenkins}, which is not an existing library.
% % \tianyu{I also consider the reason that there might exist vulnerabilities whose descriptions are incomplete. (in the following comments in the source code)
% % However, this reason might be similar to 'lack of domain knowledge'}
% % First, the information in vulnerability reports might be incomplete. 
% % For example, in CVE-2017-1000406, the affected library is \CodeIn{maven:org.opendaylight.integration:distribution-karaf} while token \CodeIn{distribution} does not occur in its description.
% % Thus, even human experts cannot identify the correct names of affected libraries.


% To address the preceding challenges, we design two categories of techniques to address the preceding challenges.
% First, we design a retrieval augmented generation (RAG) technique that provides domain knowledge into the inputs of LLMs. 
% Specifically, we add the names of affected libraries generated by IR approaches as they might be similar to the targeted library names.
% Second, we design a constrained decoding algorithm and a local search algorithm to reduce non-existing outputs.
% Specifically, the constrained decoding algorithm is more effective while the local search algorithm is non-intrinsic and can be applied in commercial LLMs, e.g., ChatGPT/GPT4.
% Both algorithms utilize the database of all library names (e.g., those in Maven or Pypi) to ensure that the output of \detector{} is an existing library name.


% We evaluate \detector{} using three state-of-the-art/practice (SOTA) approaches (LightXML~\cite{lightxml}, Chronos~\cite{chronos}, and VulLibMiner~\cite{vullibminer}) that identify vulnerable libraries on the dataset of GitHub Advisory.
% Our evaluation results show that:
% (1) \detector{} is highly effective, achieving an accuracy of 0.80 while the best of SOTA approaches achieves only 0.669.
% (2) Our RAG technique can boost the effectiveness of both ChatGPT/GPT4 and open-source LLMs by at least 12\%.
% (3) Both our constrained decoding and local search algorithms can effectively reduce incorrect/non-existing outputs by at least 5.4\%.
% (4) \detector{} brings high value to security practice. We submit 25 vulnerabilities' affected libraries to GitHub advisory and 18 of them are accepted and merged.
% (5) Although fine-tuned open-source LLMs achieve similar effectiveness with ChatGPT/GPT4, they might face the limitation of overfitting, which can be alleviated by larger open-source LLMs.


% 一个建议的intro提纲：
% 1. CVE问题的重要性（为什么需要自动预测，可以帮助及时修补？）
% 2.当前解决方案的不足（scalability）
% 3.我们提出用generation来解决scalability问题，介绍一下GitHub advisory数据集以及为什么ground truth是准确的，3.但是generation存在挑战：一个是有的example input信息不全（所以即使human expert也很难做到100%），一个是llm缺乏domain knowledge 
% 4.做一个empirical study发现input信息不全的现象只占少数。同时针对以上挑战，设计了几个方法：fine tuning，rag，constrained decoding，post processing，讨论一下它们为什么有可能解决generation的挑战。
% 5. 总结实验结果，讨论可能存在的limitation，比如fine tuning可能存在overfitting，future work如何弥补这些limitation


% To avoid potential risks posed by vulnerabilities in third-party libraries, security researchers maintain databases containing vulnerability reports, e.g., the National Vulnerability Database (NVD)~\cite{nvd}. 
% A vulnerability report in NVD includes a vulnerability's identification number in the entry of Common Vulnerability Enumeration (CVE), its description, and the name list of libraries affected by the vulnerability  (a.k.a. vulnerable libraries).
% Application developers can identify vulnerable libraries by directly querying each description and CPE entry with the name of each used library. 
% However, recent studies on about 200,000 vulnerability reports in NVD show that 53.3\% of the vulnerability reports in NVD do not mention any affected libraries~\cite{lightxml} and 59.82\% of the included vulnerable libraries are incomplete or incorrect~\cite{viem}.


% To address the preceding issue, existing approaches~\cite{viem, anwar2021cleaning, jo2022vulcan, kuehn2021ovana, fastxml, lightxml, chronos, vullibminer} fall into three main categories.
% First, named-entity-recognition (NER) approaches~\cite{viem, anwar2021cleaning, jo2022vulcan, kuehn2021ovana} use NER models to extract the mentioned library entities from vulnerability descriptions, and then match these entities with a dictionary of library names.
% Second, extreme multi-label learning (XML) approaches~\cite{fastxml, lightxml, chronos} use deep-learning classification models to assign a set of labels (i.e., vulnerable libraries) to a given vulnerability by training on labeled datasets.
% Third, entity-linking approaches~\cite{vullibminer} take library descriptions as inputs besides the description of a given vulnerability, thus achieving higher accuracy than NER and XML approaches.

% Although existing approaches make efforts to identify vulnerable libraries, they still suffer from highly inaccurate results.
% Existing NER and XML approaches cannot distinguish vulnerable libraries with similar names, such as ``org.jenkins-ci.plugins:mailer'' and ``org.jenkins-ci.plugins:mailcommander''.
% However, these libraries are not affected together by one vulnerability due to their different functionalities and scopes.
% Existing entity-linking approaches use TF-IDF techniques to reduce the number of libraries for comparison, and yet suffer from false negatives (i.e., some vulnerable libraries are missed) and thus low accuracy.
% Considering the large number of collected libraries (e.g., 310,844 in Maven) for comparison compared, this step cannot be avoided; otherwise, it might cost them two years to identify all vulnerable libraries~\cite{vullibminer}.




% To overcome the preceding limitations, we propose \detector{}, the first generative approach to generate the affected libraries of a given vulnerability.
% \detector{} is effective to generate the name list of vulnerable libraries (out of all the existing libraries) by utilizing the recent enormous advances in Large Language Models (LLMs) with two stages of fine-tuning.
% The rationale behind this step is that LLMs can correlate the input vulnerability description to vulnerable libraries based on their prior knowledge of these libraries, e.g., their functionalities, usages, and even history issues.
% With prior knowledge, \detector{} avoids the high cost of correlating one vulnerability description with each library.
% Specifically, we conduct unsupervised fine-tuning on maven~\cite{maven} corpus to fine-tune raw LLaMa models to activate their prior knowledge of Java libraries.
% The input of this stage is one library's description, and its targeted output is its library name.
% Then, we conduct supervised fine-tuning on labeled datasets to enhance the ability to identify vulnerable libraries.
% The input of this stage is a vulnerability description and its targeted output is a name list of vulnerable libraries affected by this vulnerability.

% Since we use fine-tuned LLMs to generate the affected library names of a given vulnerability, there are two main challenges that decrease LLMs' effectiveness.
% First, LLMs face the difficulty of low accuracy when identifying zero-shot libraries because they have no prior knowledge of how these libraries are affected by vulnerabilities.
% Similar to XML approaches, LLMs tend to output incorrect libraries that have already been affected by other vulnerabilities during training and fine-tuning.
% Second, LLMs face hallucinations, i.e., generating plausible-looking library names that are non-existing.
% For example, they might mix up two similar library names and lack part of the library names.



% To address the preceding challenges, we design two specialized techniques during supervised fine-tuning to improve the effectiveness by addressing the preceding challenges.
% To help identify zero-shot libraries, we design an input augmentation technique, which feeds the names of vulnerable libraries (a.k.a., recommended libraries) identified by the SOTA approach~\cite{vullibminer} to \detector{} as input.
% This technique provides examples of libraries whose functionalities are likely to be affected by a given vulnerability.
% Thus, \detector{} can generate library names from those with similar functionalities instead of all libraries when \detector{} has no prior knowledge of how these zero-shot libraries are affected by vulnerabilities.
% To address \detector{}'s hallucinations, we design our post-processing technique based on the Levenshtein distance~\cite{levenshtein} to obtain existing Java library names from the response of LLMs.
% We find that \detector{} can generate the components of the targeted library names (i.e., the targeted functionalities and scopes), and make mistakes when jointing these components of library names, thus leading to hallucinations.
% Therefore, hallucination library names are close to the targeted names of vulnerable libraries, and their closest library names tend to be the targeted names.


% We evaluate \detector{} using three state-of-the-art/practice approaches (LightXML~\cite{lightxml}, Chronos~\cite{chronos}, and VulLibMiner~\cite{vullibminer}) that identify vulnerable libraries on an open-source dataset (VulLib)~\cite{vullib}.
% Our evaluation results show a number of findings to demonstrate our \detector{} approach’s effectiveness and efficiency.
% Given the ground truth score of 0.840, \detector{} effectively achieves the F1@1 score of 0.626 while the state-of-the-art/practice (SOTA) approaches achieve only 0.561.
% Specifically, the post-processing technique helps \detector{} achieve an average improvement of F1@1 by 9.3\%, and the input augmentation technique helps \detector{} achieve an average improvement of F1@1 by 39\% in identifying zero-shot libraries.
% Additionally, \detector{} is highly efficient, identifying one vulnerability in less than 6 seconds.


% In summary, this paper makes the following main contributions:
% \begin{itemize}
% \item  We propose, \detector{}, the first generative approach for identifying vulnerable libraries via Large Language Models.
% \item  We design an input augmentation technique and a post-processing technique to help identify zero-shot libraries and help address hallucinations.
% \item  We conduct a comprehensive evaluation demonstrating the effectiveness and efficiency of \detector{}, increasing the F1@1 of 0.626 while the state-of-the-art/practice (SOTA) approaches achieve only 0.561.
% \end{itemize}



==> backup/intro-backup-5.tex <==
\begin{figure}[h]
\centering
\includegraphics[width=1\linewidth]{figures/vulnerability-report.drawio.pdf}
\caption{GitHub Advisory Report for \href{https://github.com/advisories/GHSA-485q-v457-3p58}{CVE-2020-2318}}
\label{fig: case}
\end{figure}

\section{Introduction}~\label{sec:intro}
With the increasing usage of third-party software packages, their security vulnerabilities pose great challenges to software and network systems.
A recent study~\cite{wang2020empirical} shows that 84\% third-party packages contain vulnerabilities and 60\% of them are high-risk ones.
To avoid potential risks posed by these vulnerabilities, security practitioners maintain vulnerability databases for reference, e.g., the National Vulnerability Database (NVD)~\cite{nvd} and GitHub Advisory~\cite{githubAD}.
These databases help developers realize and deploy vulnerability patches.
Figure~\ref{fig: case} shows an example report of one vulnerability, \href{https://github.com/advisories/GHSA-485q-v457-3p58}{CVE-2020-2318}.
The vulnerability's affected packages include  \CodeIn{org.jenkins-ci.plugins:mailcommander} and its corresponding versions.
The field of affected packages is specified by the developers who create this CVE. However, recent studies~\cite{lightxml,viem} show that in more than half of vulnerability reports, this field is missing or incorrect.
% \xueqing{can we say the package information is incorrect?}
% \tianyu{I think it's better not to mention incorrect, otherwise, our ground truth of labels might be challenged.}
To alleviate this problem, human maintainers manually complete or validate the affected-package information in databases such as GitHub Advisory~\cite{githubReview}.
% \xueqing{replace reference inproceedings with misc}.
% \xueqing{Add citation to show that NVD or GitHub advisory packages are verified}.
However, manual completion or validation requires high manual efforts~\cite{lightxml,vullibminer}, underscoring the need for automatic identification. 

% \xueqing{Explain how is smaller model used -> low accuracy -> leverage LLM's potential, LLM will keep improving-> if we use it the same way as smaller models, cost is high -> to leverage LLM wo high cost, propose the generative approach}

Existing work on automatic identification of vulnerable packages~\cite{fastxml, viem, lightxml, chronos, vullibminer} suffers from two limitations related to time cost and accuracy, respectively.  %lower accuracies while requiring a linear time cost with respect to the number of packages~\cite{chronos,vullibminer}. 
First, existing work has a linear time cost to the number of packages (e.g., 435k Java packages)~\cite{chronos,vullibminer}. 
Given a vulnerability description (Figure~\ref{fig: case}), existing work computes a similarity score between the vulnerability description and each package's text description from the ecosystem (e.g., PyPI, Maven), and then they rank all packages based on this score. As a result, the time cost for identifying each vulnerability = the number of candidate packages $\times$ the cost of each model inference (e.g., BERT). 
Second, existing work suffers from lower accuracies due to their time cost, which requires them to investigate approaches using smaller models such as logistic regression and BERT~\cite{fastxml,zestxml,chronos,lightxml,vullibminer}. 
% Second, regarding the time cost, given a vulnerability description (Figure~\ref{fig: case}), existing work requires to compute a similarity score between the vulnerability description and each package's text description from the ecosystem (e.g., PyPI, Maven), then they rank all package based on this score. As a result, the time cost for identifying each vulnerability = the number of candidate packages $\times$ the cost of each model inference (e.g., BERT). 

\tianyu{not completely structural}
To improve the time cost and accuracy of identifying vulnerable packages, we investigate the potential of large language models (LLMs). In particular, we propose a framework \detector{} which uses LLMs to \emph{generate} instead of ranking the names of affected packages. 
Our rationale for not following previous work's ranking approaches is that the number of packages (e.g., Java has 435k packages) brings high costs to rank the similarity scores between a vulnerability and each package.
In contrast, the generative approach invokes the model inference only once.
% When using LLMs, we cannot directly adopt previous work's ranking approach, since the number of candidate packages (e.g., Java has 435k packages) and the inference cost of LLMs are both high. In contrast, the generative approach invokes the model inference only once.

Specifically, \detector{} includes two techniques to address two main challenges of generating the names of affected packages.
First, we employ supervised fine-tuning, in-context learning, and retrieval-augmented generation (RAG) to enhance the domain knowledge of LLMs as LLMs may lack the domain knowledge required to generate the target package.
The reason is that the LLM's input vulnerability description often does not contain the full information of the package name, it thus requires the LLM to infer the missing information from the domain knowledge. 
Second, we propose a local search technique to ensure the generated package exists.
The reason is that recent studies~\cite{vazquez2023javascript} show that LLMs may generate package names that do not exist. 
Based on an empirical study of the errors of the raw output of ChatGPT, we design our local search technique that matches the generation output with the closest existing package name, thus avoiding non-existing package names.

% Second, to ensure the generated package exists, we propose a post-processing algorithm to match the generation output with the closest existing package name. Our algorithm design is based on an empirical study of the errors of the raw output of ChatGPT. 


% To address the preceding challenges, \detector{} includes two techniques. First, to enhance the domain knowledge of LLMs, we employ supervised fine-tuning, in-context learning, and retrieval-augmented generation (RAG). Second, to ensure the generated package exists, we propose a post-processing algorithm to match the generation output with the closest existing package name. Our algorithm design is based on an empirical study of the errors of the raw output of ChatGPT. 

% To improve the accuracy of the generation, \detector{} aims to address two issues with the generative approach. First, the LLM may lack the domain knowledge required to generate the target package. The reason is that the LLM's input vulnerability description often does not contain the full information of the package name, it thus requires the LLM to infer the missing information from the domain knowledge. Second, a previous study shows that the LLM may generate package names that do not exist. 

% To address the preceding issues, our approach includes two techniques. First, to enhance the domain knowledge of LLMs, we employ supervised fine-tuning, in-context learning, and retrieval-augmented generation (RAG). Second, to ensure the generated package exists, we propose a post-processing algorithm to match the generation output with the closest existing package name. Our algorithm design is based on an empirical study of the errors of the raw output of ChatGPT. 

% Existing work on automatic identification of vulnerable packages~\cite{fastxml, viem, lightxml, chronos, vullibminer} propose  ranking approaches\footnote{\xueqing{classification which can be seen as ranking approach}} that,  given the vulnerability description as the query, rank the most similar package name from an existing list of package names of the corresponding ecosystem (e.g., PyPI, Maven). Since a ranking approach requires one to compute the description's similarity with each package, the time cost is typically large, e.g., Java has 435k packages. To the best of our knowledge, most existing approaches focus on relatively smaller models such as non-neural-network models~\cite{fastxml}, logistic regression~\cite{zestxml,chronos}, or BERT~\cite{lightxml,vullibminer}. Without leveraging larger models, they typically suffer from low accuracies. 


% However, these approaches face the scalability problem due to the large number of third-party packages (e.g., more than 500 thousand).
% Now that it is time-consuming to correlate each package with a given vulnerability description, a large portion of existing approaches use only lightweight models, such as FastXML~\cite{fastxml} and ZestXML~\cite{chronos} to rank these packages, thus leading to low accuracies.
% Although other approaches~\cite{vullibminer} adopt reranking models after the lightweight ranking model, the number of candidate packages (e.g., 512) still leads to a heavy burden of time and computation resources, especially when adopting large language models (LLMs).

% Specifically, both of these approaches are limited to their training set~\cite{fernandez2011semantically}.
% Thus, they are ineffective in identifying unseen vulnerable libraries during training.

% To address the low accuracy issue, in this paper, we propose to first leverage large language models (i.e., 7B models and larger) for vulnerable package identification. Given the description, our approach will \emph{generate}, rather than rank the package names. As a result, our approach can scale to larger models since this approach requires invoking the model inference only once. However, it is unclear whether the generative approach is effective for this task. On the one hand, the description often does not include the full information about the package name (Section~\ref{sec: empirical_study}); on the other hand, the task requires the generated package name to exactly match the ground truth and previous work finds this to be challenging for LLMs~\cite{liu2023codegen4libs}. To understand the potential of the generative approach, we conduct a pilot study on the errors made by ChatGPT raw output for this task. The study shows that ChatGPT raw output has a reasonable accuracy; however, for some vulnerabilities, ChatGPT lacks the domain knowledge for generation; for other vulnerabilities, the generated package names do not exist. 
%Based on the study results,
% \xueqing{I named the task vulnerable package identification, please check}.
% Nevertheless, text generation suffers from challenges such as hallucination~\cite{ji2023survey} which may affect the accuracy. To understand the feasibility of the generative approach, we first conduct a pilot study on how ChatGPT output for this task. We observe that with 42\% probability, the raw output correctly matches the ground truth. Among the incorrect outputs, 22.4\% can be fixed by matching the output with the closest existing package.
% \xueqing{Check if this statement is true}.
%(3) Among the rest incorrect names, ChatGPT captures incorrect keywords or fails to capture keywords from vulnerability descriptions due to its lack of knowledge.
% From the results of the preceding empirical study, we categorize two main challenges that lead to incorrectly generated names.
% First, LLMs lack sufficient domain knowledge of these affected libraries.
% For example, a Java package's name consists of both group IDs and artifact IDs while the group ID might be neglected in a vulnerability description.
% Therefore, LLMs need to generate the correct group ID based on their domain knowledge.
% Second, LLMs might output non-existing package names.
% Note that LLMs generate the names of affected packages from only vulnerability descriptions, so the output names might have more/fewer tokens, e.g., \CodeIn{core} or \CodeIn{framework}, which are widely used in the names of Java packages.



% To address the preceding challenges, we design three techniques to address the preceding challenges.
% First, we design a retrieval augmented generation (RAG) technique that provides domain knowledge into the inputs of LLMs before generation.
% Specifically, we add the names of affected libraries generated by IR approaches as they might be similar to the targeted library names.
% Second, we design a constrained decoding algorithm during generation.
% We collect package names from ecosystems of each programming language and require the output of LLMs to include at least one of them, thus avoiding non-existing package names.
% This technique modifies the decoding layer of LLMs and can be applied to only open-source LLMs.
% Third, we design a local search algorithm after generation.
% It directly searches the closest package name for each generated name, thus also avoiding non-existing package names.
% This technique is non-intrinsic and can be applied to both commercial and open-source LLMs.


Our evaluation of \detector{} shows three main findings. First, we observe that the accuracy of \detector{} significantly outperforms existing approaches~\cite{fastxml,lightxml,chronos,vullibminer} and the computational time cost is comparable. In particular, \detector{} using Vicuna-13B outperforms the larger ChatGPT and GPT-4 models by employing supervised fine-tuning (SFT). Second, our ablation studies show that SFT, RAG, and local search all improve the accuracy of \detector{}. Third, \detector{} provides high value to security practice: we have submitted 28 pairs of <vulnerability, generated affected package> to GitHub Advisory, and 22 of them are accepted and merged. 

% To examine \detector{}'s performance in the real-world setting, we further randomly sample a subset of the vulnerability descriptions in Java and JS, use \detector{} to generate the package names, and submit the generated names to GitHub Advisory. Among the 28 submitted <vulnerability, affected package> pairs, 22 are accepted and merged. This result highlights the real-world performance of \detector{} in automatically generating the names of affected packages. 

% We evaluate \detector{} using four state-of-the-art/practice (SOTA) approaches (FastXML~\cite{fastxml}, LightXML~\cite{lightxml}, Chronos~\cite{chronos}, and VulLibMiner~\cite{vullibminer}) that identify vulnerable libraries on the dataset of GitHub Advisory.
% Our evaluation results show that:
% (1) \detector{} is highly effective, achieving an accuracy of 0.806 while the best of SOTA approaches achieves only 0.669.
% (2) Our RAG technique and local search algorithm can boost the effectiveness of \detector{} by 8.9\% and 3.0\% on average, respectively.
% (3) \detector{} achieves better trade-offs between efficiency and accuracy than both existing and future ranking approaches.
% (4) \detector{} brings high value to security practice. 
% We have submitted 28 pairs of <vulnerability, affected package> to GitHub advisory, and 22 of them have been accepted and merged.
% We submit 25 vulnerabilities' affected libraries to GitHub advisory and 18 of them are accepted and merged.
% (5) Although fine-tuned open-source LLMs achieve similar effectiveness with ChatGPT/GPT4, they might face the limitation of overfitting, which can be alleviated by larger open-source LLMs.\tianyu{is it necessary to keep (5)?}



% Existing approaches~\cite{fastxml, viem, lightxml, chronos, vullibminer} model this task as an information retrieval (IR) task or a classification task.
% For example, they take the description field \CodeIn{``Jenkins Mail Commander Plugin for Jenkins-ci Plugin 1.0.0 and earlier stores passwords unencryted $\dots$''} as inputs and their targeted outputs, are the field of affected libraries, e.g., \CodeIn{maven:org.jenkins-ci.plugins:mailcommander}.
% However, these approaches face the scalability problem as it is unavoidable for IR/classification approaches.
% Specifically, both of these approaches are limited to their training set~\cite{fernandez2011semantically}.
% Thus, they are ineffective in identifying unseen vulnerable libraries during training.

% To address the scalability problem, in this paper, we propose to model this task as a generation task, thus utilizing the tremendous capabilities of Large Language Models (LLMs) in comprehending vulnerability descriptions.
% Here, we collect the dataset from the reviewed reports in GitHub Advisory.
% The affected libraries in each report are submitted by library developers and users, and they are manually validated by the maintainers of GitHub Advisory.
% Therefore, the ground truth of this dataset is reliable.
% Specifically, the number of Java, JavaScript, Python, and Go vulnerabilities are 4308, 3193, 2237, and 1351, respectively.


% Before employing LLMs for this task, we conduct an empirical study on the results when directly querying ChatGPT, revealing two main categories of challenges faced by LLMs.
% First, LLMs lack sufficient domain knowledge of these affected libraries.
% For example, in CVE-2022-24197, the affected library is \CodeIn{maven:com.itextpdf:itext7-core} while its description only mentions the affected library's artifact ID \CodeIn{itext7-core}, and its group ID \CodeIn{com.itextpdf} is neglected. 
% This group ID can be complemented based on the domain knowledge that only \CodeIn{itext7-core} corresponds to only one group ID \CodeIn{com.itextpdf}.
% Second, LLMs might output non-existing library names.
% For example, in CVE-2020-2167, the affected library is \CodeIn{maven:com.openshift.jenkins:openshift-pipeline} while LLMs might change the group ID into \CodeIn{com.openshift.jenkins}, which is not an existing library.
% % \tianyu{I also consider the reason that there might exist vulnerabilities whose descriptions are incomplete. (in the following comments in the source code)
% % However, this reason might be similar to 'lack of domain knowledge'}
% % First, the information in vulnerability reports might be incomplete. 
% % For example, in CVE-2017-1000406, the affected library is \CodeIn{maven:org.opendaylight.integration:distribution-karaf} while token \CodeIn{distribution} does not occur in its description.
% % Thus, even human experts cannot identify the correct names of affected libraries.


% To address the preceding challenges, we design two categories of techniques to address the preceding challenges.
% First, we design a retrieval augmented generation (RAG) technique that provides domain knowledge into the inputs of LLMs. 
% Specifically, we add the names of affected libraries generated by IR approaches as they might be similar to the targeted library names.
% Second, we design a constrained decoding algorithm and a local search algorithm to reduce non-existing outputs.
% Specifically, the constrained decoding algorithm is more effective while the local search algorithm is non-intrinsic and can be applied in commercial LLMs, e.g., ChatGPT/GPT4.
% Both algorithms utilize the database of all library names (e.g., those in Maven or Pypi) to ensure that the output of \detector{} is an existing library name.


% We evaluate \detector{} using three state-of-the-art/practice (SOTA) approaches (LightXML~\cite{lightxml}, Chronos~\cite{chronos}, and VulLibMiner~\cite{vullibminer}) that identify vulnerable libraries on the dataset of GitHub Advisory.
% Our evaluation results show that:
% (1) \detector{} is highly effective, achieving an accuracy of 0.80 while the best of SOTA approaches achieves only 0.669.
% (2) Our RAG technique can boost the effectiveness of both ChatGPT/GPT4 and open-source LLMs by at least 12\%.
% (3) Both our constrained decoding and local search algorithms can effectively reduce incorrect/non-existing outputs by at least 5.4\%.
% (4) \detector{} brings high value to security practice. We submit 25 vulnerabilities' affected libraries to GitHub advisory and 18 of them are accepted and merged.
% (5) Although fine-tuned open-source LLMs achieve similar effectiveness with ChatGPT/GPT4, they might face the limitation of overfitting, which can be alleviated by larger open-source LLMs.


% 一个建议的intro提纲：
% 1. CVE问题的重要性（为什么需要自动预测，可以帮助及时修补？）
% 2.当前解决方案的不足（scalability）
% 3.我们提出用generation来解决scalability问题，介绍一下GitHub advisory数据集以及为什么ground truth是准确的，3.但是generation存在挑战：一个是有的example input信息不全（所以即使human expert也很难做到100%），一个是llm缺乏domain knowledge 
% 4.做一个empirical study发现input信息不全的现象只占少数。同时针对以上挑战，设计了几个方法：fine tuning，rag，constrained decoding，post processing，讨论一下它们为什么有可能解决generation的挑战。
% 5. 总结实验结果，讨论可能存在的limitation，比如fine tuning可能存在overfitting，future work如何弥补这些limitation


% To avoid potential risks posed by vulnerabilities in third-party libraries, security researchers maintain databases containing vulnerability reports, e.g., the National Vulnerability Database (NVD)~\cite{nvd}. 
% A vulnerability report in NVD includes a vulnerability's identification number in the entry of Common Vulnerability Enumeration (CVE), its description, and the name list of libraries affected by the vulnerability  (a.k.a. vulnerable libraries).
% Application developers can identify vulnerable libraries by directly querying each description and CPE entry with the name of each used library. 
% However, recent studies on about 200,000 vulnerability reports in NVD show that 53.3\% of the vulnerability reports in NVD do not mention any affected libraries~\cite{lightxml} and 59.82\% of the included vulnerable libraries are incomplete or incorrect~\cite{viem}.


% To address the preceding issue, existing approaches~\cite{viem, anwar2021cleaning, jo2022vulcan, kuehn2021ovana, fastxml, lightxml, chronos, vullibminer} fall into three main categories.
% First, named-entity-recognition (NER) approaches~\cite{viem, anwar2021cleaning, jo2022vulcan, kuehn2021ovana} use NER models to extract the mentioned library entities from vulnerability descriptions, and then match these entities with a dictionary of library names.
% Second, extreme multi-label learning (XML) approaches~\cite{fastxml, lightxml, chronos} use deep-learning classification models to assign a set of labels (i.e., vulnerable libraries) to a given vulnerability by training on labeled datasets.
% Third, entity-linking approaches~\cite{vullibminer} take library descriptions as inputs besides the description of a given vulnerability, thus achieving higher accuracy than NER and XML approaches.

% Although existing approaches make efforts to identify vulnerable libraries, they still suffer from highly inaccurate results.
% Existing NER and XML approaches cannot distinguish vulnerable libraries with similar names, such as ``org.jenkins-ci.plugins:mailer'' and ``org.jenkins-ci.plugins:mailcommander''.
% However, these libraries are not affected together by one vulnerability due to their different functionalities and scopes.
% Existing entity-linking approaches use TF-IDF techniques to reduce the number of libraries for comparison, and yet suffer from false negatives (i.e., some vulnerable libraries are missed) and thus low accuracy.
% Considering the large number of collected libraries (e.g., 310,844 in Maven) for comparison compared, this step cannot be avoided; otherwise, it might cost them two years to identify all vulnerable libraries~\cite{vullibminer}.




% To overcome the preceding limitations, we propose \detector{}, the first generative approach to generate the affected libraries of a given vulnerability.
% \detector{} is effective to generate the name list of vulnerable libraries (out of all the existing libraries) by utilizing the recent enormous advances in Large Language Models (LLMs) with two stages of fine-tuning.
% The rationale behind this step is that LLMs can correlate the input vulnerability description to vulnerable libraries based on their prior knowledge of these libraries, e.g., their functionalities, usages, and even history issues.
% With prior knowledge, \detector{} avoids the high cost of correlating one vulnerability description with each library.
% Specifically, we conduct unsupervised fine-tuning on maven~\cite{maven} corpus to fine-tune raw LLaMa models to activate their prior knowledge of Java libraries.
% The input of this stage is one library's description, and its targeted output is its library name.
% Then, we conduct supervised fine-tuning on labeled datasets to enhance the ability to identify vulnerable libraries.
% The input of this stage is a vulnerability description and its targeted output is a name list of vulnerable libraries affected by this vulnerability.

% Since we use fine-tuned LLMs to generate the affected library names of a given vulnerability, there are two main challenges that decrease LLMs' effectiveness.
% First, LLMs face the difficulty of low accuracy when identifying zero-shot libraries because they have no prior knowledge of how these libraries are affected by vulnerabilities.
% Similar to XML approaches, LLMs tend to output incorrect libraries that have already been affected by other vulnerabilities during training and fine-tuning.
% Second, LLMs face hallucinations, i.e., generating plausible-looking library names that are non-existing.
% For example, they might mix up two similar library names and lack part of the library names.



% To address the preceding challenges, we design two specialized techniques during supervised fine-tuning to improve the effectiveness by addressing the preceding challenges.
% To help identify zero-shot libraries, we design an input augmentation technique, which feeds the names of vulnerable libraries (a.k.a., recommended libraries) identified by the SOTA approach~\cite{vullibminer} to \detector{} as input.
% This technique provides examples of libraries whose functionalities are likely to be affected by a given vulnerability.
% Thus, \detector{} can generate library names from those with similar functionalities instead of all libraries when \detector{} has no prior knowledge of how these zero-shot libraries are affected by vulnerabilities.
% To address \detector{}'s hallucinations, we design our post-processing technique based on the Levenshtein distance~\cite{levenshtein} to obtain existing Java library names from the response of LLMs.
% We find that \detector{} can generate the components of the targeted library names (i.e., the targeted functionalities and scopes), and make mistakes when jointing these components of library names, thus leading to hallucinations.
% Therefore, hallucination library names are close to the targeted names of vulnerable libraries, and their closest library names tend to be the targeted names.


% We evaluate \detector{} using three state-of-the-art/practice approaches (LightXML~\cite{lightxml}, Chronos~\cite{chronos}, and VulLibMiner~\cite{vullibminer}) that identify vulnerable libraries on an open-source dataset (VulLib)~\cite{vullib}.
% Our evaluation results show a number of findings to demonstrate our \detector{} approach’s effectiveness and efficiency.
% Given the ground truth score of 0.840, \detector{} effectively achieves the F1@1 score of 0.626 while the state-of-the-art/practice (SOTA) approaches achieve only 0.561.
% Specifically, the post-processing technique helps \detector{} achieve an average improvement of F1@1 by 9.3\%, and the input augmentation technique helps \detector{} achieve an average improvement of F1@1 by 39\% in identifying zero-shot libraries.
% Additionally, \detector{} is highly efficient, identifying one vulnerability in less than 6 seconds.


% In summary, this paper makes the following main contributions:
% \begin{itemize}
% \item  We propose, \detector{}, the first generative approach for identifying vulnerable libraries via Large Language Models.
% \item  We design an input augmentation technique and a post-processing technique to help identify zero-shot libraries and help address hallucinations.
% \item  We conduct a comprehensive evaluation demonstrating the effectiveness and efficiency of \detector{}, increasing the F1@1 of 0.626 while the state-of-the-art/practice (SOTA) approaches achieve only 0.561.
% \end{itemize}



==> backup/intro-backup.tex <==
\section{Introduction}~\label{sec:intro}
Vulnerability databases, e.g., the National Vulnerability Database (NVD)~\cite{nvd} and GitHub Advisory~\cite{githubAD}, maintain vulnerability reports to avoid potential risks posed by vulnerabilities in third-party libraries.
A vulnerability report includes a vulnerability's identification number, Common Vulnerability Enumeration (CVE), its description, and the name list of libraries affected by the vulnerability  (a.k.a. vulnerable libraries).
For example, Figure~\ref{fig: case} shows an example of CVE-2020-2318, whose affected library is \CodeIn{org.jenkins-ci.plugins:mailcommander}.
Developers can identify vulnerable libraries from their used ones by directly querying the field of affected libraries, and then update them to avoid potential risks.
However, the data in this field are labor-intensive and error-prone.
Recent studies show that 53.3\% of the vulnerability reports in NVD do not include this field~\cite{lightxml} and 59.82\% of the data in this field is incomplete or incorrect~\cite{viem}.
Therefore, it is necessary to automatically identify libraries affected by a given CVE.

\begin{figure}[t]
\centering
\includegraphics[width=1\linewidth]{figures/vulnerability-report.drawio.pdf}
\caption{GitHub Advisory Report for CVE-2020-2318}
\label{fig: case}
\end{figure}


Existing approaches~\cite{fastxml, viem, lightxml, chronos, vullibminer} model this task as an information retrieval (IR) task or a classification task.
For example, they take the description field \CodeIn{``Jenkins Mail Commander Plugin for Jenkins-ci Plugin 1.0.0 and earlier stores passwords unencryted $\dots$''} as inputs and their targeted outputs, are the field of affected libraries, e.g., \CodeIn{maven:org.jenkins-ci.plugins:mailcommander}.
However, these approaches face the scalability problem as it is unavoidable for IR/classification approaches.
Specifically, both of these approaches are limited to their training set~\cite{fernandez2011semantically}.
Thus, they are ineffective in identifying unseen vulnerable libraries during training.

To address the scalability problem, in this paper, we propose to model this task as a generation task, thus utilizing the tremendous capabilities of Large Language Models (LLMs) in comprehending vulnerability descriptions.
Here, we collect the dataset from the reviewed reports in GitHub Advisory.
The affected libraries in each report are submitted by library developers and users, and they are manually validated by the maintainers of GitHub Advisory.
Therefore, the ground truth of this dataset is reliable.
Specifically, the number of Java, JavaScript, Python, and Go vulnerabilities are 4308, 3193, 2237, and 1351, respectively.


Before employing LLMs for this task, we conduct an empirical study on the results when directly querying ChatGPT, revealing two main categories of challenges faced by LLMs.
First, LLMs lack sufficient domain knowledge of these affected libraries.
For example, in CVE-2022-24197, the affected library is \CodeIn{maven:com.itextpdf:itext7-core} while its description only mentions the affected library's artifact ID \CodeIn{itext7-core}, and its group ID \CodeIn{com.itextpdf} is neglected. 
This group ID can be complemented based on the domain knowledge that only \CodeIn{itext7-core} corresponds to only one group ID \CodeIn{com.itextpdf}.
Second, LLMs might output non-existing library names.
For example, in CVE-2020-2167, the affected library is \CodeIn{maven:com.openshift.jenkins:openshift-pipeline} while LLMs might change the group ID into \CodeIn{com.openshift.jenkins}, which is not an existing library.
% \tianyu{I also consider the reason that there might exist vulnerabilities whose descriptions are incomplete. (in the following comments in the source code)
% However, this reason might be similar to 'lack of domain knowledge'}
% First, the information in vulnerability reports might be incomplete. 
% For example, in CVE-2017-1000406, the affected library is \CodeIn{maven:org.opendaylight.integration:distribution-karaf} while token \CodeIn{distribution} does not occur in its description.
% Thus, even human experts cannot identify the correct names of affected libraries.


To address the preceding challenges, we design two categories of techniques to address the preceding challenges.
First, we design a retrieval augmented generation (RAG) technique that provides domain knowledge into the inputs of LLMs. 
Specifically, we add the names of affected libraries generated by IR approaches as they might be similar to the targeted library names.
Second, we design a constrained decoding algorithm and a local search algorithm to reduce non-existing outputs.
Specifically, the constrained decoding algorithm is more effective while the local search algorithm is non-intrinsic and can be applied in commercial LLMs, e.g., ChatGPT/GPT4.
Both algorithms utilize the database of all library names (e.g., those in Maven or Pypi) to ensure that the output of \detector{} is an existing library name.


We evaluate \detector{} using three state-of-the-art/practice (SOTA) approaches (LightXML~\cite{lightxml}, Chronos~\cite{chronos}, and VulLibMiner~\cite{vullibminer}) that identify vulnerable libraries on the dataset of GitHub Advisory.
Our evaluation results show that:
(1) \detector{} is highly effective, achieving an accuracy of 0.80 while the best of SOTA approaches achieves only 0.669.
(2) Our RAG technique can boost the effectiveness of both ChatGPT/GPT4 and open-source LLMs by at least 12\%.
(3) Both our constrained decoding and local search algorithms can effectively reduce incorrect/non-existing outputs by at least 5.4\%.
(4) \detector{} brings high value to security practice. We submit 25 vulnerabilities' affected libraries to GitHub advisory and 18 of them are accepted and merged.
(5) Although fine-tuned open-source LLMs achieve similar effectiveness with ChatGPT/GPT4, they might face the limitation of overfitting, which can be alleviated by larger open-source LLMs.


% 一个建议的intro提纲：
% 1. CVE问题的重要性（为什么需要自动预测，可以帮助及时修补？）
% 2.当前解决方案的不足（scalability）
% 3.我们提出用generation来解决scalability问题，介绍一下GitHub advisory数据集以及为什么ground truth是准确的，3.但是generation存在挑战：一个是有的example input信息不全（所以即使human expert也很难做到100%），一个是llm缺乏domain knowledge 
% 4.做一个empirical study发现input信息不全的现象只占少数。同时针对以上挑战，设计了几个方法：fine tuning，rag，constrained decoding，post processing，讨论一下它们为什么有可能解决generation的挑战。
% 5. 总结实验结果，讨论可能存在的limitation，比如fine tuning可能存在overfitting，future work如何弥补这些limitation


% To avoid potential risks posed by vulnerabilities in third-party libraries, security researchers maintain databases containing vulnerability reports, e.g., the National Vulnerability Database (NVD)~\cite{nvd}. 
% A vulnerability report in NVD includes a vulnerability's identification number in the entry of Common Vulnerability Enumeration (CVE), its description, and the name list of libraries affected by the vulnerability  (a.k.a. vulnerable libraries).
% Application developers can identify vulnerable libraries by directly querying each description and CPE entry with the name of each used library. 
% However, recent studies on about 200,000 vulnerability reports in NVD show that 53.3\% of the vulnerability reports in NVD do not mention any affected libraries~\cite{lightxml} and 59.82\% of the included vulnerable libraries are incomplete or incorrect~\cite{viem}.


% To address the preceding issue, existing approaches~\cite{viem, anwar2021cleaning, jo2022vulcan, kuehn2021ovana, fastxml, lightxml, chronos, vullibminer} fall into three main categories.
% First, named-entity-recognition (NER) approaches~\cite{viem, anwar2021cleaning, jo2022vulcan, kuehn2021ovana} use NER models to extract the mentioned library entities from vulnerability descriptions, and then match these entities with a dictionary of library names.
% Second, extreme multi-label learning (XML) approaches~\cite{fastxml, lightxml, chronos} use deep-learning classification models to assign a set of labels (i.e., vulnerable libraries) to a given vulnerability by training on labeled datasets.
% Third, entity-linking approaches~\cite{vullibminer} take library descriptions as inputs besides the description of a given vulnerability, thus achieving higher accuracy than NER and XML approaches.

% Although existing approaches make efforts to identify vulnerable libraries, they still suffer from highly inaccurate results.
% Existing NER and XML approaches cannot distinguish vulnerable libraries with similar names, such as ``org.jenkins-ci.plugins:mailer'' and ``org.jenkins-ci.plugins:mailcommander''.
% However, these libraries are not affected together by one vulnerability due to their different functionalities and scopes.
% Existing entity-linking approaches use TF-IDF techniques to reduce the number of libraries for comparison, and yet suffer from false negatives (i.e., some vulnerable libraries are missed) and thus low accuracy.
% Considering the large number of collected libraries (e.g., 310,844 in Maven) for comparison compared, this step cannot be avoided; otherwise, it might cost them two years to identify all vulnerable libraries~\cite{vullibminer}.




% To overcome the preceding limitations, we propose \detector{}, the first generative approach to generate the affected libraries of a given vulnerability.
% \detector{} is effective to generate the name list of vulnerable libraries (out of all the existing libraries) by utilizing the recent enormous advances in Large Language Models (LLMs) with two stages of fine-tuning.
% The rationale behind this step is that LLMs can correlate the input vulnerability description to vulnerable libraries based on their prior knowledge of these libraries, e.g., their functionalities, usages, and even history issues.
% With prior knowledge, \detector{} avoids the high cost of correlating one vulnerability description with each library.
% Specifically, we conduct unsupervised fine-tuning on maven~\cite{maven} corpus to fine-tune raw LLaMa models to activate their prior knowledge of Java libraries.
% The input of this stage is one library's description, and its targeted output is its library name.
% Then, we conduct supervised fine-tuning on labeled datasets to enhance the ability to identify vulnerable libraries.
% The input of this stage is a vulnerability description and its targeted output is a name list of vulnerable libraries affected by this vulnerability.

% Since we use fine-tuned LLMs to generate the affected library names of a given vulnerability, there are two main challenges that decrease LLMs' effectiveness.
% First, LLMs face the difficulty of low accuracy when identifying zero-shot libraries because they have no prior knowledge of how these libraries are affected by vulnerabilities.
% Similar to XML approaches, LLMs tend to output incorrect libraries that have already been affected by other vulnerabilities during training and fine-tuning.
% Second, LLMs face hallucinations, i.e., generating plausible-looking library names that are non-existing.
% For example, they might mix up two similar library names and lack part of the library names.



% To address the preceding challenges, we design two specialized techniques during supervised fine-tuning to improve the effectiveness by addressing the preceding challenges.
% To help identify zero-shot libraries, we design an input augmentation technique, which feeds the names of vulnerable libraries (a.k.a., recommended libraries) identified by the SOTA approach~\cite{vullibminer} to \detector{} as input.
% This technique provides examples of libraries whose functionalities are likely to be affected by a given vulnerability.
% Thus, \detector{} can generate library names from those with similar functionalities instead of all libraries when \detector{} has no prior knowledge of how these zero-shot libraries are affected by vulnerabilities.
% To address \detector{}'s hallucinations, we design our post-processing technique based on the Levenshtein distance~\cite{levenshtein} to obtain existing Java library names from the response of LLMs.
% We find that \detector{} can generate the components of the targeted library names (i.e., the targeted functionalities and scopes), and make mistakes when jointing these components of library names, thus leading to hallucinations.
% Therefore, hallucination library names are close to the targeted names of vulnerable libraries, and their closest library names tend to be the targeted names.


% We evaluate \detector{} using three state-of-the-art/practice approaches (LightXML~\cite{lightxml}, Chronos~\cite{chronos}, and VulLibMiner~\cite{vullibminer}) that identify vulnerable libraries on an open-source dataset (VulLib)~\cite{vullib}.
% Our evaluation results show a number of findings to demonstrate our \detector{} approach’s effectiveness and efficiency.
% Given the ground truth score of 0.840, \detector{} effectively achieves the F1@1 score of 0.626 while the state-of-the-art/practice (SOTA) approaches achieve only 0.561.
% Specifically, the post-processing technique helps \detector{} achieve an average improvement of F1@1 by 9.3\%, and the input augmentation technique helps \detector{} achieve an average improvement of F1@1 by 39\% in identifying zero-shot libraries.
% Additionally, \detector{} is highly efficient, identifying one vulnerability in less than 6 seconds.


% In summary, this paper makes the following main contributions:
% \begin{itemize}
% \item  We propose, \detector{}, the first generative approach for identifying vulnerable libraries via Large Language Models.
% \item  We design an input augmentation technique and a post-processing technique to help identify zero-shot libraries and help address hallucinations.
% \item  We conduct a comprehensive evaluation demonstrating the effectiveness and efficiency of \detector{}, increasing the F1@1 of 0.626 while the state-of-the-art/practice (SOTA) approaches achieve only 0.561.
% \end{itemize}



==> tables/cases.tex <==
{'cve_id': 'CVE-2020-2318',
 'labels': ['maven:org.jenkins-ci.plugins:mailcommander'],
 'source': 'Below is an Java vulnerability description. Please identify the software name affected by it.Input: Jenkins Mail Commander Plugin for Jenkins-ci Plugin 1.0.0 and earlier stores passwords unencrypted in job config.xml files on the Jenkins controller where they can be viewed by users with Extended Read permission, or access to the Jenkins controller file system. Top 1 search result are maven:org.jenkins-ci.plugins:job-direct-mail ### Response:  The affected packages',
 'target': 'The affected packages is maven:org.jenkins-ci.plugins:mailcommander.',
 'response_text': ' is maven:org.jenkins-ci.plugins:mail-commander.',
 'predict_labels': ['maven:org.jenkins-ci.plugins:mailcommander'],
 'zero': True}

 'mailcommander' only one group id
 'mail-commander' no group id

len(artifacts) = 274232, len(groups) = 53074

An example: CVE-2020-2311
there are 1,208 Java libraries with group id 'org.jenkins-ci.plugins'

and 2,34 Java libraries with group id 'io.jenkins.plugins'.

However, there are only one Java libraries with artifact id 'aws-global-configuration'

 {'cve_id': 'CVE-2020-2311',
  'labels': ['maven:io.jenkins.plugins:aws-global-configuration'],
  'source': 'Below is an Java vulnerability description. Please identify the software name affected by it.Input: A missing permission check in Jenkins AWS Global Configuration Plugin 1.5 and earlier allows attackers with Overall/Read permission to replace the global AWS configuration. Top 1 search result are maven:io.jenkins.plugins:aws-global-configuration ### Response:  The affected packages',
  'target': 'The affected packages is maven:io.jenkins.plugins:aws-global-configuration.',
  'response_text': ' is maven:org.jenkins-ci.plugins:aws-global-configuration.',
  'predict_labels': ['maven:io.jenkins.plugins:aws-global-configuration'],
  'zero': True})


==> tables/eval-todo.tex <==
\item \textbf{RQ1}: How effectively can \detector{} identify vulnerable Java libraries when compared with baseline approaches?
\item \textbf{RQ2}: To what extent can recommended libraries help \detector{} identify zero-shot libraries?
\item \textbf{RQ3}: How effectively can \detector{} generate legal Java libraries names?
\item \textbf{RQ4}: How efficiently can \detector{} identify vulnerable Java libraries?


模型 	预训练 		监督学习 		强化学习 		预测							监督学习时间 	强化学习时间 	预测时间 (一个checkpoint)	后处理时间 	
								原始结果 			后处理 							
	数据集 	loss 	数据集 	loss 	数据集 	loss 	数据集 	Raw 	Zero-Shot 	No-Zero-Shot 	Raw 	Zero-Shot 	No-Zero-Shot 					
Group Truth 								0.829	0.861 	0.857 								
LightXML	-	-	-	-	-	-	-	(0.444, 0.328, 0.377), (0.295, 0.398, 0.339), (0.225, 0.434, 0.297)	0,0,0	(0.619, 0.458, 0.526)								
Chronos	-	-	-	-	-	-	-	(0.416, 0.318, 0.360), (0.247, 0.355, 0.292), (0.182, 0.381, 0.247)	0,0,0	(0.583, 0.445, 0.505), (0.346, 0.494, 0.407), (0.254, 0.533, 0.344)								
VulLibMiner								(0.629, 0.477, 0.542)	(0.453, 0.386, 0.417)	(0.699, 0.513, 0.591)								
GPT-2 	训练 		无prompt 				无prompt 											
			预排序 				预排序 											
			重排序 				重排序 											
	不训练		重排序 				重排序 											
			无prompt 				无prompt 											
			预排序 				预排序 											
			重排序 				重排序 											
			重排序 				重排序 											
LLaMa-7B 	训练 	0.377624371495631	无prompt 		？？ 		无prompt 											
	（训练用时）	138:00:42	预排序 				预排序 											
			重排序 	0.358	无 		重排序 	(0.658, 0.507, 0.573)			(0.699, 0.545, 0.612)			34:52:33				已完成
			重排序 		有 		重排序 											
	不训练 		不fine-tune				无prompt 									04:30:18		
			无prompt 		无 		无prompt 											
			预排序 top1		无 		预排序 top1											
			预排序 top2		无 		预排序 top2											
			预排序 top3		无 		预排序 top3											
			重排序 top1		无 		重排序 top1											
			重排序 top2		无 		重排序 top2											
			重排序 top3		无 		重排序 top3											
			重排序 		有 		重排序 											
LLaMa-13B 	训练 		无prompt 		无 		无prompt 											
			预排序 top1		无 		预排序 top1	(0.642, 0.491, 0.557)	(0.319, 0.295, 0.306)	(0.770, 0.568, 0.654)	(0.692, 0.533, 0.602)	(0.456, 0.426, 0.441)	(0.785, 0.576, 0.664)	30:47:50				onpred
			重排序 top1		无 		重排序 top1	(0.680, 0.534, 0.598)	(0.500, 0.455, 0.477)	(0.751, 0.566, 0.645)	(0.697, 0.550, 0.615)	(0.544, 0.496, 0.516)	(0.758, 0.572, 0.652)	30:46:23		00:30:20	00:04:33	已完成 
			重排序 top2				重排序 top2											ongoing
			重排序 top3				重排序 top3											
			重排序 		有 		重排序 											
	不训练 		不fine-tune				无prompt 	(0.0, 0.0, 0.0)						-		05:01:16	-	已完成 
			无prompt 		无 		无prompt 	(0.607, 0.461, 0.524)	(0.225, 0.204, 0.214)	(0.758, 0.562, 0.646)	(0.687, 0.522, 0.593)	(0.419, 0.372, 0.394)	(0.793, 0.581, 0.670)	30:27:07		00:32:47	00:08:27	已完成 
			预排序 top1		无 		预排序 top1	(0.639, 0.484, 0.551)	(0.294, 0.271, 0.282)	(0.775, 0.568, 0.656)	(0.688, 0.537, 0.604)	(0.462, 0.431, 0.446)	(0.778, 0.579, 0.664)	30:30:45		00:39:31	00:06:19	已完成 
			预排序 top2		无 		预排序 top2	(0.637, 0.483, 0.549)	(0.312, 0.293, 0.302)	(0.765, 0.557, 0.645)	(0.687, 0.529, 0.597)	(0.456, 0.430, 0.443)	(0.778, 0.567, 0.656)	30:32:58		00:33:41	00:05:49	已完成 
			预排序 top3		无 		预排序 top3	(0.641, 0.487, 0.553)	(0.331, 0.302, 0.316)	(0.763, 0.559, 0.646)	(0.696, 0.531, 0.602)	(0.469, 0.424, 0.445)	(0.785, 0.574, 0.663)	30:37:19		00:30:46	00:04:58	已完成 
			重排序 top1		无 		重排序 top1	(0.687, 0.525, 0.595)	(0.419, 0.380, 0.399)	(0.793, 0.582, 0.671)	(0.720, 0.554, 0.626)	(0.506, 0.461, 0.483)	(0.805, 0.591, 0.681)	30:37:40		00:39:28	00:05:36	已完成 
			重排序 top2		无 		重排序 top2	(0.685, 0.535, 0.601)	(0.531, 0.478, 0.503)	(0.746, 0.557, 0.638)	(0.703, 0.551, 0.618)	(0.575, 0.522, 0.547)	(0.753, 0.563, 0.644)	30:36:17		00:38:42	00:04:42	已完成 
			重排序 top3		无 		重排序 top3	(0.680, 0.526, 0.593)	(0.556, 0.495, 0.524)	(0.728, 0.538, 0.619)	(0.701, 0.543, 0.612)	(0.575, 0.520, 0.546)	(0.751, 0.552, 0.636)	30:47:47		00:32:23	00:03:59	已完成 
			重排序 top1		有 		重排序 top1											


==> tables/overall.tex <==
./LLaMa13B/java_0.2_re_rank_top_1_prompt_1/checkpoint-400/test_predict.json 1
524 542 619 633
./LLaMa13B/java_0.2_re_rank_top_2_prompt_1/checkpoint-100/test_predict.json 2
569 584 614 633
./LLaMa13B/java_0.2_re_rank_top_3_prompt_1/checkpoint-300/test_predict.json 3
550 554 598 633
./LLaMa13B/java_0.2_top_1_prompt_1/checkpoint-400/test_predict.json 1
489 513 609 633
./LLaMa13B/java_0.2_top_2_prompt_1/checkpoint-400/test_predict.json 2
485 523 608 633
./LLaMa13B/java_0.2_top_3_prompt_1/checkpoint-700/test_predict.json 3
508 535 612 633

LLaMa13B/java_0.2_prompt_1/checkpoint-300/test_predict.json 1
454 485 584 633



The best score after post-processing:
raw: 0.6566371681415929, 0.5119329195877869, 0.5753256670291043
post-processing: 0.6991150442477876 0.5491010611807072 0.6150935098727557

模型（Metrics F1@Top1）	预训练	监督学习	预测	数据集
	输入	loss	数据格式	训练方法	Prompt	Raw	Zero-Shot	No-Zero-Shot
Group Truth	-	-		人工挑选group truth		0.829	0.861	0.857
Bert-Based	-	-		TF-IDF搜索+Cross Attention		0.552	0.517	0.614
GPT2-Fine Tune 0.1	Maven: desc + soft_name
TrainData: vul_desc + soft_name	0.2113	Query: vul_desc
Response: <search_top_1> This vulnerability  description
 soft_name	计算response loss	This vulnerability  description	0.485	0.198	0.656
LLaMa7B-Fine Tune	-	-	Query: vul_desc
Response: The affected packages is <soft_name>	计算response loss	None	0.496	0.197	0.643
LLaMa7B-Fine Tune			Query: vul_desc
Response: The affected packages is soft_name + EOS	计算response loss	None	0.461	0.174	0.618
LLaMa7B-Fine Tune			Query: vul_desc
Response: The affected packages is soft_name + EOS	计算response loss	The affected packages	0.52	0.184	0.694
LLaMa7B-Fine Tune			Query: vul_desc + search top 1
Response: The affected packages is soft_name + EOS	计算response loss	The affected packages	0.544	0.292	0.693
LLaMa7B-Fine Tune			Query: vul_desc + bert-re-rank search top 1
Response: The affected packages is soft_name + EOS	计算response loss	The affected packages	0.578	0.412	0.697
LLaMa7B-Fine Tune	Maven:	？？	Query: vul_desc + search top 1
Response: The affected packages is soft_name + EOS	计算response loss	The affected packages	0.589	0.458	0.694





(base) root@0c7216911321:~/VulnerabilityGPT-Refactor# CUDA_VISIBLE_DEVICES=1 python llama_infer.py --data_url=../input/ --checkpoint_path=../checkpoint/ --train_url=.. --toal_eval_work_nums=1 --checkpoint_prefix=checkpoint- --current_eval_work_index=1 --dataset_relative_path=dataset/java_0.2_re_rank_top_1_prompt_1 --is_lora_mode=False --base_heckpoint_path=LLaMa/SFT/add_eos_search_top_1_epoch_20/checkpoint-700/
all input args: ['--data_url=../input/', '--checkpoint_path=../checkpoint/', '--train_url=..', '--total_eval_work_nums=1', '--checkpoint_prefix=checkpoint-', '--current_eva_work_index=1', '--dataset_relative_path=dataset/java_0.2_re_rank_top_1_prompt_1', '--is_lora_mode=False', '--base_checkpoint_path=LLaMa/SFT/add_eos_search_top_1_epoch_20/ceckpoint-700/']
2023-07-04 09:17:55: Is GPU available: True; gpu count 1
2023-07-04 09:17:55: all eval folders [(100, 'checkpoint-100'), (200, 'checkpoint-200'), (300, 'checkpoint-300'), (400, 'checkpoint-400'), (500, 'checkpoint-500'), (600, 'ceckpoint-600'), (700, 'checkpoint-700'), (800, 'checkpoint-800'), (900, 'checkpoint-900'), (1000, 'checkpoint-1000'), (1100, 'checkpoint-1100')]
current_checkpoint_path: ../checkpoint/checkpoint-100
start loading model
load after <class 'transformers.models.llama.modeling_llama.LlamaForCausalLM'>
2023-07-04 09:26:59: Begin ../input/dataset/java_0.2_re_rank_top_1_prompt_1/validate.json dataset evaluate checkpoint checkpoint-100
2023-07-04 09:26:59: checkpoint-100 progress 0/620
2023-07-04 09:28:11: checkpoint-100 progress 50/620
2023-07-04 09:29:13: checkpoint-100 progress 100/620
2023-07-04 09:30:17: checkpoint-100 progress 150/620
2023-07-04 09:31:18: checkpoint-100 progress 200/620
2023-07-04 09:32:32: checkpoint-100 progress 250/620
2023-07-04 09:33:32: checkpoint-100 progress 300/620
2023-07-04 09:34:35: checkpoint-100 progress 350/620
2023-07-04 09:35:43: checkpoint-100 progress 400/620
2023-07-04 09:36:47: checkpoint-100 progress 450/620
2023-07-04 09:37:53: checkpoint-100 progress 500/620
2023-07-04 09:38:57: checkpoint-100 progress 550/620
2023-07-04 09:40:03: checkpoint-100 progress 600/620
2023-07-04 09:40:37: Begin ../input/dataset/java_0.2_re_rank_top_1_prompt_1/test.json dataset evaluate checkpoint checkpoint-100
2023-07-04 09:40:37: checkpoint-100 progress 0/633
2023-07-04 09:41:40: checkpoint-100 progress 50/633
2023-07-04 09:42:39: checkpoint-100 progress 100/633
2023-07-04 09:43:41: checkpoint-100 progress 150/633
2023-07-04 09:45:01: checkpoint-100 progress 200/633
2023-07-04 09:46:01: checkpoint-100 progress 250/633
2023-07-04 09:47:07: checkpoint-100 progress 300/633
2023-07-04 09:48:08: checkpoint-100 progress 350/633
2023-07-04 09:49:09: checkpoint-100 progress 400/633
2023-07-04 09:50:07: checkpoint-100 progress 450/633
2023-07-04 09:51:11: checkpoint-100 progress 500/633
2023-07-04 09:52:14: checkpoint-100 progress 550/633
2023-07-04 09:53:18: checkpoint-100 progress 600/633
current_checkpoint_path: ../checkpoint/checkpoint-200
start loading model
^[OR^H^HTraceback (most recent call last):
  File "/root/VulnerabilityGPT-Refactor/llama_infer.py", line 142, in <module>
    eval_result(script_args)
  File "/root/VulnerabilityGPT-Refactor/llama_infer.py", line 92, in eval_result
    model, tokenizer = _load_model(input_args, current_checkpoint_path)
  File "/root/VulnerabilityGPT-Refactor/llama_infer.py", line 54, in _load_model
    model.cuda()
  File "/root/anaconda3/lib/python3.10/site-packages/torch/nn/modules/module.py", line 689, in cuda
    return self._apply(lambda t: t.cuda(device))
  File "/root/anaconda3/lib/python3.10/site-packages/torch/nn/modules/module.py", line 579, in _apply
    module._apply(fn)
  File "/root/anaconda3/lib/python3.10/site-packages/torch/nn/modules/module.py", line 579, in _apply
    module._apply(fn)
  File "/root/anaconda3/lib/python3.10/site-packages/torch/nn/modules/module.py", line 579, in _apply
    module._apply(fn)
  [Previous line repeated 2 more times]
  File "/root/anaconda3/lib/python3.10/site-packages/torch/nn/modules/module.py", line 602, in _apply
    param_applied = fn(param)
  File "/root/anaconda3/lib/python3.10/site-packages/torch/nn/modules/module.py", line 689, in <lambda>
    return self._apply(lambda t: t.cuda(device))
RuntimeError: CUDA out of memory. Tried to allocate 270.00 MiB (GPU 0; 79.17 GiB total capacity; 56.67 GiB already allocated; 118.88 MiB free; 56.67 GiB reserved in total b PyTorch) If reserved memory is >> allocated memory try setting max_split_size_mb to avoid fragmentation.  See documentation for Memory Management and PYTORCH_CUDA_ALLOC_COF
(base) root@0c7216911321:~/VulnerabilityGPT-Refactor# CUDA_VISIBLE_DEVICES=1 python llama_infer.py --data_url=../input/ --checkpoint_path=../checkpoint/ --train_url=.. --toal_eval_work_nums=11 --checkpoint_prefix=checkpoint- --current_eval_work_index=2 --dataset_relative_path=dataset/java_0.2_re_rank_top_1_prompt_1 --is_lora_mode=False --basecheckpoint_path=LLaMa/SFT/add_eos_search_top_1_epoch_20/checkpoint-700/
all input args: ['--data_url=../input/', '--checkpoint_path=../checkpoint/', '--train_url=..', '--total_eval_work_nums=11', '--checkpoint_prefix=checkpoint-', '--current_evl_work_index=2', '--dataset_relative_path=dataset/java_0.2_re_rank_top_1_prompt_1', '--is_lora_mode=False', '--base_checkpoint_path=LLaMa/SFT/add_eos_search_top_1_epoch_20/heckpoint-700/']
2023-07-04 10:04:06: Is GPU available: True; gpu count 1
2023-07-04 10:04:06: all eval folders [(200, 'checkpoint-200')]
current_checkpoint_path: ../checkpoint/checkpoint-200
start loading model
load after <class 'transformers.models.llama.modeling_llama.LlamaForCausalLM'>
2023-07-04 10:07:33: Begin ../input/dataset/java_0.2_re_rank_top_1_prompt_1/validate.json dataset evaluate checkpoint checkpoint-200
2023-07-04 10:07:33: checkpoint-200 progress 0/620
2023-07-04 10:08:56: checkpoint-200 progress 50/620
2023-07-04 10:10:20: checkpoint-200 progress 100/620
2023-07-04 10:11:54: checkpoint-200 progress 150/620
2023-07-04 10:13:18: checkpoint-200 progress 200/620
2023-07-04 10:14:47: checkpoint-200 progress 250/620
2023-07-04 10:15:55: checkpoint-200 progress 300/620
2023-07-04 10:17:09: checkpoint-200 progress 350/620
2023-07-04 10:18:28: checkpoint-200 progress 400/620
2023-07-04 10:19:38: checkpoint-200 progress 450/620
2023-07-04 10:21:02: checkpoint-200 progress 500/620
2023-07-04 10:22:12: checkpoint-200 progress 550/620
2023-07-04 10:23:43: checkpoint-200 progress 600/620
2023-07-04 10:24:12: Begin ../input/dataset/java_0.2_re_rank_top_1_prompt_1/test.json dataset evaluate checkpoint checkpoint-200
2023-07-04 10:24:12: checkpoint-200 progress 0/633
2023-07-04 10:25:16: checkpoint-200 progress 50/633
2023-07-04 10:26:29: checkpoint-200 progress 100/633
2023-07-04 10:27:35: checkpoint-200 progress 150/633
2023-07-04 10:29:16: checkpoint-200 progress 200/633
2023-07-04 10:30:24: checkpoint-200 progress 250/633
2023-07-04 10:31:34: checkpoint-200 progress 300/633
2023-07-04 10:32:39: checkpoint-200 progress 350/633
2023-07-04 10:33:56: checkpoint-200 progress 400/633
2023-07-04 10:35:06: checkpoint-200 progress 450/633
2023-07-04 10:36:18: checkpoint-200 progress 500/633
2023-07-04 10:37:32: checkpoint-200 progress 550/633
2023-07-04 10:38:39: checkpoint-200 progress 600/633
(base) root@0c7216911321:~/VulnerabilityGPT-Refactor# CUDA_VISIBLE_DEVICES=1 python llama_infer.py --data_url=../input/ --checkpoint_path=../checkpoint/ --train_url=.. --total_eval_work_nums=11 --checkpoint_prefix=checkpoint- --current_eval_work_index=3 --dataset_relative_path=dataset/java_0.2_re_rank_top_1_prompt_1 --is_lora_mode=False --base_checkpoint_path=LLaMa/SFT/add_eos_search_top_1_epoch_20/checkpoint-700/
all input args: ['--data_url=../input/', '--checkpoint_path=../checkpoint/', '--train_url=..', '--total_eval_work_nums=11', '--checkpoint_prefix=checkpoint-', '--current_eval_work_index=3', '--dataset_relative_path=dataset/java_0.2_re_rank_top_1_prompt_1', '--is_lora_mode=False', '--base_checkpoint_path=LLaMa/SFT/add_eos_search_top_1_epoch_20/checkpoint-700/']
2023-07-04 10:41:04: Is GPU available: True; gpu count 1
2023-07-04 10:41:04: all eval folders [(300, 'checkpoint-300')]
current_checkpoint_path: ../checkpoint/checkpoint-300
start loading model
load after <class 'transformers.models.llama.modeling_llama.LlamaForCausalLM'>
2023-07-04 10:49:42: Begin ../input/dataset/java_0.2_re_rank_top_1_prompt_1/validate.json dataset evaluate checkpoint checkpoint-300
2023-07-04 10:49:42: checkpoint-300 progress 0/620
2023-07-04 10:51:08: checkpoint-300 progress 50/620
2023-07-04 10:52:15: checkpoint-300 progress 100/620
2023-07-04 10:53:37: checkpoint-300 progress 150/620
2023-07-04 10:54:47: checkpoint-300 progress 200/620
2023-07-04 10:56:17: checkpoint-300 progress 250/620
2023-07-04 10:57:25: checkpoint-300 progress 300/620
2023-07-04 10:59:05: checkpoint-300 progress 350/620
2023-07-04 11:00:22: checkpoint-300 progress 400/620
2023-07-04 11:01:33: checkpoint-300 progress 450/620
2023-07-04 11:02:55: checkpoint-300 progress 500/620
2023-07-04 11:04:13: checkpoint-300 progress 550/620
2023-07-04 11:05:23: checkpoint-300 progress 600/620
2023-07-04 11:05:50: Begin ../input/dataset/java_0.2_re_rank_top_1_prompt_1/test.json dataset evaluate checkpoint checkpoint-300
2023-07-04 11:05:50: checkpoint-300 progress 0/633
2023-07-04 11:06:58: checkpoint-300 progress 50/633
2023-07-04 11:08:04: checkpoint-300 progress 100/633
2023-07-04 11:09:11: checkpoint-300 progress 150/633
2023-07-04 11:10:23: checkpoint-300 progress 200/633
2023-07-04 11:11:29: checkpoint-300 progress 250/633
2023-07-04 11:12:46: checkpoint-300 progress 300/633
2023-07-04 11:14:02: checkpoint-300 progress 350/633
2023-07-04 11:15:21: checkpoint-300 progress 400/633
2023-07-04 11:16:41: checkpoint-300 progress 450/633
2023-07-04 11:17:59: checkpoint-300 progress 500/633
2023-07-04 11:19:19: checkpoint-300 progress 550/633
2023-07-04 11:20:32: checkpoint-300 progress 600/633


chronos:
pre-processing: 110min57s50ms

full-shot-chronos
K = 1
P@1 =  0.582716049382716
R@1 =  0.44532734754956926
F@1 =  0.5048413197740937
K = 2
P@2 =  0.3460905349794239
R@2 =  0.49432018598685235
F@2 =  0.40713316322908516
K = 3
P@3 =  0.2543209876543209
R@3 =  0.533001443001443
F@3 =  0.34434038235745984
K = 100
P@100 =  0.012172839506172655
R@100 =  0.7434049489605044
F@100 =  0.02395345461426251

chronos: limited labels (train+valid+test)
K = 1
P@1 =  0.3424778761061947
R@1 =  0.25597421752289023
F@1 =  0.29297418218915544
K = 2
P@2 =  0.23141592920353982
R@2 =  0.3188068421254262
F@2 =  0.2681713133344389
K = 3
P@3 =  0.179941002949853
R@3 =  0.3516823736735242
F@3 =  0.23807109251115732
K = 100
P@100 =  0.010707964601769782
R@100 =  0.6061425889744472
F@100 =  0.021044168149754315


==> tables/temp_table.tex <==
\begin{table*}[t]
\centering
\caption{res}
\label{tab: res}
\begin{tabular}{llllll}
\toprule
Model                                                  & \multicolumn{2}{l}{Extra   pre-train}                                   & Raw   & Zero-Shot & No-Zero-Shot \\
\midrule
\multicolumn{2}{l}{Ground   Truth}                                                &                                              & 0.829 & 0.861     & 0.857        \\
\midrule
\multicolumn{2}{l}{TF-IDF+BertFNN}                                                &                                              & 0.552 & 0.517     & 0.614        \\
GPT2-Fine Tune                                         & Maven & Query: vul\_desc                             & 0.485 & 0.198     & 0.656        \\
\midrule
\multicolumn{1}{c}{\multirow{4}{*}{LLaMa7B-Fine Tune}} &                          & Query: vul\_desc                             & 0.52  & 0.184     & 0.694        \\
\multicolumn{1}{c}{}                                   &                          & Query: vul\_desc + search top 1              & 0.544 & 0.292     & 0.693        \\
\multicolumn{1}{c}{}                                   &                          & Query: vul\_desc + bert-re-rank search top 1 & 0.578 & 0.412     & 0.697        \\
\multicolumn{1}{c}{}                                   & Maven                    & Query: vul\_desc + bert-re-rank search top 1 & 0.589 & 0.458     & 0.694        \\
\midrule
LLaMa13B-Fine Tune                                     & \multicolumn{5}{c}{tbd}                                                                                   \\
\bottomrule
\end{tabular}
\end{table*}

==> temp/github-advisory.tex <==

github/advisory-database [GHSA-qhxw-54m9-6wwc] Jenkins Maven Plugin 2.17 and earlier bundled a version...
#3127 opened 16 hours ago by q5438722 • subscribed 16 hours ago • updated 3 hours ago

1

github/advisory-database [GHSA-ppg2-ww3w-hq84] The IronJacamar container before 1.0.12.Final for JBoss...
#3072 opened last week by q5438722 • subscribed last week • updated 3 days ago

1

github/advisory-database [GHSA-f5ch-36rg-vfcc] Cross-Site Request Forgery in Apache CXF Fediz
#3071 opened last week by q5438722 • subscribed last week • updated 7 hours ago

3

github/advisory-database [GHSA-4px2-gqhv-mrc7] OpenDaylight Karaf 0.6.1-Carbon fails to clear the cache...
#3070 opened last week by q5438722 • subscribed last week • updated 5 hours ago

4

github/advisory-database [GHSA-c2fp-mpmm-cqxv] The WSDL/WADL import functionality in SoapUI before 4.6.4...
#3068 opened last week by q5438722 • subscribed last week • updated 6 hours ago


def generate_inputs(reports, folder_name, language='Java', prefix='maven:'):
    train_sep_idx, valid_sep_idx = int(len(reports) * 3 / 5), int(len(reports) * 4 / 5)
    train_conversation = [construct_conversation(vuln, language, prefix) for vuln in reports[:train_sep_idx]]
    valid_conversation = [construct_conversation(vuln, language, prefix) for vuln in reports[train_sep_idx:valid_sep_idx]]
    test_conversation = [construct_conversation(vuln, language, prefix) for vuln in reports[valid_sep_idx:]]
    
    target_path = os.path.join('/data/chentianyu/libgen/inputs/', folder_name)
    if not os.path.isdir(target_path):
        os.mkdir(target_path)
    target_train = os.path.join(target_path, 'train.json')
    target_valid = os.path.join(target_path, 'valid.json')
    target_test = os.path.join(target_path, 'test.json')
    
    with open(target_train, 'w') as f:
        json.dump(train_conversation, f)
    with open(target_valid, 'w') as f:
        json.dump(valid_conversation, f)
    with open(target_test, 'w') as f:
        json.dump(test_conversation, f)

==> temp/gpt-result.tex <==
0个搜索结果：0536/0.463（后处理前），0.676/0.591（后处理后）
1个搜索结果：0.730/0.630（后处理前），0.782/0.676（后处理后） 
2个搜索结果：0.726/0.624 （后处理前），0.773/0.665（后处理后） 
3个搜索结果：0.742/0.638 （后处理前），0.784/0.676（后处理后） 
5个搜索结果：0.741/0.638 （后处理前），0.792/0.683（后处理后） 
10个搜索结果：0.744/0.642（后处理前），0.797/0.690（后处理后） 
20个搜索结果：0.734/0.634（后处理前），0.792/0.685（后处理后） 

==> temp/icse24_review_response.tex <==
maybe considering the following paper:
https://aclanthology.org/2023.acl-long.855.pdf












Meta Review:

However, the reviewers decided to reject the paper, due to the following important weaknesses:

* Missing or unfair comparison with some important baselines (Review A and Review B)
[We have addressed this issue by re-running Chronos (achieving similar results) and using the same evaluation metrics in the preceding work.]

* Experimental settings and metrics are unclear or not well-designed
[Clarify the the experimental settings use the same evaluation metrics in the preceding work]

* Missing deep insights into the experimental results
[Add a motivating example to illustrate the importance of this problem, and add tow case studies to show the effectiveness of each component]


Weakness:
Reviewer A
----------
- potential unfair comparison with the state-of-the-art approach Chronos
- questionable/redundant relative precision metrics 
(other string similarity measures, such as n-grams? )
- sloppy runtime analysis (lack of details)
- missing discussion of the implications of the results 
- English needs to be improved

Reviewer B
----------
- unclear problem/motivation
- confusing terminology and setup
- potentially misleading results

Reviewer C
----------
- The motivation of proposing the generative approach is weak and unclear.
- The rationale behind unsupervised fine-tuning is questionable.
- Limited novelty and soundness in supervised fine-tuning.
- The used dataset is small-scale and only subset of prior studies.
- Missing NER-based approaches as baselines.
- Limited improvement over VulLibMiner.





Review #128A
===========================================================================

Overall merit
-------------
1. Reject

Paper summary
-------------
The paper presents VulLibGen, an approach that give the description of a vulnerability outputs a list of potential vulnerable Java libraries. VulLibGen utilizes the LLaMa models and adds two stages of fine-tuning to improve upon existing approaches. First, it in the unsupervised stage it fine tunes the LLaMa models with the descriptions of Maven Java libraries. Next, in the supervised stage it first uses an existing approach to generate names of potential vulnerable libraries to increase its performance in detecting zero-shot libraries. Second, to mitigate the hallucination problem of LLMs, VulLibGen post-processes generated library names using a technique based on Levenshtein to obtain library names that exist. The evaluation of VulLibGen is performed with a dataset curated in some other work. VulLibGen's performance is compared to three existing approaches and using various configurations. The results show that VulLibGen outperforms existing approaches in terms of f1-score. They also show only small differences in the performance when using LLaMa-7B and LLaMa-13B and when not fine-tuning these LLMs. Both techniques added in the supervised stage show to increase the performance of VulLibGen, in particular for detecting zero-shot libraries. The analysis of the runtime shows that VulLibGen takes significantly longer to train and to predict potentially vulnerable libraries.

Overall Comments for authors
----------------------------
The ideas of using potential vulnerable library names to improve zero-shot prediction and the post-processing step to mitigate LLMs hallucinations are promising and have the potential to advance the state-of-the-art in identifying vulnerable third-part libraries. That said, my main issue is with the comparison with existing approaches, most prominently Chronos. Without a detailed explanation of the differences in the results reported in the original Chronos paper [28] and this submission, it is unclear to me, whether the shown improvements over Chronos are valid.

Strengths
---------
+ input augmentation technique for improving zero-shot prediction 
+ post-processing step to deal with LLMs hallucinations

Weaknesses
----------
- potential unfair comparison with the state-of-the-art approach Chronos
[We have addressed this issue by re-running Chronos (achieving similar results) and using the same evaluation metrics in the preceding work.]

- questionable/redundant relative precision metrics
[use the same evaluation metrics as that of Chronos.]

- sloppy runtime analysis
[add evaluation details in runtime analysis: evaluate on ten epoches and use the average time consumption as the runtime overhead]

- missing discussion of the implications of the results
[add discussion of identifying vulnerable library versions]

- English needs to be improved
[refine this whole paper with ChatGPT]

Comments on Rigor
-----------------
The technical contribution, namely the VulLibGen approach is presented in Section 3. The stages of fine-tuning the input to the LLaMa model and post-processing the library names are well presented. Regarding the post-processing of library names, I only have a minor question: did you also experiment with other string similarity measures, such as n-grams? 

The evaluation setup is presented in Section 4. For the evaluation, the dataset created in a recent work [10] was used. Why was only that dataset used and not also a dataset from some state-of-the-art approach, such as Chronos? In my opinion, it would improve the validity of the results and allow for a more fair comparison with existing approaches when using (or adopting) a dataset that was used in previous studies. 

The metrics R, P, and F1-Score for evaluating and comparing the approaches are OK. They were also used in previous research.

RQ2 is misleading and should be rephrased to, for example: To what extent can the input augmentation improve the performance of VulLibGen? This way, it is clear that this RQ is about evaluating the contributions of the input augmentation techniques. 

I did not fully understand the explanations at the begin of Section 5.1. please explain why three testing sets were used, and in particular, why was Raw used? 

Please also better explain the maximum value of the ground truth. Why exactly can the approaches not achieve 1.0? I did not fully understand the argument at the begin of Section 5.1. 

Why are the values reported for Chronos so different to the values reported in [28]? This needs to be explained in detail to clearly show whether VulLibGen outperforms Chronos.

The comparison with VulLibMiner is questionable because this approach was not peer-reviewed, yet and its results might be biased. In my opinion, it might be better to remove the comparison with VulLibMiner and use the space for a detailed comparison with the other state-of-the-art approaches.

Concerning RQ2, I did not fully understand the reasons for using the relative precision metrics. Why not simply comparing the results for R, P, and F1-score of the different configurations? What are the insights that the authors would like to add with the relative precision metrics?

The values in Table 8 mainly show, at least in my opinion, that the post-processing technique helps to improve the F1@1 score of zero-shot identification. I suggest to stress this finding in the answer to RQ3 instead of reporting the average improvement.

The presentation of the results for the runtime are confusing. In Table 11, are these really minutes? Are the values the total time for predicting the names for all 633 vulnerabilities? How exactly is the average end-t-end time of 6 seconds computed? What is the post-processing time for Chronos? Did you do multiple runs to obtain the runtimes or only a single rund per approach? If so, the runtime might be biased because the computer might have been busy for one approach in that run.

The discussion of the applicability of the approach to other programing languages should be moved to the threats to external validity. The discussion on the larger pre-trained language models could be moved to threats to internal validity. Instead Section 6 could include a discussion of implications of the findings on research and practice, i.e., what do the findings mean for researchers; what do they mean for practitioners? That said, I suggest to structure Section 6 into:
6. Discussion
6.1 Implications
6.2 Threats to validity

Regarding the related work, I miss a discussion of the differences to approaches to identify vulnerable library versions.

Comments on the Relevance of the Contribution to SE
---------------------------------------------------
There are several approaches which aim to identify vulnerable libraries, however, as mentioned in the introduction existing approaches have some problems that VulLibGen aims to address. In that sense, the addressed problem and presented contributions are relevant to advance the field on this problem.

"Considering the large number of collected libraries (e.g., 310,844 in Maven) for comparison compared, this step cannot be avoided; otherwise, it might cost them two years to identify all vulnerable libraries [10]." -> in my opinion, this is only true when an engineer wants to classify all libraries and all vulnerabilities. I assume that, in practice, this classification is done incrementally, for instance, only when planning to use a library. Furthermore, the classification of libraries and vulnerabilities can also be parallelized to reduce the total time it will take.

The ideas for improving, in particular zero-shot identification, are well motivated and could make a relevant contribution. However, the relevance is questionable, mainly because I miss a detailed comparison and discussion with recent state-of-the-art approaches. Most notable, the comparison with Chronos raises a major issue: Chronos (according to [28]) also aims to improve zero-shot identification and reports F1@1 (and F1@2, F2@3) scores (e.g., F1@1 = 0.67) that are way higher as reported in this submission. Why is that the case? Is it because Chronos was evaluated with a different dataset? Is the dataset that is used in the submission allowing a fair comparison with Chronos? Section 2.2. tries to provide some background information on Chronos but lacks details to fully understand the differences in the performance. Thi issue needs to be clarified otherwise it remains unclear whether VulLibGen really outperforms the state-of-the-art, i.e., Chronos.

Comments on Novelty
-------------------
There exist several approaches for identifying vulnerable libraries and some of them, such as Chronos, also address the problem of zero-shot identification. Therefore, the problem is not new. 

The main novelties that also seem to improve the performance of VulLibGen concern the two supervised fine-tuning techniques: 1) the technique to augment the input to the LLaMa models by providing names of potentially vulnerable libraries (using TD-IDF or VulLibMiner); and 2) the technique to post-process the names output by the LLaMa  using Levenshtein. These novelties and the problems they aim to address are well motivated in the introduction.

Comments on Verifiability and Transparency
------------------------------------------
A link to a replication package is provided in the submission. It contains the VulLib dataset that was used for the evaluation and a short description of it. The source code for performing the experiments, however is not provided. This makes replicating the studies difficult. As a reason the authors mention "due to the security requirement of our industry partner". However, in the paper I did not read anything about an industry partner so I do not understand this reason.

Comments on Presentation
------------------------
Overall, the paper is well structured and quite written. There are a couple of potentially  misleading sentences and phrases that need to checked and corrected.
l14, l71 (and other places): ... the name list of libraries ... -> better write "list of names of libraries"
l20,l107: avoid using adjectives, such as "enormous" because it is not really clear what exactly it means (can you measure it?)
l104: ... to generate the names of affected libraries of a given ....
l223: ... is one ... XML approach that identifies ...
l519: what do you mean by "included" - do you mean "one"  here?
l552: To evaluate VulLibGen, we selected ...
l895: the number 2,34 seems to miss a digit
l903: To show how ...


* * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * *


Review #128B
===========================================================================

Overall merit
-------------
1. Reject

Paper summary
-------------
This paper focuses on the problem of identifying vulnerable third-party libraries, given a vulnerability report. The paper proposes VulLibGen, which is a generative approach to generate the affected libraries of a given vulnerability. VulLibGen first uses an off-the-shelf LLM to determine a package name from a given Java library and then uses this fine-tuned LLM to determine affected packages related to the given vulnerability. Additionally, the authors experiment with adding top k search results of other techniques in the prompt as well as post-processing affected libraries with levenshtein distance.

Overall Comments for authors
----------------------------
I'm honestly very confused about the use case this paper is tackling. The paper describes the problem as "given a vulnerability report, we want to identify vulnerable libraries". Given that and from the title, this could be understood as given a vulnerability, identify the impacted libraries (i.e., those that have the vulnerable library as their dependency). However, after reading through the paper, it seems the task is really "given a vulnerability report (for a specific library such as the description in Table 2?), we want to identify the vulnerable components in this library as identified by their maven artifact names". I'm honestly not sure if that is the given problem or not and the paper does not provide any motivating example to explain why this task (whatever it actually is) is important (or real). Perhaps the paper can provide a real example of a complete CVE that doesn't mention the library name the vulnerability is found in and how that prevents others from figuring out if they are affected (or even tools like dependabot from issuing warnings based on the CVE)? Or perhaps any more general background on this so the reader can appreciate how difficult the problem is?

I also found the terminology and evaluation setup of the paper is also confusing:

- the paper keeps using the term "library name" while it is talking about the maven package name that can be added as a dependency in gradle, maven etc. Perhaps this should be made clear.
- "zero-shot learning" In Section 2.1, the paper says "The affected libraries of V������ might not occur in the training dataset due to the data imbalance of the large number of Java libraries (310,844) and the small number of affected Java libraries (2,811 and 985 in two recent work [10, 11])". Does this mean that a given library is considered as zero-shot if the model has not observed **a vulnerability** for it before? However, (1) the model has observed this library through the unsupervised fine-tuning step and already has information on its description. It just hasn't seen it associated with a vulnerability before so is this really an unseen library? and (2) if the model has seen a vulnerability for this library before, what is really the point of the given task? So the experiment would ask it about a different unseen vulnerability?
- I think the bigger question should have been what happens with vulnerability reports and libraries that have been issued after the model's training cut-off date? This is truly unseen data that the model has no information about and would show the generalizability/transferability of the model's learning. 
- What data was Llama trained on? Does it already have knowledge of certain CVEs in its training data (Regardless of what is used in the supervised fine tuning). In general, I think there is a risk of data leakage and/or memorization here.
- I do not understand what "the ground truth results" mean and why can't 1.0 be achieved. (Lines 617-621)
- I also don't understand the point of the task of providing the model with the top X libraries suggested by another approach. So are we then just using the model as a post-processor? I know that the results show that it sometimes provides suggestions not in the list, but wouldn't that mean that we are incurring the additional costs of running these techniques (Along with the criticisms about them in the intro). Before Summary 1, the paper says "Focusing on the top libraries can be practical in some cases. For example, developers might not concern about vulnerable libraries not being used in their project" -- but then again, this confuses me more as i don't understand the use case. So a developer takes a vulnerability report that doesn't mention the libraries it affects and they want to know if it is related to the dependencies of the project they are working on?
- Am I understanding the results in Table 5 correctly that not using the unsupervised fine-tuning on zero-shot libraries leads to a better F1 score?
- I don't understand the metrics in 5.2.1
- In the discussion, I don't understand how the authors reached the conclusions on Python library pairs. I don't believe this was discussed in the paper
- All in all, I would like to see some practical use case for this work and the implications it has.


Questions about technique:
- what happens if the name of the package in the unsupervised fine-tuning stage is wrong?

Strengths
---------
+ large-scale experiment
+ various research questions and impact of different steps are explored

Weaknesses
----------
- unclear problem/motivation
[add a motivating example]

- confusing terminology and setup
- potentially misleading results

Artifact Assessment
-------------------
4. Good (largely as promised)

Comments on Verifiability and Transparency
------------------------------------------
the artifact contains no source code but contains all the data used and produced. It is not clear why the authors did not share their source code though, but I appreciate that the authors provide the complete data.

The data does however confirm my confusion about the problem being tackled (at least in terms of how unclearly it is explained in the paper). For example, the first CVE description is "JGroups before 4.0 does not require the proper headers for the ENCRYPT and AUTH protocols from nodes joining the cluster, which allows remote attackers to bypass security restrictions and send and receive messages within the cluster via unspecified vectors." -- clearly mentioning the library name itself so I guess the issue is the specific jgroups artifact that would appear as a Python dependency?

Comments on Presentation
------------------------
Generally OK but some unclear sentences here and there.


* * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * *


Review #128C
===========================================================================

Overall merit
-------------
1. Reject

Paper summary
-------------
This paper aims to address the issue of incomplete or incorrect vulnerability information in third-party library databases like NVD. A significant portion of these databases lacks information about which libraries are vulnerable, leading to potential security risks. In response to this problem, the paper introduces a novel generative approach called VulLibGen. VulLibGen leverages recent advancements in Large Language Models (LLMs) and takes only the vulnerability description as input to generate accurate lists of vulnerable libraries. It also incorporates techniques for identifying zero-shot vulnerable libraries (those not seen during training) and post-processing to mitigate inaccuracies. The paper evaluates VulLibGen against three state-of-the-art/practice approaches using an open-source dataset (VulLib). The results demonstrate that VulLibGen outperforms existing methods, achieving an average F1 score of 0.626 compared to the state-of-the-art/practice approaches' 0.561.

Overall Comments for authors
----------------------------

This paper tackles a critical issue in the field of software composition analysis, namely the accuracy of vulnerability information in third-party library databases such as NVD. This is a relevant and significant topic within the realm of software security. The paper's exploration of using LLMs to generate precise lists of vulnerable libraries presents an innovative and interesting idea. This investigation into LLMs in this context constitutes a valuable contribution to the field. 

One notable weakness in this paper is the lack of a clear and compelling motivation for proposing the generative approach, VulLibGen. In Section 1, the authors argue that “NER and XML approaches cannot distinguish vulnerable libraries with similar names.” I am quite confused with this statement since there is not any reasons or references given. AFAIK, NER-based approach labels and extracts the software names and components from the CVE description, like VIEM did [15]. Obviously, it can clearly distinguish vulnerable libraries with similar names owing to the extractive nature. Also, how XML approaches can’t do this is not clear. Regarding the TF-IDF, why do they suffer from false negatives? The claim of “they still suffer from highly inaccurate results” needs further clarification and evidence. For example, VIEM even achieves over 97\% precision and recall. Although I like the idea of identifying vulnerable libs proposed, the benefit of it should be carefully considered. Being able to work on zero-shot (or should be named as unseen) is not a significant difference between generative LLM and NER/TFIDF.

Moreover, the rationale behind employing unsupervised fine-tuning in VulLibGen is not adequately justified and appears somewhat ad hoc. Since LLMs have already learned the prior knowledge of libs and CVE reports, it is intuitively unnecessary to “activate” their prior knowledge of Java libraries. And the experimental results (Table 5) also indicate the little gain or even worse performance using such a step. A more detailed explanation is required to clarify the reasoning behind this approach. 

The paper lacks sufficient demonstration of novelty and soundness in the supervised fine-tuning aspect of VulLibGen. The most problematic part is to adopt the existing VulLibMiner as one main component. This not only weakens the novelty, but also makes the proposed approach unsound, with respect to the drawbacks of existing work discussed in the paper. Now that TF-IDF techniques are blamed to be inaccurate and inefficient (Sec. 1), how can VulLibGen be more effective and efficient? Will the recommended results have a negative impact on VulLibGen? And is the time cost always greater than TF-IDF techniques? 

Another notable limitation is the use of a small-scale dataset, which is comparatively limited in scope compared to prior studies.  For example, in Stefanus et al. [17], the dataset consists of more than 7,600 samples. However, in this work, only less than 3,000 samples are used for training and evaluation.  This raises another issue about the decision of only considering Java libs.  All in all, this may not adequately represent the diversity of vulnerabilities and libraries encountered in real-world scenarios. 

The omission of NER-based approaches as baselines is also a significant oversight, as these approaches are commonly employed for similar tasks and should be considered for benchmarking VulLibGen. 

Finally, the paper claims that VulLibGen outperforms existing methods, but the extent of improvement over VulLibMiner is relatively limited.  This again involves the concern of novelty and effectiveness of the proposed approach.

In summary, while the paper addresses a critical issue in software security and introduces an intriguing approach using LLMs, it should address the mentioned weaknesses to present a more convincing case for its contribution.

Strengths
---------
+ An important and relevant topic on software composition analysis of vulnerabilities.
+ Interesting idea to consider the LLM for identifying vulnerable libs in a generative way.

Weaknesses
----------
- The motivation of proposing the generative approach is weak and unclear.
- The rationale behind unsupervised fine-tuning is questionable.
- Limited novelty and soundness in supervised fine-tuning.
- The used dataset is small-scale and only subset of prior studies.
- Missing NER-based approaches as baselines.
- Limited improvement over VulLibMiner.

Comments on Rigor
-----------------
This paper does not provide sufficient justification behind the proposed approach, the efficacy of unsupervised fine-tuning, and the soundness of supervised fine-tuning using VulLibMiner. Furthermore, there raises questions about the small-scale dataset and its representativeness, which is another important aspect that impacts the rigor of the study. The absence of NER-based approaches as baselines is also noted as a potential gap.

Comments on the Relevance of the Contribution to SE
---------------------------------------------------
The paper's contribution is highly relevant to the field of SE, particularly in the context of software security. The issue of incomplete or incorrect vulnerability information in third-party library databases directly impacts the security and reliability of software systems.

Comments on Novelty
-------------------
While the paper introduces an interesting approach using LLMs to generate lists of vulnerable libraries, its novelty compared to existing work is not well-established. Please refer to the detailed comments above.

Comments on Verifiability and Transparency
------------------------------------------
No source code or dataset provided, which hinders the reproducibility and practical applicability of the proposed approach.

Comments on Presentation
------------------------
This paper is well-structured, and I appreciate the illustrative examples that makes it easy to follow.


* * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * *


Review #128D
===========================================================================

Meta-Review Recommendation before Revision
------------------------------------------
D. Reject

Strengths
---------
Thank you for submitting your work to ICSE 2024. The reviewers would like to highlight the following strengths of the work:
* The work presents an important topic in SE with an interesting approach like using LLM.
* Evaluation comes with extensive comparison experiments

Weaknesses
----------
However, the reviewers decided to reject the paper, due to the following important weaknesses:

* Missing or unfair comparison with some important baselines
* Experimental settings and metrics are unclear or not well-designed
* Missing deep insights into the experimental results

Please see the reviews for more details, which we hope will be helpful for future improvement of the paper.

—-


==> temp/plan.tex <==
Major Issue:
做一些empirical study，看一看模型直接生成会遇到哪些问题，这里面具体有哪些幻觉的场景，这些问题我们通过什么方法解决的
多加几个模型
跨语言的场景下的效果
其他方法是怎么解决幻觉的


Storyline:

强调我们旨在解决模型的幻觉问题，其中包括两个核心的技术：few-shot样本的选取，基于制品仓数据的增强
是否可以decode的时候直接加上数据库的知识

Current:
1.用ChatGPT跑一下结果，0/1/2/3/5/10/20-shot的结果:2789/550个漏洞
2.扩展到别的语言上：考虑veracode的数据集




Minor issuse:
1.强调我们是用大预言模型来做（不要提生成式语言模型）
2.abstract里最好说明，为什么include a complete name list很重要

max
(0.7090909090909091, 0.5414553325462416, 0.6140373561631741)

avg
(0.6431515151515151, 0.5019028794437886, 0.5638153067606327)

prompt-tuning 
2-shot
(0.03333333333333333, 0.03333333333333333, 0.03333333333333333)

(0.03333333333333333, 0.03333333333333333, 0.03333333333333333)

3-shot
(0.07256637168141593, 0.05567712523464736, 0.06300961937390981)

(0.12743362831858407, 0.10184231697506034, 0.1132097477725503)

4-shot
(0.07079646017699115, 0.05483775811209439, 0.06180353109604439)

(0.11150442477876106, 0.09073746312684365, 0.1000547288854927)


==> temp/post.tex <==
#!/usr/bin/env python
# coding: utf-8

# In[1]:


import os, sys
import json
import time, datetime
import pandas as pd


import Levenshtein

weights = (1, 4, 4)
metric_k = 1

def f1(prec, rec):
    if prec < 0.01 and rec < 0.01:
        return 0.0
    return 2 * prec * rec / (prec + rec)


def precision(entry, k):
    preds = entry['predict_labels']
    labels = entry['labels']
    return sum([item in labels for item in preds[0:k]]) / k



def recall(entry, k):
    preds = entry['predict_labels']
    labels = entry['labels']
    if len(labels) == 0: return 0.0
    return sum([item in labels for item in preds[0:k]]) / len(labels)


def cloest_artifact_new(artifact_id, artifacts):
    if artifact_id in artifacts:
        return artifact_id
    
    global weights
    distances = [(Levenshtein.distance(artifact_id, item, weights = weights), item) for item in artifacts]
    distances.sort()
    # print(f'wow {distances[0][1]}')
    return distances[0][1]

def cloest_group(group_id, groups):
    if len(groups) == 0:
        return group_id
    if len(groups) == 1:
        return next(iter(groups))
    
    global weights
    distances = [(Levenshtein.distance(group_id, item.split(':')[-2], weights = weights), item) for item in groups]
    distances.sort()
    return distances[0][1]


    
def closest_lib_new_ad(label, artifacts, lib_names):
    if label in lib_names:
        return label
    if len(label.split(':')) > 1:
        group_id, artifact_id = label.split(':')[-2], label.split(':')[-1]
    else:
        group_id, artifact_id = "", label.split(':')[-1]
    if artifact_id in artifacts:
        return cloest_group(group_id, artifacts[artifact_id])
    else:
        advanced_artifact_id = cloest_artifact_new(artifact_id, artifacts)
        return cloest_group(group_id, artifacts[advanced_artifact_id])


def closest_lib_raw(label):
    if label in lib_names:
        return label
    artifact_id = label.split(':')[-1]
    if artifact_id in artifacts:
        return next(iter(artifacts[artifact_id]))
    else:
        return label


def post_process(raw_preds, maven_path = '/clouddragonData/tianyu/vul_mapping/top_names.json'):
    with open(maven_path, 'r') as maven_f:
        lib_names = json.load(maven_f)
    
    artifacts = {item.split(':')[2]: set() for item in lib_names}
    for item in lib_names:
        components = item.split(':')
        artifacts[components[2]].add(item)
        

    post_preds = [closest_lib_new_ad(item, artifacts, lib_names) for item in raw_preds]
    return post_preds


    
if __name__ == '__main__':
    st_time = datetime.datetime.now()
    restrict_lib = len(sys.argv) > 4 and sys.argv[4][0] == 'r'
    post_process(test_path = sys.argv[1], output_path = sys.argv[2], maven_path = sys.argv[3], restrict_lib = restrict_lib)
    end_time = datetime.datetime.now()
    print(sys.argv[1], st_time, end_time, end_time - st_time)



def get_words_from_object_name(object_name):
    object_name = object_name.strip('/')
    object_name = object_name.replace('pypi:', '').replace('maven:', '').replace('https://github.com/', '').replace(
        "pkg:cpp/", "")
    words = re.split(r'[:|/]', object_name)
    return words


==> temp/rag-res.tex <==
 rerank_20_llama_13b_932.json
0.7026548672566372 0.5453842470214152 0.6141103933531303 


1358it [00:09, 141.19it/s]

 top_5_13b_932.json
0.6530973451327433 0.5019336857832433 0.5676238106914944 


1579it [00:15, 99.63it/s]

 top_20_13b_932.json
0.6230088495575221 0.483540589204306 0.5444855071846124 


1731it [00:20, 85.93it/s]

 top_10_7b_932.json
0.5911504424778761 0.45520591502892394 0.5143470982086445 


1250it [00:07, 177.77it/s]

 top_10_13b_932.json
0.6353982300884956 0.490222771328966 0.5534485956805287 


850it [00:03, 254.16it/s]

 rerank_10_llama_7b_932.json
0.6654867256637168 0.5166969313871969 0.5817284767531629 


1472it [00:17, 83.06it/s]

 rerank_5_vicuna_7b_932.json
0.6849557522123894 0.5304137455464888 0.5978592464835161 


866it [00:04, 197.59it/s]

 rerank_5_llama_13b_932.json
0.7008849557522124 0.5439093207677278 0.6124993782671817 


981it [00:03, 263.41it/s]

 rerank_10_llama_13b_932.json
0.7044247787610619 0.5475966364019462 0.6161885647898775 


946it [00:02, 357.82it/s]

 rerank_20_llama_7b_932.json
0.6831858407079646 0.5316084358119755 0.5979405125089737 


1111it [00:13, 84.94it/s]

 top_20_7b_932.json
0.6088495575221239 0.4702522698540398 0.5306503596988179 


1176it [00:08, 133.41it/s]

 top_5_7b_932.json
0.5628318584070796 0.4331873730988776 0.4895721819970983 


1072it [00:04, 266.02it/s]

 rerank_5_llama_7b_932.json
0.6778761061946903 0.5265936865494388 0.5927342967590264 


1495it [00:15, 93.76it/s]

 rerank_10_vicuna_7b_932.json
0.7061946902654868 0.5462973604566524 0.6160395110501589 





2443it [00:33, 72.51it/s] 

 vicuna_top_3_7b_932.json
0.40353982300884955 0.321710339807685 0.35800869890725184 


1006it [00:03, 267.28it/s]

 rerank_20_llama_13b_932.json
0.7026548672566372 0.5453842470214152 0.6141103933531303 

1358it [00:09, 144.37it/s]

 top_5_13b_932.json
0.6530973451327433 0.5019336857832433 0.5676238106914944 


732it [00:01, 480.49it/s] 

 vicuna_rerank_10_13b_699.json
0.7185840707964601 0.5609897329808833 0.6300821176713747 

2000it [00:25, 77.61it/s]

 vicuna_top_2_7b_932.json
0.39823008849557523 0.3180230241734667 0.35363570452991355 


1579it [00:16, 96.90it/s]

 top_20_13b_932.json
0.6230088495575221 0.483540589204306 0.5444855071846124 

1731it [00:19, 88.70it/s]

 top_10_7b_932.json
0.5911504424778761 0.45520591502892394 0.5143470982086445 

1418it [00:19, 72.76it/s]

 vicuna_top_3_13b_932.json
0.4176991150442478 0.3356167873424511 0.37218605002970817 

1487it [00:08, 166.48it/s]

 vicuna_top_1_13b_932.json
0.6088495575221239 0.4708548825805464 0.5310338204944987 


1250it [00:07, 175.64it/s]

 top_10_13b_932.json
0.6353982300884956 0.490222771328966 0.5534485956805287 

850it [00:03, 273.00it/s]

 rerank_10_llama_7b_932.json
0.6654867256637168 0.5166969313871969 0.5817284767531629 


2513it [00:39, 63.91it/s] 

 vicuna_top_1_7b_932.json
0.5964601769911504 0.46172508907022186 0.5205149555202871 

1472it [00:17, 84.58it/s]

 rerank_5_vicuna_7b_932.json
0.6849557522123894 0.5304137455464888 0.5978592464835161 


866it [00:04, 198.56it/s]

 rerank_5_llama_13b_932.json
0.7008849557522124 0.5439093207677278 0.6124993782671817 


1121it [00:03, 294.46it/s]

 vicuna_top_20_13b_932.json
0.679646017699115 0.5263289660192315 0.593241801171902 


981it [00:03, 300.64it/s]

 rerank_10_llama_13b_932.json
0.7044247787610619 0.5475966364019462 0.6161885647898775

946it [00:02, 382.69it/s]

 rerank_20_llama_7b_932.json
0.6831858407079646 0.5316084358119755 0.5979405125089737 

1111it [00:13, 84.38it/s]

 top_20_7b_932.json
0.6088495575221239 0.4702522698540398 0.5306503596988179 

1176it [00:08, 131.00it/s]

 top_5_7b_932.json
0.5628318584070796 0.4331873730988776 0.4895721819970983 


1072it [00:04, 265.39it/s]

 rerank_5_llama_7b_932.json
0.6778761061946903 0.5265936865494388 0.5927342967590264 

1028it [00:03, 271.99it/s]

 rerank_3_13b_932.json
0.7008849557522124 0.5456652492050722 0.6136111686856967 

1495it [00:16, 91.66it/s]

 rerank_10_vicuna_7b_932.json
0.7061946902654868 0.5462973604566524 0.6160395110501589 

1278it [00:19, 64.29it/s]

 vicuna_top_2_13b_932.json
0.4495575221238938 0.36194422097076967 0.401021312674374 


750it [00:01, 406.83it/s]

 vicuna_rerank_5_13b_699.json
0.7221238938053097 0.561727196107727 0.6319060415910492 

==============================================================

2443it [00:33, 73.34it/s] 

 vicuna_top_3_7b_932.json
0.3752212389380531 0.2978165344979504 0.3320678079628883 


1006it [00:03, 296.98it/s]

 rerank_20_llama_13b_932.json
0.6902654867256637 0.5347647779948664 0.6026457964294925 

1358it [00:08, 153.68it/s]

 top_5_13b_932.json
0.6017699115044248 0.45734800597632463 0.5197122332473436 


732it [00:01, 526.78it/s]

 vicuna_rerank_10_13b_699.json
0.6991150442477876 0.5448996283952036 0.6124486088363695 

2000it [00:25, 78.93it/s]

 vicuna_top_2_7b_932.json
0.36991150442477877 0.29682622687047466 0.3293631992930221 

1579it [00:16, 98.53it/s]

 top_20_13b_932.json
0.5982300884955752 0.4618591732751025 0.5212731872019049 

1731it [00:19, 86.86it/s]

 top_10_7b_932.json
0.5575221238938053 0.4273298088342337 0.48382059212587436 

1418it [00:19, 73.27it/s]

 vicuna_top_3_13b_932.json
0.3752212389380531 0.29962858675248066 0.33319119384074475 

1487it [00:08, 180.96it/s]

 vicuna_top_1_13b_932.json
0.5415929203539823 0.41451269968969096 0.46960741332845285 

1250it [00:06, 185.24it/s]

 top_10_13b_932.json
0.6 0.4611533157108379 0.5214929555040861 

850it [00:02, 288.45it/s]

 rerank_10_llama_7b_932.json
0.6513274336283186 0.5057824771099108 0.5694014021191773 


2513it [00:38, 65.39it/s] 

 vicuna_top_1_7b_932.json
0.5380530973451327 0.40892272918821604 0.46468375400878564 

1472it [00:17, 85.51it/s]

 rerank_5_vicuna_7b_932.json
0.6743362831858407 0.5215641880243649 0.588192185657849 


866it [00:04, 194.46it/s]

 rerank_5_llama_13b_932.json
0.6884955752212389 0.5337323296172852 0.6013155907164035 


1121it [00:03, 309.63it/s]

 vicuna_top_20_13b_932.json
0.6495575221238938 0.4980103819484351 0.5637773390880941 


981it [00:03, 309.90it/s]

 rerank_10_llama_13b_932.json
0.6902654867256637 0.5352072558709726 0.6029266651661188 

946it [00:02, 382.48it/s]

 rerank_20_llama_7b_932.json
0.6707964601769911 0.5209889667854269 0.5864773084223203 

1111it [00:13, 83.74it/s]

 top_20_7b_932.json
0.5716814159292035 0.4389838332758687 0.4966212097914062 

1176it [00:08, 135.56it/s]

 top_5_7b_932.json
0.5132743362831859 0.3910044822434204 0.4438731992733001 

1072it [00:04, 237.10it/s]

 rerank_5_llama_7b_932.json
0.6690265486725664 0.5186290847795273 0.584305108077029 


1028it [00:03, 311.91it/s]

 rerank_3_13b_932.json
0.679646017699115 0.5300176224954987 0.5955777366036475 

1495it [00:15, 94.57it/s]

 rerank_10_vicuna_7b_932.json
0.695575221238938 0.5374478029345285 0.6063720905473915 

1278it [00:19, 64.50it/s]

 vicuna_top_2_13b_932.json
0.41238938053097346 0.32861088763743634 0.3657640792047232 


750it [00:01, 466.04it/s]

 vicuna_rerank_5_13b_699.json
0.7008849557522124 0.5447521357698348 0.6130334094474195 






==> threats.tex <==
\section{Threats to Validity} \label{sec:threats}

A major threat to external validity is that the maven corpus we used during post-processing does not include all Java libraries.
This corpus contains Java libraries and descriptions until 2022, so new libraries or private ones are not contained in this corpus and cannot be generated by \detector{}.
This threat could be reduced by extending this corpus with the libraries used by the developers themselves.
The threats to internal validity are instrumentation effects that can bias our results. Faults in our tool or its underlying third-party tools (e.g., the entity-linking approaches for library recommendation) might cause such effects. 
To reduce these threats, we manually inspect the intermediate results to make sure that the accuracy of their recommended libraries is quite similar to the reported values in their paper~\cite{vullib}.


